Deep Generative Modeling for Volume Reconstruction in Cryo-Electron Microscopy

Recent breakthroughs in high-resolution imaging of biomolecules in solution with cryo-electron microscopy (cryo-EM) have unlocked new doors for the reconstruction of molecular volumes, thereby promising further advances in biology, chemistry, and pharmacological research. Recent next-generation volume reconstruction algorithms that combine generative modeling with end-to-end unsupervised deep learning techniques have shown promising preliminary results, but still face considerable technical and theoretical hurdles when applied to experimental cryo-EM images. In light of the proliferation of such methods, we propose here a critical review of recent advances in the field of deep generative modeling for cryo-EM volume reconstruction. The present review aims to (i) unify and compare these new methods using a consistent statistical framework, (ii) present them using a terminology familiar to machine learning researchers and computational biologists with no specific background in cryo-EM, and (iii) provide the necessary perspective on current advances to highlight their relative strengths and weaknesses, along with outstanding bottlenecks and avenues for improvements in the field. This review might also raise the interest of computer vision practitioners, as it highlights significant limits of deep generative models in low signal-to-noise regimes -- therefore emphasizing a need for new theoretical and methodological developments.

==> CryoReview 2021 (6)/appA-abinitio-vs-refinement.tex <==

Section~\ref{sec1-generative_models_and_lvms} established how cryo-EM methods target either homogenenous or heterogeneous reconstruction, and refined these categories by drawing a distinction between methods that are reference-based, and those that are reference-free --- that is, those that do not try to parametrize heterogeneity as "small" deviations from a reference shape. Here, we introduce an additional nuance between these methods, and differentiate between methods that operate \textit{ab-initio} (ie. from scratch) , or \textit{by refinement} (ie, "warm-starting " the algorithm by using an existing and external volume estimate, such as for example a low resolution estimate). While, for the sake of clarity and conciseness, we did not elaborate on this distinction in the main text, the latter introduces an other (independent) axis of variation in our comparison of existing methods. In fact, methods can target reference-free heterogeneous reconstruction whilst warm-starting their algorithm close to a known solution (as is done in the heterogeneous version of \relion), or vice versa, prefer to opt for reference-based heterogeneity, with no prior knowledge of what the reference should look like (e.g. \threedflex).

This distinction can be understood as a way of infusing further knowledge into the recovery. \textit{From a statistical and compute science perspective}, choosing to operate by refinement depends on whether or not we have a reasonable prior for the shape (refinement), or if we'd rather not bias the algorithm with external inputs (ab initio). In this high-dimensional (and highly non-convex) setting, imposing a specific starting point for the algorithm is in fact likely to introduce an additional bias to the solution --- thereby potentially allowing it to recover more easily interesting structures. Conversely, in the absence of good guesses, ab initio methods prefer to use a random initialization. \textit{From a biological perspective}, this boils down to how much we trust potential external reconstruction methods, and we think that they could be instrumental in recovering the structure.

% \paragraph{Difference between Ab-initio/Refinement and Reference-Free/Reference-Based} Ab-initio and refinement methods address the purpose of the reconstruction: whether we want a rough first estimate of the molecular shape, or we are interested in a high-resolution volume. They also differ in the initialization of the reconstruction: ab-initio operate with a initial volume that has been randomly initialized, while refinement have a blunt homegeneous reconstruction as the initial volume. Reference-free or reference-based methods address the parametrization of the molecular volume, which is represented as deviations from a template. We shall use the word "initial volume" to refer to the initialization in refinement methods, and "template volume" to refer to the reference volume used to parametrize the conformation landscape.

\paragraph{Ab-initio vs refinement: Pros, Cons, Discussions.} Figure~\ref{fig:cryoem_recon} summarizes the methods performing ab-initio reconstruction versus refinement. While ``bias-free'', ab-initio methods can be challenging to fit: due to the highly non-convex, non-linear nature of the problem, these methods are at higher risk of  inconsistencies, especially when targeting an heterogeneous reconstruction. In fact, solutions initialised at various random points might not necessarily converge to same point, and/or get stuck in local minima. By contrast, warm-starting the problem can yield faster, and more consistent convergence towards the solution. Warm-starting the solution might also increase consistency across recovered conformation, thereby preventing aberrations. 
% This explains why many heterogeneous reconstruction methods prefer refinement approaches --- with the exceptions of CryoDRGN, MultiCryoGAN and E2GMM. We note that refinement strategies are not solely restricted to heterogeneous reconstructions. 
Homogeneous reconstruction approaches can also benefit from warm-starting strategies: in RELION \cite{Scheres2012RELION} for instance, the hypothesised template is converted into Fourier coefficients, that are used in the initialisation part of the inference process. Refinement for homogeneous reconstruction holds several advantages, especially if the homogeneous reconstruction is either slow or very sensitive to initialization. 

Yet, refinement also holds several disadavantages. This approach requires a two-step procedure and another fragmentation of the estimation pipeline, as it relies on a prior estimation of an initial "blunt" value by another pipeline. Moreover, as highlighted in the review of Bendory et al \cite{bendory2020single}, it also exposes this solution to model bias: the structure recovered will be biased towards our initial prior --- potentially hindering our ability to detect flaws in this original template or discovering new conformations. Finally, while the literature on the sensitivity of the methods to an erroneous warm-starting is also nonexistent, the impact of a wrong initialization could also either severely hinder the performance of the algorithm, or push the algorithm to hallucinate nonexistent solutions (allowing us to recover ``Einstein from noise'' \cite{henderson2013avoiding}--- see discussion in part \ref{sec3-discussion}). 

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{figs/cryoem_reconstruction_cleaned.pdf}
    \caption{Works differentiated by the objective of the reconstruction (homogeneous/heterogeneous), and its initialization (ab-initio/warm-start).}
    \label{fig:cryoem_recon}
\end{figure}

==> CryoReview 2021 (6)/appA2-details-input-domain.tex <==

\subsection{Details on Parameterizations using a Discrete Input Domain}


We give details on cryo-EM reconstruction methods which leverage a discrete input domain to represent the biomolecular volume:

\begin{itemize}
\item \relion-Class3D\cite{SCHERES2010295} and \cryosparc use discrete conformational heterogeneity through $K$ clusters and $z \in \{1, ..., K\}$, in Fourier space with a reference-free encoding. As a result, each of the $K$ volumes $\tilde{V}_z$ is parametrized by its $J$ 3D Fourier coefficients, where $J = D^3$. The target of inference is thus the coefficients $\tilde{V}_{j,k}$ for the volume corresponding to each of these $K$ clusters, where $j=1 \cdots J$ indexes the Fourier coefficients, and $k$ the $K$ clusters. \relion-Refine3D is a homogeneous reconstruction method where the volume is a single parameter $\tilde V$ independent of the image $X_i$.

\item \cryoposenet does not consider conformational heterogeneity: it is a homogeneous reconstruction method, where the volume is a single parameter $V$ independent of the image $X_i$. \cryoposenet operates in image space, using a reference-free encoding, where the volume is represented as 3D map over a discrete domain, i.e. as a set of image intensities on the voxel grid: $V \in \mathbb{R}^{D^3}$. \cryogan also uses the same representation in image space with a reference-free encoding for homogeneous reconstruction, while \multicryogan uses the same representation for heterogeneous reconstruction.

\item \threedflex models conformational heterogeneity through a continuous conformation variable $z$, in image space, with a reference-based encoding where the volume is represented as deviations from an initial template $V_0$. Here, Punjani \textit{et al.} propose learning a deformation field $U \in {\mathbb{R}^3}^{D^3}$ with respect to the conformation $V_0$, that is explicitly represented by the coefficients of its 3D vectors at each of the voxels of the discrete domain. Consequently, the function $V$ writes: $V(z) = f(U(z),V_0)$, where $f$ is a ``convection operator" used to deform the volume $V_0$ based on $U$, and $z$ is the conformation variable. The deformation flow $U$ is parametrized through a neural network.
\end{itemize}

\subsection{Details on Parameterizations using a Continuous Input Domain}

We give additional details on the parameterization of the biomolecular volume with (pseudo-)atome coordinates. Among this general
class of methods, different works differ in the interpretation given to the variable $c_j$ and in whether $A_j, \sigma^2_j$ are assumed
to be known:

\begin{itemize}
\item \textbf{ $c_j$ as  coordinates of ``coarse-grained atoms".} The $c_j$ are coordinates of ``coarse-grained atoms", which are not explicitly mapped onto groups of atoms within the molecular structure, nor are they linked by any molecular chain structure, but rather consist of independently moving ``blobs". \egmm introduces this approach and uses it in a reference-free encoding. The authors describe its benefits as (a) reducing the number of parameters to represent the molecule at any level of detail (in constrast with the grid-approaches) and (b) providing a natural way of modeling cryo-EM maps --- which, as described in the introduction, are the projections of the electrostratic potential "blob" around each atom. In \egmm, Chen \textit{et al.} use a conformation variable $z$ that encodes the coefficients $c_j, A_j, \sigma_j^2$ defining $V_z$ in Equation~\eqref{eq:mixture}.
\item \textbf{$c_j$ as 3D coordinates of groups of atoms.}  The $c_j$ are interpreted as coordinates of ``residues", \textit{i.e.} physical groups of atoms that constitute the molecular structure of proteins. \cryofold relies on this approach in a reference-free encoding. The conformation variable $z$ only encodes the coordinates $c_j$, while $A_j = A$ and $\sigma_j = \sigma$ are assumed known and fixed.
\item \textbf{$c_j$ as 3D coordinates of (pseudo)-atoms.} The $c_j$ are coordinates of actual atoms that constitute the molecular structure of proteins, or potentially pseudo-atoms: i.e. a 3D position that does not exactly correspond to the actual atom but averages known positions of real atoms. In \cryodeepmind, Rosenbaum \textit{et al.} explore this approach, using a reference-based encoding. In other words, Rosenbaum \textit{et al.} consider that a template molecular shape $V_0$ is given, with associated coordinates $c_j$ that form a ``base conformation", that is chosen as a folded molecular chain. The volume is here parametrized in terms of the deviations from that template, expressed as residuals, or small variations $\Delta c_j$ corresponding to different conformations relative to this base conformation. In this work, the conformation variable $z$ encodes the deviations $\Delta c_j$ while $A_j = A$ and $\sigma_j = \sigma$ are assumed known and fixed.
\end{itemize}

==> CryoReview 2021 (6)/appA4-relion-examples.tex <==
\paragraph{Example: Modeling Choices in \relion-Refine3D \cite{Scheres2012RELION} and \relion-Class3D\cite{SCHERES2010295}} We illustrate the choices that can be made for inference, through the examples of \relion-Refine3D \cite{Scheres2012RELION} and \relion-Class3D\cite{SCHERES2010295}. \relion-Refine3D\cite{Scheres2012RELION} 
assumes the \acrshort{ctf} to be known, and the volume $V^{(i)}=V$ to be a parameter. Given this image generative model, \relion-Refine3D\cite{Scheres2012RELION} uses a Bayesian approach that consists of (a) modeling the unknown parameter $V$ as a random variable, \textit{i.e.} modeling the Fourier coefficients of the volume $\tilde{V}_j$ as random variables, (b) modeling latent variables in $H_i$ as random variables, \textit{i.e.} assuming that the Fourier poses (describing particles' orientation and position) are random variables, and (c) specifying probability distributions on these random variables, \textit{i.e.} priors in statistical terminology. 
Specifically, \relion-Refine3D\cite{Scheres2012RELION} assumes that the Fourier coefficients $\tilde{V}_{j}$ are sampled from independent Gaussian distributions: $\tilde{V}_{j} \sim N(0, \tau_j^2)$, while the pose latent variables are assumed to be uniformly distributed. The purpose of the inference is to find the parameters of the probability distributions --- \textit{i.e}, for the Gaussian variables $\tilde{V}_{j}$, the means and standard deviations --- that best explain the observed data.
\relion-Class3D\cite{SCHERES2010295} operates similarly, but each image is generated from a set of $K$ volumes, $V_1, ..., V_K$, which are parameters modeled as random variables. 

==> CryoReview 2021 (6)/appB-operators.tex <==

As described in the main text, an alternative (and often simpler) generative model can also be formulated via the Fourier equivalent of Equation~\eqref{eq:image}. 

 \paragraph{Fourier-Slice Theorem.}
In Fourier Space, the convolution $*$ of the projected 2D volume by the PSF conveniently becomes an element-wise matrix multiplication $\odot$ between the 2D Fourier transform of the projected image and that of the PSF. The latter is better known as the Contrast Transfer Function (\acrshort{ctf}), with $\text{CTF}_i = \mathcal{F}(\text{PSF}_i)$, so that:
\begin{equation}\label{eq:fourier}
\tilde{X}_{i} = \text{CTF}_{i} \odot (P_i^{(R_i,t_i)} \circ \tilde{V}^{(i)}) + N_{i}, \qquad \text{with} \quad i=1 \cdots n.
\end{equation}
\noindent Here, $\tilde{X}_{i}$ is the 2D-Fourier transform of the observed image $X_i$ ($\tilde{X}_{i}=\mathcal{F}(X_i)$), and $\tilde{V}^{(i)}$ is the 3D Fourier transform of the molecule (i.e, the volume) $V^{(i)}$, with $\tilde{V}_{i}=\mathcal{F}(V_i)$. In Equation~\eqref{eq:fourier}, the operator $P_i^{(R_i,t_i)}$ first extracts out of $\tilde{V}^{(i)}$ a slice oriented by the rotation $R_i$ and then applies a phase shift in Fourier space accounting for the 2D translation $t_i$.  Finally, $N_{i}$ represents the noise. We note that using the operator $P_i$ circumvents the 3D-to-2D projection step and is therefore more computationally efficient.

%We refer the reader to Section~\ref{sec1-generative_models_and_lvms} and Table~\ref{table:comp_one} for a detailed discussion on the models' complexity.




\paragraph{Efficiency and differentiability of the different generative models} The methods described in this review  (Eq~\ref{eq:image} and \ref{eq:fourier}) leverage the ability to do inference with gradient-based optimization techniques. This requires the generative models to be differentiable --- that is, to allow the differentiation of the loss associated with the output (an image) with respect to the parameters of the model through backpropagation. As explained in Section~\ref{sec1-generative_models_and_lvms}, the volume $V$ (or $\tilde{V}$ in Fourier space) can always be seen as a function from $\mathbb{R}^3$ to $\mathbb{R}$ (or $\mathbb{C}$). The parameters defining this function depend on the choice of \textit{parametrization}, as summarized in Table~\ref{tab:diff}. To make sure that the model is differentiable, we need to ensure that all the operations required in the forward model presented by Equation~\ref{eq:image} are differentiable. Table ~\ref{tab:diff} summarizes the operations required to ``rotate'', ``translate'' and ``project'' the volume $V$ and obtain the observed image. Those operations are:
\begin{itemize}[noitemsep]
    \item multiplication with a matrix $R\in\mathbb{R}^{3\times 3}$,
    \item addition of a vector $\mathbf{t} \in \mathbb{R}^3$,
    \item application of an interpolation kernel,
    \item summation (if the volume is in image space),
    \item and analytical integration.
\end{itemize}
All these operations, if they involve the ``differentiable parameters'' can be differentiated through by backpropagation. As shown in Equation~\eqref{eq:image} (resp. Equation~\eqref{eq:fourier}) the last step of the generative model is the application of the PSF (resp. CTF) which is done with a convolution (resp. element-wise multiplication) with the projected volume. This last operation is also differentiable, which in turn ensures that the whole generative model, transforming a volume $V$ into an image (potentially in Fourier space), is differentiable.

\begin{table}[h]
\centering
\begin{tabular}{c|c|c|c|c|}
\cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}                                                                                     & \textbf{\begin{tabular}[c]{@{}c@{}}Differentiable\\ Parameters\end{tabular}} & \textbf{Domain}                                                                                                          & \textbf{\begin{tabular}[c]{@{}c@{}}Rotation\\ Translation\end{tabular}}                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Projection\\ (in image space)\end{tabular}}                                                                                         \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Voxel\\ Grid\end{tabular}}           & \begin{tabular}[c]{@{}c@{}}$V(x)$\\ for $x\in\{1,\ldots,D\}^3$\end{tabular}    & \begin{tabular}[c]{@{}c@{}}$V: \{1,\ldots,D\}^3$\\ With interpolation kernel,\\ $\hat{V}: \mathbb{R}^3$, see \cite{Ullrich2019}\end{tabular}     &                                                                                                           & \begin{tabular}[c]{@{}c@{}}$\sum_x \hat{V}\hat{(x)}$\\ $\hat{V}:\mathbb{R}^3\rightarrow\mathbb{R}$\end{tabular} \\ \cline{1-3} \cline{5-5} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Neural\\ Network\end{tabular}}       & Weights $W$                                                                    & $V: \mathbb{R}^3$                                                                                                        & \multirow{-2}{*}{$\hat{x}=R^{-1}x-\mathbf{t}$}                                                            & $\sum_x V\hat{(x)}$                                                                                             \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Mixture of\\ Gaussians\end{tabular}} & $A_j$, $c_j$, $\sigma_j$                                                       & \begin{tabular}[c]{@{}c@{}}$V: \mathbb{R}^3$\\ With analytical integration,\\ $\int V(.,z)dz: \mathbb{R}^2$\end{tabular} & \begin{tabular}[c]{@{}c@{}}$c_j\rightarrow\hat{c}_j=Rc_j+\mathbf{t}$\\ $V\rightarrow\hat{V}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\int \hat{V}(y,z)dz$\\ for $y\in\mathbb{R}^2$\end{tabular}                        \\ \hline
\end{tabular}
\caption{Differentiable parameters and operations realized in the generative model, depending of the volume parametrization. $V$ can be equivalently replace with $\tilde{V}$ in Fourier space. Using an interpolation kernel transforms the function $V$ defined on $\{1,\ldots,D\}^3$ into $\hat{V}$ defined on $\mathbb{R}^3$.}
\label{tab:diff}
\end{table}


==> CryoReview 2021 (6)/appC-elbo.tex <==
\renewcommand{\thesubsection}{C.\arabic{subsection}}


This appendix provides more details on the Bayesian formulation of the cryoEM recovery problem, and on the corresponding methods. As a reminder, in the main text, we argue that the lower bounds $\mathcal{L}(q, X, \theta)$ are found by showing that, for any probability distribution $q_i$ on the variables $h_i$, the observed log-likelihood can be written as the sum of two terms:
\begin{align}\label{eq:KL2}
     L(X, \theta)  =  \mathcal{L}(q, X, \theta) + \sum_{i=1}^n \text{KL}(q_i(h_i) \parallel p_{\theta}(h_i|x_i))
     = \sum_{i=1}^n \Big[ \mathcal{L}_i(q_i, x_i, \theta) +  \text{KL}(q_i(h_i) \parallel p_{\theta}(h_i|x_i)) \Big]
\end{align}
where
%  = \int_{z_i} q(z_i) \log\left(\frac{\log p(x_i, z_i| \theta)}{q(z_i)}\right)d_zi\\
%  = \int_{z_i} \log p(x_i, z_i| \theta)q(z_i) dz_i -\int_{z_i} q(z_i)\log q(z_i) dz_i
%  =  \int_{z_i} \log p(x_i, z_i| \theta)q(z_i) dz_i + H(q)
    %  & = \log L(X, \theta) - KL(q \parallel p(z|x, \theta)) \\
    %  &= \int_z \log p(x, z| \theta)q(z|x) dz  + H(q) \\
$KL$ is the \acrfull{kl} defined as $KL(q \parallel p)=\int  q(x) \log \frac{q(x)}{p(x)} dx$, and the terms $\mathcal{L}_i$ write:
\begin{equation}\label{eq:elbo2}
\mathcal{L}_i(q_i,x_i, \theta) 
 =  \int_{h_i} q_i(h_i) \log p_\theta(x_i|h_i) dh_i - \text{KL} \left( q_i(h_i) \parallel p_\theta(h_i) \right). 
%  = \int_{h_i}  q_i(h_i) \log p_\theta(x_i, h_i) dh_i - \int_{h_i}  q_i(h_i) \log q_i(h_i) dh_i.
\end{equation}
The objective of this appendix is to derive these bounds and present the corresponding variational techniques in greater details.

\subsection{A Bayesian take on  cryo-EM}

Before we show these bounds, let us begin by a preliminary remark regarding the model that we are trying to fit. In our formulation in the main text, the parameters $\theta$ are considered as unknown, fixed values. Alternatively, one could also try and incorporate the uncertainty of these parameters by adopting a hierarchical approach, and modelling the parameters $\theta$ as random variables with prior $p(\theta)$. In this case, inference seeks to estimate $\theta$ through the maximum of its posterior distribution $p(\theta | x_1, ..., x_n)$, written in its logarithm form as:
\begin{align}\label{eq:logpost}
\log p(\theta | x_1, ..., x_n) 
\propto \log p(\theta, x_1, ..., x_n)
= \log p_\theta(x_1, ..., x_n) + \log p(\theta)
= L(X, \theta) + \log p(\theta).
\end{align}
This can increase robustness by embedding in the design of the algorithm the inherent variability and uncertainty associated with $\theta$. In fact, following Scheres \cite{Scheres2012RELION}, adding priors on $\theta$ can be viewed as a kind of regularization. Such approaches --- referred to as Maximum a Posteriori (MAP) approaches --- are chosen in Relion-Refine3D and Relion-Class3D\cite{Scheres2012ADetermination}, \cryomaxwelling, and \cryosparc.  In the original RELION\cite{Scheres2012RELION}  method for instance, the underling volume is represented through its Fourier components $V_l$, whose prior is chosen to be zero-mean Gaussian distributedwith unknown variance $\tau_l^2$.

%In this case, the problem of consistency is no longer an issue: the posterior can be shown to be consistent 
We observe that the ML and MAP objectives in Equations~\eqref{eq:loglike}-\eqref{eq:logpost} only differ through the prior term $\log p(\theta)$, while the challenge of the optimization stems froms the intractable term $ L(X, \theta)$. Both approaches traditionally employ the same optimization techniques. 


\subsection{ELBO Computations}

We provide the derivations leading to Equations \eqref{eq:KL2}-\eqref{eq:elbo2} and the definition of the ELBO as a lower bound to the log-likelihood of the generative model. We start by expressing the observed log-likelihood of the model as:
\begin{align*}
    L(X, \theta) 
    &= \sum_{i=1}^n\log p(x_i| \theta) \\
    &= \sum_{i=1}^n \left( \log p(x_i,h_i| \theta) - \log p(x_i,h_i| \theta) + \log p(x_i| \theta) \right)\\
    &= \sum_{i=1}^n\left( \log p(x_i,h_i| \theta) -  \log p(h_i|x_i, \theta) \right) \qquad \text{( Bayes rule:}\quad p(h_i| x_i, \theta) = \frac{p(x_i, h_i|\theta)}{p(x_i|\theta)}) 
\end{align*}
In what follows, we drop the index $i$ and associated sum for convenience. Consider any distribution $q(z)$. If we multiply both sides of the above equation by $q$, and integrate the $z$ out, we get:
\begin{align*}
    \int_{z} L(X, \theta)q(h)dh &= \int_h\left(
            \log p(x,h| \theta) 
                - \log p(h|x, \theta)\right)q(h)dh\\
    \implies   L(X, \theta)&= \int_h\left(
            \log p(x,h| \theta) 
                - \log p(h|x, \theta)\right)q(h)dh,
\end{align*}
since $L(X, \theta)$ does not depend on $h$. Now expanding the right hand side:
\begin{align*}
    L(X, \theta)
    &= \int_h q(h)\log p(x,h| \theta) dh 
        - \int_h q(h) \log p(h|x, \theta) dh  \\
    &= \int_h q(h)\log p(x,h| \theta) dh 
        - \int_h q(h) \log \frac{p(h|x, \theta)q(h)}{q(h)} dh  \\
    &= \int_h q(h) \log p(x,h| \theta) dh  
        - \int_h q(h) \log q(h) dh
        - \int_h q(h) \log \frac{p(h|x,\theta)}{q(h)}dh \\
    &= \int_h q(h) \log p(x,h| \theta) dh  
        - \int_h q(h) \log q(h) dh
        + KL(q(h) \parallel p(h|x,\theta))\\
    &= \mathbb{E}_q[ \log(p_{\theta}(x, h) ] 
        - \int_h q(h) \log q(h) dh
        + KL(q(h) \parallel p(h|x,\theta))  \\ 
    &= \mathbb{E}_q[ \log(p_{\theta}(x, h) ] 
        + H(q) + KL(q(h) \parallel p(h|x,\theta)),
\end{align*}
by introducing the entropy of $q$ as $H(q) = - \int_z q(z) \log q(z)dz$, and writing the KL-divergence between two distributions $p_1$ and $p_2$ as $KL(p_1||p_2) = \int p_1(x) \log ( \frac{p_1(x)}{p_2(x)})dx$.\\

In other words, for any distribution $q$ on the latent variable $H$, the observed marginal likelihood $L(X, \theta)$ is the sum of three terms: (a) the expected log-likelihood, assuming that $h$ has distribution $q$, (b) the Entropy of $q$, which can be understood of the amount of uncertainty in the estimation of $h$ and (c) the KL-divergence between $q$ and the true posterior $ p(h|x, \theta)$, which measures how different these distributions are.\\

Note that, in the previous equations, terms (a) and (b) can be computed, but term (c) --- the KL divergence between the proposed distribution $q$ for $h$ and the actual posterior distribution $p(h|x, \theta)$ is not unknown, because we do not know $p(h|x, \theta)$. However, because the KL-divergence is always non-negative, we know that:
$$ L(X, \theta) \geq   \mathbb{E}_q[ \log(p_{\theta}(x, h) ] + H(q).$$
Thus, introducing the ELBO term $\mathcal{L}(q, X, \theta) = \mathbb{E}_q[ \log(p_{\theta}(x, h) ] + H(q)$, we get:
\begin{equation}\label{eq:ell}
    L(X, \theta)
    = \mathcal{L}(q, X, \theta) 
    + KL(q(h) \parallel p(h|x,\theta)).
\end{equation}
which provides Equation~\eqref{eq:KL2} and the right hand side of Equation~\eqref{eq:elbo2}. Developping the ELBO term gives:
\begin{align*}
    \mathcal{L}(q, X, \theta)
    &=  \int_h q(h) \log p(x,h| \theta) dh  
        - \int_h q(h) \log q(h) dh \\
    &=  \int_h q(h) \log p(x| h, \theta) dh  
        +  \int_h q(h) \log p(h| \theta) dh  
        - \int_h q(h) \log q(h) dh  \\
    &=  \int_h q(h) \log p(x| h, \theta) dh  
        - KL(q(h) \parallel p(h|\theta),
\end{align*}
which gives the left side of Equation~\eqref{eq:elbo2}.

\subsection{Expectation-maximization (EM) Algorithm}\label{subsec:em}

Historically, inference in latent variable models has been achieved through the Expectation-maximization (EM) algorithm \cite{Dempster1977MaximumAlgorithm}. The EM algorithm is often introduced as a data imputation technique (see following subsection), but it can also be understood as a dual ascent algorithm --- a perspective that allows unifying most cryoEM inference methods and that we present here.

\paragraph{EM as a Dual Ascent Algorithm} The EM algorithm can be seen as a dual ascent procedure, \textit{i.e.} as a maximization-maximization procedure, that leverages Equation~\eqref{eq:KL2} rewritten as: $\mathcal{L}(q, X, \theta) = L(X, \theta)  -  \sum_{i=1}^n \text{KL}(q_i(h_i) \parallel p_\theta(h_i|x_i))$. Starting with an initial guess $\theta^{(0)}$ of the parameter, the EM algorithm performs two steps at each iteration $t$:
  \begin{description}[noitemsep]
  \item[(a) Inference on hidden variables (E-step)] Given the current $\theta^{(t-1)}$, maximize each term $\mathcal{L}_i(q_i, \theta^{(t-1)}) = L_i(X_i,  \theta^{(t-1)})  - KL(q_i(h_i) || p_{ \theta^{(t-1)}}(h_i,x_i))$ (by Equation \ref{eq:ell}) with respect to the distribution $q_i$ defined on the hidden variables $h_i$. Since $\theta^{(t-1)}$ is fixed, the best choice of $q$ is the one that minimizes the KL term $KL(q_i(h_i) || p_{ \theta^{(t-1)}}(h_i,x_i))$:
  \begin{equation}
       \text{For each $i = 1, ..., n$:} \quad\quad q_i^{(t)}(h_i) = \argmax_q \mathcal{L}_i(q, X, \theta^{(t-1)})= \argmin_q KL(q_i(h_i) || p_{ \theta^{(t-1)}}(h_i,x_i))  = p_{\theta^{(t-1)}}(h_i| x_i).
  \end{equation}
  
  This choice $q_i^{(t)}(h_i)=p_{\theta^{(t-1)}}(h_i| x_i)$ corresponds to the green distribution in Figure~\ref{fig:posterior_distributions} and makes the lower bound $\mathcal{L}$ tangent to $L$ at $\theta^{(t-1)}$ in Figure~\ref{fig:lb} (left).
%   which yields: $L(X, \theta^{(t-1)}) \leq \mathcal{L}(q^{(t)}, \theta^{(t-1)})$.
  
 %This step is typically easy. Note that 
 % $\log(L(X, \theta^{(t)})$ does not depend on $\theta$. Thus, maximizing the energy $\mathcal{L}(q, \theta^{(t)})$  with respect to $q$ is equivalent to minimizing the KL divergence $KL(q||p(z|x, \theta^{(t)})$. This is achieved when $q=p(z|x, \theta^{(t)}$.
  %In expectation maximization, we simply take $q$ to be $p(z|x, \theta^{(t)})$, where $\theta^{(t)}$ are the parameters at the $j^{th}$ iteration.  This yields an
%In the case of cryo-EM, there is no default closed form that exists for the posterior and the posterior needs to be sampled from using a Monte-Carlo technique. Alternatively, when the latent variables are modeled as unknown deterministic values, the goal is to estimate them. In this case, this is achieved by solving a minimization problem for each $i$. Due to the volume of data, this is the method chosen in pratice within the EM algorithms.
    \item[(b) Maximization on the model's parameters (M-step)] Given the current $q^{(t)} = \{q_1^{(t)}, ..., q_n^{(t)}\}$, maximize $\mathcal{L}(q^{(t)}, X, \theta)$ with respect to the model parameters $\theta$:
    \begin{equation}
        \theta^{(t)} = \argmax_{\theta} \mathcal{L}(q^{(t)}, X, \theta) = \argmax _{\theta} \sum_{i=1}^n \mathcal{L}_i(q_i^{(t)}, X, \theta).
    \end{equation} %Depending on whether we consider the parameters to be deterministic values or random variables, the EM solves for the maximum likelihood or for the maximum a posteriori estimators.
    % which ensures:
    %   $ \mathcal{L}(q^{(t)}, \theta^{(t-1)}) \leq \mathcal{L}(q^{(t)}, \theta^{(t)}) $.
    The argument maximum of $\mathcal{L}$ is used to update $\theta^{(t-1)}$ to $\theta^{(t)}$ in Figure~\ref{fig:lb} (left).
  \end{description}
These steps are iterated until convergence in $\theta$. In other words, one first finds the "best" lower bound to $L(X, \theta)$ given $\theta^{(t)}$ by choosing the one that is tangent to $L(X, \theta)$ at $\theta^{(t)}$. Once this bound has been established, we subsequently maximize this bound with respect to the parameter $\theta$.
%This view of the EM algorithm links it with the inference methods described later in this section. 
% We note, first, that the prior $\log p(\theta)$ can be added in the M-step, if one wishes to perform MAP estimation as opposed to MLE estimation. 
We note that to alleviate potential computational bottleneck in the  M step (respectively $\mathcal{L}(q^{(t)}, X, \theta)$), the closed form solution can be replaced by simply taking a gradient step. This gives rise to ``gradient EM" methods, which we will refer to later, as all methods introduced in the next subsections can be formulated as ``gradient" methods too.
 

 
\paragraph{Computational Bottleneck: E-step.} One of the issues with the EM algorithm relies in the computation of  the posterior of the latent variable $h_i$ given $x_i$ and current estimate $\theta^{(t-1)}$:
\begin{equation}\label{eq:post}
p_{\theta^{(t-1)}}(h_i|x_i)  = \frac{p_{\theta^{(t-1)}}(x_i|h_i)p(h_i)}{p_{\theta^{(t-1)}}(x_i)} = \frac{p_{\theta^{(t-1)}}(x_i|h_i)p(h_i)}{\int_{h_i} p_{\theta^{(t-1)}}(x_i, h_i) dh_i}.
\end{equation}

Unless the posterior can be computed efficiently, this computation can be lengthy. In fact, unless the priors of the different variables are specified using conjugacy --- which would constrain the choice of prior distributions that we could consider ---, it is difficult to get closed-form updates for the posterior. Alternatively, one can evaluate $p_{\theta^{(t-1)}}(h_i|x_i)$ for each $h_i$ discretized on a grid by computing the integral in Equation~\eqref{eq:post} via a Riemann sum as in \relion or via Importance Sampling as in \cryosparc. \relion and \cryosparc use the EM algorithm with MAP estimation of $\theta$, as opposed to ML estimation. 

This discretization remains however a computationally intensive approach. Consequently, despite many advances leveraging GPU computing, the integral in Equation~\eqref{eq:post} represents the main computational bottleneck in cryo-EM reconstruction methods, and the main reason we might want to look for other, more efficient alternatives. 
%The E-step of the EM algorithm still represents a major bottleneck, despite many advances leveraging GPU computing.

% \paragraph{EM in \relion and \cryosparc} The computation of the posterior could be achieved by using a closed form for the expression of the probability $p(h_i|x_i, \theta^{(t-1)})$ . In cryo-EM generative models, however, such a closed form is not necessarily possible. Alternatively, one can evaluate $p_{\theta^{(t-1)}}(h_i|x_i)$ for each $h_i$ discretized on a grid by computing the integral in Equation~\eqref{eq:post} via a Riemann sum as in \relion or via Importance Sampling as in \cryosparc. \relion and \cryosparc use the EM algorithm with MAP estimation of $\theta$, as opposed to ML estimation. Additionally, \cryosparc uses stochastic gradient descent for the maximizations in the M-step, at each iteration $t$.\\




\begin{figure}
 \vspace*{-0.3in}
 \centering
    \includegraphics[width=0.4\textwidth]{figs/posterior_distributions.pdf}
    %  \setlength{\belowcaptionskip}{-4pt} 
    %   \setlength{\abovecaptionskip}{-4pt} 
    \caption{Possible choices for the distribution $q$ on the hidden variables $h$, where we have dropped the indices $i$ for convenience of notations. The choice of $q$ determines the lower bounds to $L(X, \theta)$ in Figure~\ref{fig:lb}. The inference methods used in cryoEM reconstruction can be contrasted by the choice of $q$: as the true posterior $p_\theta(h|x)$ represented by the green line, as the Dirac distribution $\delta(h)$ represented by the vertical dashed gray line or as a distribution within a known parameterized family $\mathcal{Q}$, such as the family of Gaussian distributions, represented by the brown dashed line.}
    \label{fig:posterior_distributions}  \vspace*{-0.18in}
\end{figure}

 
 
%  \subsection{EM as a Data Imputation Technique}

% The EM algorithm is often presented as a data imputation technique. Indeed, recall that in Equation~\eqref{eq:loglike}, it would be easier to maximize the full log-likelihood $p_{\theta}(x_i, h_i)$ than the observed log-likelihood $L(X, \theta) = \log p_\theta(x_i)$, if only we knew the hidden variables $h_i$. The trick proposed by the EM is to "impute" (or fill in) the missing $h_i$ values. To this end, instead of considering $L(X, \theta)$, we start with the "expected" log-likehood with respect to any distribution $q$, defined as:
% $$ \mathbb{E}_{q_i}[ \log p_{\theta}(x_i, h_i) ] = \int_{h_i} \log p_{\theta}(x_i, h_i)  q_i(h_i) dh_i.$$
% In contrast to Equation~\eqref{eq:loglike}, the $\log$ is now inside the integral, similarly to the second formulation of the ELBO in Equation~\eqref{eq:elbo2}. We simply have to find an appropriate distribution for $q_i$, for which we choose to be the posterior $q_i^{(t+1)} = p_{\theta^{(t)}}(h_i|x_i)$ given parameters computed in the current iteration $t$, as motivated by the tangent lower bounds described above.
% %The candidate distribution here will be within the family of distributions $\mathcal{Q} = \{ p_{\tilde{\theta}}(h_i|x), ~\tilde \theta \}$. Since by design, $\theta^{(t)}$ is the best $\theta$ in that family that maximizes $\mathcal{L}(X, \theta)$, at each iteration $t+1$, we take $q^{(t+1)} = p_{\theta^{(t)}}(h|x)$ the marginal distribution of $h$ given parameters computed in the previous step. This allows us to compute the expectation. 
% This can be considered an imputation step, since, for each value of $h$, we are filling in the $h$ in the term $\log p_{\theta}(x, h)$ while associating with the corresponding this complete log-likelihood  value with a different weight depending on $p_{\theta^{(t)}}(h| x)$. We get: $Q_i(\theta, \theta^{(t)}) = \int_{h_i} p_{\theta}(x_i , h_i) p_{\theta^{(t)}}(h_i|x_i) dh_i,$
% with $\theta^{(t)}$ the current estimate of the true $\theta$ at iteration $t$, and $Q(\theta, \theta^{(t)}) = \sum_{i=1}^n Q_i(\theta, \theta^{(t)})$. 
% In this view, the EM algorithm starts with an initial guess $\theta^{(0)}$ of the parameter $\theta$ and performs two steps at each iteration $t$: 
%   \begin{description}
%   \item[(a) Expectation step (E-step)]: Given the current estimate $\theta^{(t-1)}$ of $\theta$, we compute the expectation defining function $Q_i$: 
%   \begin{equation}
%   \text{For each $i = 1, ..., n$:} \quad\quad
%       Q_i(\theta, \theta^{(t-1)}) 
%     %   = \mathbb{E}_{p_{\theta^{(t-1)}}(h_i|x_i )}[p_\theta(x_i, h_i)]
%       = \int_{h_i} p_\theta(x_i, h_i) p_{\theta^{(t-1)}}(h_i|x_i) dh_i.
%   \end{equation}
%   \item[(b) Maximization step (M-step)]: Optimize $Q(\theta, \theta^{(t-1)})$ over $\theta$ to update the current estimate $\theta^{(t-1)}$ into $\theta^{(t)}$.
%   \begin{equation}
%      \theta^{(t)} = \argmax_{\theta} Q(\theta, \theta^{(t-1)}) 
%   \end{equation}
%   \end{description}

% These steps are iterated until convergence of $\theta^{(t)}$. In this setting, the tangent lower bound $\mathcal{L}_i$ which is used as a proxy for $L(X, \theta)$ in the optimization over $\theta$  becomes the expected value $\mathcal{Q}_i$ of the complete log-likelihood $p_\theta(x_i, h_i)$
% % %, using as our best approximation of $p(h_i|\theta)$ the function $p(h_i|\theta^{(t)})$, 
% used as the proxy for $L(X, \theta)$ in the M-step. In fact,  $\mathcal{L}_i$ and $\mathcal{Q}_i$ only differ by the Entropy term $\int_{h_i}q_i(h_i)\log q_i(h_i) dh_i$ in Equation~\eqref{eq:elbo2}, \textit{i.e.} a term that is independent of $\theta$.








\subsection{Variations on the EM algorithm}\label{subsec:variations_EM}

We present details on the variations on the EM algorithm discussed in the main text.

\subsubsection{Modal EM algorithm}\label{subsec:mem}

The computational bottleneck observed in the EM algorithm has also motivated the use of approximations in the E-step. The modal approximation of EM amounts to finding a proxy for the posterior $p_{\theta^{(t-1)}}(h_i|x_i)$ in the E-step. This approximation replaces the posterior by its "mode" $\hat{h}_i = \argmax_h p_{\theta^{(t-1)}}(h|x_i)$, i.e. the most probable $\hat h_i$ for each image $x_i$. 
%This is illustrated in the second column of Table~\ref{tab:inference}.

\paragraph{Modal EM: The algorithm.} The E-step of the EM algorithm is replaced by its modal approximation, but the M-step is largely unchanged:
\begin{description}
  \item[(a) Inference on hidden variables $h_i$] Given current $\theta^{(t)}$, compute the modes:
  \begin{equation}
  \text{For each $i = 1, ..., n$:} \quad\quad
  \hat{h}_i^{(t)} = \argmax_h p_{\theta^{(t-1)}}(h|x_i) = \argmax_h p_{\theta^{(t-1)}}(x_i|h)p(h).
  \end{equation}
  
  This amounts to approximating the solution of the E step (which, we've shown, is the posterior of $h$ given $X$ and $\theta^{(t-1)}$) by  $q_i^{(t)}(h_i)=\delta (\hat h_i^{(t)})$, the Dirac distribution at $\hat h_i^{(t)}$, represented in gray in Figure~\ref{fig:posterior_distributions}. This choice for $q_i^{(t)}(h_i)$ creates a lower bound $\mathcal{L}$ that may not be tangent to $L$ in Figure~\ref{fig:lb} (right). Since this approximation does not require us to compute complicated posteriors, it is a simpler, but looser ELBO to the observed likelihood.
  \item[(b) Maximization on model's parameter $\theta$] The parameter $\theta$ is updated via:
  \begin{equation}\label{eq:modal-m}
      \theta^{(t)} = \argmax_\theta \sum_{i=1}^n \mathcal{L}(\delta (\hat h_i^{(t)}), \theta) =  \argmax_\theta \sum_{i=1}^n p_{\theta}(x_i, \hat h_i^{(t)}).
  \end{equation}
  The argument maximum of $\mathcal{L}$ is used to updated $\theta^{(t-1)}$ to $\theta^{(t)}$ in Figure~\ref{fig:lb} (right), just as in the EM algorithm in Figure~\ref{fig:lb} (left).
 \end{description}
%  where  and we highlight the imputation of the hidden variable $h_i$ by the value $\hat h_i$ which allows us to maximize the full likelihood in Step (b).
 
% We note that the computation of the modes in Step (a) do not require the evaluation of the integral defining the posteriors $p_{\theta^{(t-1)}}(h|x_i)$ in Equation~\eqref{eq:post}, as this integral does not depend on $h$. 

% We note again that the prior $\log p(\theta)$ can be added in the M-step, if one wishes to perform MAP estimation as opposed to MLE estimation, and that we can build a gradient Modal EM algorithm by only performing gradient steps in (a) and (b).
 
 
\paragraph{Modal EM in \relion, \cryosparc, \threedflex, \cryodrgn, \cryofold} The EM algorithm with modal approximation is used in cryo-EM in \cryosparc, \threedflex, \cryodrgn and \cryofold to infer the latent variable associated with the rotation $R_i$. In other words, they estimate the best rotation $\hat R_i$ for each input image $i$, relying on a branch-and-bound optimization algorithm to address this maximization. This approach is also used in \relion to estimate the best noise variance $\hat \sigma_i$ that is associated with each image $i$.


\subsubsection{Variational EM algorithm}\label{subsec:vem}



The modal approximation in the EM algorithm speeds up the E-step; yet it has the drawback of summarizing the whole posterior distribution $p_{\theta^{(t)}}(h_i|x_i)$ by a single estimate $\hat h_i$, reducing accuracy and leading to non-tangent lower bounds $\mathcal{L}$. \acrfull{vi}, also known as Variational Bayes, has appeared in cryo-EM as a compromise between the guarantees of the EM and the efficiency of modal EM during the computation of the E-step. 

\acrfull{vi} replaces the evaluation of the posterior of the latent variables $p_{\theta^{(t-1)}}(h_i|x_i)$, by an optimizing over a different family of candidate distributions $\mathcal{Q}$, called the ``variational family''. $\mathcal{Q}$ is typically a family with a restricted form, so that the updates are easier to perform: for instance, if there is a complex dependency structure between entries in our parameter $\theta$, we might select $\mathcal{Q}$ to be a family of posteriors where the entries are independent, so that the updates are simpler to perform: this is usually the `mean field' approximation to the posterior of $\theta$. The $q$ that is chosen in Equation \ref{eq:elbo2} is the "closest" to the posterior, where ``closest" is defined in terms of the KL divergence (see Equation~\eqref{eq:vi} below). 

%This is illustrated in the third column of Table~\ref{tab:inference}.

%As for the EM algorithm, the foundation behind this approach is the definition of the observed likelihood as the sum of two terms:
%$ \log L(X, \theta) = \mathcal{L}(q, \theta) + KL(q||p(Z|\theta, X)).$
% However, VI does not perform an ascent on $q$ in  $\mathcal{L}(q, \theta) $ to find the "best values of the latent variables given the current parameters", i.e. does not compute the posterior $p(Z | \theta, X )$. Instead, in a step equivalent to the E-step, 

The variational family $\mathcal{Q} = \{ q_\eta | \eta\}$ with parameters $\eta$ is typically chosen to be a family of Gaussian distributions, in which case $\eta$ represents the mean and variance, i.e. $\mathcal{Q} = \{ q_\eta = N(\mu, \sigma) | \eta=(\mu, \sigma)\}$. Other approaches consider the variational family of Gaussian distributions with fixed isotropic variance $\sigma_0$, i.e. $\mathcal{Q} = \{q_\eta = \mathcal{N}(\eta, \sigma_0) | \eta\}$.  In  modal EM, the parametric family can be seen as a family of Dirac distributions, as in Equation~\eqref{eq:modal-m}.
%Yet, we will see that we can unify approaches through variational inference by considering that some methods use a variational family of dirac distributions $\mathcal{Q} = \{q_\eta = \delta_\eta | \eta\}$, parametrized by the value $\eta$ at which the dirac stands. In this case, variational inference boils down to the estimation of each $h_i = \eta_i$ as in the E-step where the $h_i$ are considered deterministic values. 


%Generally, we denote $\eta$ the parameters parametrizing the probability distributions within $\mathcal{Q}$.
%In this case, typically, $z$ looses its interpretability as a latent variable. The information from the latent variables becomes implicitly encoded as a variable $\tilde{z}$. In this case, $\tilde{z}$ can be considered as one of the instances of "implicit" parametrizations of the problem: it is a proxy variable for all latent variables and parameters of the distribution.

\paragraph{Variational EM as a Dual Ascent Algorithm} The E-step of the EM algorithm is replaced by VI and the M-step is unchanged. The VI framework thus gives rise to a variational EM which performs the following two steps at each iteration $t$:
\begin{description}
  \item[(a) Inference on hidden variables $h_i$] The $n$ parameters $\eta_i$ corresponding to each $q_i$ are computed via:
  \begin{equation}\label{eq:vi}
      \text{For each $i = 1, ..., n$:} \quad\quad \eta_i^{(t)} = \argmin_\eta KL(q_{\eta}||p_{\theta^{(t-1)}}(h_i|x_i)
  \end{equation}
  This choice for $q$ is represented in brown in Figure~\ref{fig:posterior_distributions}. Similarly to the Modal EM, this creates a lower bound $\mathcal{L}$ that may not be tangent to $L$ in Figure~\ref{fig:lb} (right).
  \item[(b) Maximization on model's parameter $\theta$] The parameter $\theta$ is updated via:
  \begin{equation}
      \theta^{(t)} = \argmax_\theta \sum_{i=1}^n \mathcal{L}_i(q_{\eta_i}^{(t)}, \theta).
  \end{equation}
    The argument maximum of $\mathcal{L}$ is used to updated $\theta^{(t-1)}$ to $\theta^{(t)}$ in Figure~\ref{fig:lb} (right), just as in the EM and the Modal EM algorithms.
 \end{description}



Thus, the Variational Inference approximation in the E-step replaces the samplings in evaluation of the true posterior, required to compute the integral in Equation~\eqref{eq:post}, by an optimization on the fewer parameters $\eta_i$ parametrizing each approximate posterior $q_{\eta_i}$. This optimization can be efficiently conducted with (stochastic) gradient descent. In this sense, it also represents a solution to the computational bottleneck of the E-step.



\paragraph{Variational EM in \threedflex and \cryomaxwelling} Variational gradient EM is used in \threedflex to infer the rotation variable $R_i$, using the variational family of Gaussian distributions with fixed isotropic variance $\sigma_0$.% The authors called this approach an ``auto-decoder" architecture. 
Variational EM is also used in \cryomaxwelling in the context of homogeneous reconstruction. Here, VI happens both in Step (a), to estimate the approximate posterior of the rotation $R_i$, and in Step (b) to also estimate the approximate posterior of the volume $V$, which is a parameter included in $\theta$. The approximate posterior of $V$ provides an approximate measure of uncertainty on the homogeneous reconstruction.

%. As per Punjani et al\cite{Punjani2021}, auto-decoders are a useful tool, as they allow ``precise inference", as opposed to the amortized inference that we will introduce in the next subsection.  The inference is led independently for each image, as an optimization on $q_i$ is performed for each image $i$ in step (a). In fact, the authors of 3DFlex --- which mainly focuses on estimating heterogeneity in volumes --- argue that this independence was key in yielding high-resolution structures.

\paragraph{Amortized Variational EM as Dual Optimization Algorithm} Amortized Inference in the E-step of variational EM leads to an amortized variational EM. In this case, the algorithm can be written as:
\begin{description}
  \item[(a) Inference on hidden variables $h_i$] The parameters $\xi$ parametrizing the encoder is computed via:
  \begin{equation}
      \xi^{(t)} = \argmax_\xi \sum_{i=1}^n KL(q_{\text{Enc}_\xi(x_i)}||p_{\theta^{(t-1)}}(h_i|x_i)
  \end{equation}
  which generates $n$ distributions $q_{\eta_i}^{(t)}$ parametrized by $\eta_i = \text{Enc}_{\xi^{(t)}}(x_i)$.
  \item[(b) Maximization on model's parameter $\theta$] The parameter $\theta$ is updated via:
  \begin{equation}
      \theta^{(t)} = \argmax_\theta \mathcal{L}(q_{\eta_i}^{(t)}, \theta).
  \end{equation}
 \end{description}

This method has the advantage of further improving  the flexibility and efficiency of the Variational EM algorithm, by allowing the updates to be even more efficient by parametrizing the $q_i$ as a function of the input $x_i$. 

\subsection{Generative Adversarial Networks}\label{subsec:gans}

Cryo-EM reconstruction methods from Subsections~\ref{subsec:mem}-\ref{subsec:vem} have naturally explored adaptations of the computationally expensive E-step from the EM algorithm of Subsection~\ref{subsec:em}. As a result, they differ in their inference on the hidden variables of the generative model. Yet, the only hidden variable of interest is the conformation variable and associated molecular volumes. As a result, recent works have explored methods that avoid the inference on the ``nuisance" latent variables altogether. This is the approach taken by \acrfull{gan}.

\paragraph{Generative Adversarial Networks as Minimax Games} A generative adversarial model (GAN)\cite{Goodfellow2014GenerativeNets} is a method that estimates the parameters of a generative model, such as the one in Equation~\eqref{eq:image}, through an adversarial process. The GAN trains a ``generator" to produce images $x_i$ that best capture the training data distribution, while a discriminator estimates the probability that a given image $x_i$ came from the training data rather than the generator.

In other words, the generator and discriminator play the following two-player minimax game with value function $V$:
\begin{align*}
    V = \min_\theta \max_\phi 
    \mathbb{E}_{x \sim p_{\text{data}}(x)}\left[ 
            \log \text{Dis}_\phi(x)\right] 
    + \mathbb{E}_{h \sim p(h)} \left[
        \log \left(1 - \text{Dis}_\phi (f_{V_\theta}(h))\right) \right],
\end{align*}
where the generator is the cryo-EM generative model defined in Equation~\eqref{eq:image} and the discriminator has weights $\phi$ and is denoted by $\text{Dis}_\phi$. In this equation, $p_{\text{data}}(x)$ represents the probability distribution of the images, and $p(h)$ is a prior distribution on the hidden variables. The GAN training iterates two steps:
\begin{description}
 \item[(a) Discriminator - Update of parameters $\phi$], according to the gradient step:
    \begin{equation}
        \phi^{(t+1)} = \phi^{(t)} + \nabla_\phi
                \frac{1}{n}\sum_{i=1}^n \Big[ 
                \log \text{Dis}_\phi(x_i) + \log \left(1 - \text{Dis}_\phi (f_{V_\theta^{(t)}}(h_i))\right)
                \Big],
    \end{equation}  
 \item[(b) Generator - Estimation of model's parameter $\theta$], according to the gradient step:
     \begin{equation}
        \theta^{(t+1)} = \theta^{(t)} - \nabla_\theta
                \frac{1}{n}\sum_{i=1}^n \Big[ 
                \log \left(1 - \text{Dis}_{\phi^{(t)}} (f_{V_\theta}(h_i))\right)
                \Big],
    \end{equation}  
\end{description}
where in each Step (a) or (b), the "hidden variables" $h_i$ are sampled according to a prior distribution $p_h$. Even though a GAN iterates two steps, including one step related to the estimation of the model's parameters, its framework differ from the variations of the EM algorithm in the sense that the hidden variables are not inferred: it is enough to be able to randomly sample from them from some prior distribution.

\paragraph{GANs in \cryogan and \multicryogan} \cryogan uses a GAN to perform homogeneous reconstruction of molecular volumes, while using uniform sampling on the rotation, translation and CTF hidden variables. \multicryogan introduces heterogeneous reconstruction with this approach. Both \cryogan and \multicryogan use the Wasserstein variant \cite{wgan2017} of the traditional GANs.

% In other words:
% \begin{equation}
%     \hat \theta 
%     = \argmin_\theta \mathcal{D}\left(p_\theta(x), p_{\text{data}}(x) \right)
%     = \argmin_\theta \mathcal{D}\left(
%         p_\theta(x), p_{\theta_{\text{true}}}(x) \right)
% \end{equation}


==> CryoReview 2021 (6)/appD-AEs.tex <==
\setcounter{subsection}{0}
\renewcommand{\thesubsection}{D.\arabic{subsection}}

Autoencoders (AEs) and variational autoencoders (VAEs) are the main realizations of the amortized variational inference approaches in the cryo-EM reconstruction literature. This appendix provides additional details to link the traditional presentations of the AEs and VAEs to the framework described in Section~\ref{sec2-inference}.
 
\subsection{Autoencoders}

An autoencoder traditionally aims to minimize the following loss function:
\begin{equation}
     \ell (\theta, \xi)
     = \sum_{i=1}^n  ||x_i -  \hat{x_i} ||^2 
     = \sum_{i=1}^n  ||x_i -  f_{V_\theta}(h_i)  ||^2 
     = \sum_{i=1}^n  ||x_i -  f_{V_\theta}(\text{Enc}_{\xi}(x_i) ||^2,
\end{equation}
where $f_{V_\theta}$ denotes here the output of the generative model (such as the one in Equation~\ref{eq:image}) and is usually called a reconstruction: $\hat x_i = f_{V_\theta}(h_i)$, while $\ell (\theta, \xi)$ is called the reconstruction loss. Note that the mean square error is used to quantify the reconstruction loss, but it can be replaced by other metrics. For example, the binary-cross entropy is a metric traditionally used to compare images $x_i$ and $\hat x_i$. In this context, the goal is to perform the double minization in $\theta$ and $\xi$ such that: 
\begin{equation}
  \hat \theta, \hat \xi = \argmin_{\theta, \xi} \ell(\theta, \xi). 
\end{equation}

By considering the decoder as latent variable model: $\hat x_i = f_{V_\theta}(h_i) + \epsilon_i$ with $\epsilon_i$ a standard Gaussian noise, this loss corresponds to the negative log-likelihood, informed by the encoder. 

%We observed that this loss can also be seen as the negative ELBO where the KL divergence gives rise to ...TODO... due to the variational family of dirac distribution considered.



To minimize this objective, the AE takes a gradient step at each iteration $t$, or backward pass through the network, such that:
% Latent space models constitute a large family of pipelines that all have in common the notion of a latent variable $z$. Within this family, depending on the variational family assumed for the latent variable $z$ these algorithms can be further brocken down into 2 categories:
\begin{description}
\item[(a) Encoder - Inference on latent variables $h_i$] The encoder updates its weight $\xi$ through a gradient step with learning rate $\alpha$:
\begin{equation}
    \xi^{(t)} = \xi^{(t-1)} - \alpha \nabla_\xi \ell(\theta, \xi).
\end{equation}
\item[(b) Decoder - Estimation of model's parameter $\theta$] The decoder updates its weight $\theta$ through a gradient step with learning rate $\alpha$:
\begin{equation}
    \theta^{(t)} = \theta^{(t-1)} - \alpha \nabla_\theta \ell(\theta, \xi).
\end{equation}
\end{description}
We note that this gradient descent is usually performed via stochastic gradient descent, such that only a mini-batch of the data is considered at each iteration to compute $\ell$, as opposed to the full dataset of $n$ images.
% \item[1. Auto-Encoders.] In this setting, the loss is simply a reconstruction loss, ie. a simple Mean Squared Error. This is the approach chosen for instance by 3D-Flex.
% In this case, the loss can simply be written as:

% $$$$
%  Note that there is a high amount of flexibility in the decoder. In 3D-Flex for instance,  the decoder is adapted to fit the parametrization and constraints injected in problem, so that the first step of the decoder links the representation $z$ to the volume through the operation $ D(f_{\theta}(x_i), V))$ where $D$ is a convection operator and V is a canonical 3D density map. The second part is more standard and corresponds to the forward/generative step, and the outputted volume $\hat{V}$ at the end of the first step is fed into the generative model: $CTF_i \Pi^{2D}_{\phi}(\hat{V})$, so that: $\mathcal{D}ec_{\theta} (z)  = CTF_i \Pi^{2D}_{\phi}( D(f_{\theta}(x_i), V)))$.

\subsection{Variational Autoencoders}

A variational autoencoder traditionally aims to minimize the following loss function, which is the negative ELBO \cite{Kingma2014Auto-EncodingBayes}:
\begin{equation}
    \mathcal{L}(\xi, \theta)  
    = \sum_{i=1}^n \mathbb{E}_{q_{\xi} (h_i|X_i))} (\log(p_\theta(X_i|z)) + KL ( q_{\xi}(h_i|X_i) || p(h_i)).
\end{equation}
In this loss, the first term is called the reconstruction term, estimated with one Monte Carlo sample through the so-called ``reparametrization trick", and is akin to the reconstruction loss of the AE. The second term is a KL divergence term that is called the regularization term, as it regularizes the posterior of the latent variable $h_i$ by forcing it to be close to the prior $p(h_i)$ of $h_i$ which is modeled by a standard Gaussian distribution.

We can rewrite this loss by using the functions $\text{Enc}_\xi$ and $\text{Dec}_\theta$, and assuming that the Monte Carlo sampling performed to compute the expectation happens by sampling a unique $\tilde h_i$ through $q_{\xi} (h_i|X_i)$ which is the convention adopted in these architectures:
\begin{equation}
    \mathcal{L}(\xi, \theta)  
    = \sum_{i=1}^n ||x_i - \hat{x_i} ||^2  - KL ( q_{\xi}(h_i|x_i) \parallel p(h_i)) \\
    = \sum_{i=1}^n ||x_i - \text{Dec}_{\theta}(\text{Enc}_{\xi}(x_i)||^2  - KL ( q_{\text{Enc}_\xi}(h_i|x_i) \parallel p(h_i)), \\
\end{equation}
where the KL term has a closed form in terms of the output of the encoder, due to the fact that the $q$ distribution belongs to a Gaussian family of diagonal covariance.

By realizing that the decoder only participates in the first term of the loss function, the VAE takes a gradient step at each iteration $t$, or backward pass through the network, such that:
\begin{description}
\item[(a) Encoder - Inference on latent variables $h_i$] The encoder updates its weight $\xi$ through a gradient step of learning rate $\alpha$ such that:
\begin{equation}
     \xi^{(t)} = \xi^{(t-1)} - \alpha \nabla_\xi \mathcal{L}(\xi, \theta) .
\end{equation}
\item[(b) Decoder - Estimation of model's parameter $\theta$] The decoder updates its weight $\theta$ through a gradient step with learning rate $\alpha$:
\begin{equation}
    \theta^{(t)} 
    = \theta^{(t-1)} - \alpha \nabla_\theta \mathcal{L}(\xi, \theta) 
    = \theta^{(t-1)} - \alpha \nabla_\theta \ell(\theta, \xi).
\end{equation}
 \end{description}
  
%   In this case, the whole pipeline also has to be adapted to deal with the variability of the latent space, and the reconstructed image is modeled as:
% \begin{equation}\label{eq:model}
%  \forall i=1...n, \qquad   \hat{x}_i = \mathcal{D}_{w}(h_i) + \epsilon_i \qquad \text{where: } h_i \sim N(0, \mathbb{I}_L), \text{ and } \epsilon_i \sim N(0, \Psi).
%  \end{equation}

The main difference with the autoencoder is that the latent variable $h_i$ is considered as a random variable, rather than a fixed deterministic value. That is, $h_i$ is endowed with a parametric probability distribution represented by $q$ --- which is a Gaussian distribution with parameters output by the encoder, so that  $h_i \sim N(\mu_{\xi}(X_i),\sigma^2_{\xi}(X_i))$ and $\text{Enc}_\xi(X_i) = (\mu_xi(X_i), \sigma^2_\xi(X_i)$. Considering $h_i$s as random variables has been shown to lead superior reconstruction results over the autoencoder.

% The problem of inferring the distribution of $z$ simply boils down to fitting the mean $\mu_{\phi}(x_i)$ and variance $\sigma^2_{\phi}(x_i)$. The encoder is thus a neural network with two outputs per coefficient of the hidden variable
%   $\text{Enc}_\xi(x_i) = \left( \mu_\xi(x_i) , \log \sigma_\xi^2(x_i) \right)$. 

The VAE loss can be adapted as: $\mathcal{L}(\xi, \theta)  = \sum_{i=1}^n \mathbb{E}_{q_{\xi} (z|X_i))} (\log(p(X_i|z)) + \beta KL ( q_{\xi}(X_i|Z || p(x))$, where $\beta$ is an additional hyperparameter introduced in $\beta$-VAE\cite{Thiagarajan2017-VAE:Framework}. Traditional VAEs have $\beta=1$, to ensure that the actual negative ELBO is minimized. Yet, to prevent pathological issues in the fitting of VAEs (including posterior collapse), recent work has shown that counterbalancing the reconstruction error with the KL divergence through a $\beta$ could yield superior results.

In the cryo-EM implementations of the VAE architectures, the ELBO loss can be supplemented with additional terms that we name ``structure losses" for now. We will explain it in the next appendix as it depends on the structure of the decoder (i.e. exact choice of generative model) chosen by the method.

In practive, \cryoposenet, \cryoai and \egmm use an autoencoder, and \egmm additionally implements an variational autoencoder with a variational family of Gaussian distributions with fixed isotropic variance $\sigma_0$. The AE architecture is used in \cryoposenet with a traditional L2 reconstruction loss, in \cryoai with a ``symmetrized" L2 reconstruction loss and in \egmm with a tailored reconstruction loss that relies on the Fourier ring correlation (FRC) reconstruction metric.
%and can be interpreted as using a different noise model for $\epsilon_i$ in $\text{Dec}_\theta(h_i) +\epsilon_i$.

\cryovaegan, \cryodrgn, \cryofold, and \cryodeepmind use VAEs with a variational family of Gaussian distributions with diagonal covariance matrix, to respectively infer $(R_i, \text{CTF}_i)$ (CryoVAEGAN), $z_i$ (CryoDRGN and CryoFold) and $(z_i, R_i)$ (atomVAE) -- see Table~\ref{tab:inference}.

%\cryovaegan uses this inference method to infer the rotation $R_i$ and the $\text{CTF}_i$ latent variables.\cryodrgn and \cryofold use this method to infer the conformation variable $z_i$. \cryodeepmind uses it to infer the rotation $R_i$ and the conformation variable $z_i$.

The VAE architecture is used in \cryodrgn with the negative ELBO loss, and in \cryovaegan with the negative ELBO loss extended with the $\beta$ hyper-parameter described in the supplementary materials, an additional geometric regularization term, while the reconstruction loss relies on the binary cross-entropy as opposed to the L2 reconstruction loss. \cryodeepmind also implements a VAE with a modified ELBO loss that relies on important sampling (not detailed in this review), that leverages the $\beta$ hyperparameter and additionally includes a ``structure loss" --- see supplementary materials. 


==> CryoReview 2021 (6)/appE-constraints.tex <==
\setcounter{subsection}{0}
\renewcommand{\thesubsection}{E.\arabic{subsection}}

As described in the introduction and following the exposition by Scheres \cite{Scheres2012RELION} (2012), the molecule reconstruction problem is a difficult, highly non-linear inverse problem, which makes the parametrization of the shape and associated constraints particularly important. This parametrization amounts to impose structure on the desired reconstructed shapes --- either by leveraging domain knowledge on the properties of molecular volumes, or by using external information to guide the reconstruction.

\textit{From a physics/biology perspective}, this can be seen as a necessary enrichment of the cryo-EM data with either external assumptions and/or domain knowledge on the properties of the solution to ensure a more accurate recovery. \textit{From a statistics perspective}, formulated this way, the problem rapidly takes on a Bayesian flavour, and the objective of this step is to find the right ``prior" on the distribution of our latent variables. \textit{From a computational perspective}, this corresponds to adding additional terms to the loss/objective defining the optimization problem, and effectively explains what we term ``structure loss" in Section~\ref{sec2-inference}. We detail here the additional constraints that can equip the inference methods across the reconstruction algorithms.

%We can first incorporate constraints that relate to the structure of the volume itself, its invariances, symmetries or properties. In other words, we help the reconstruction problem by constraining the model to behave a certain way. Generally, in statistics, to constrain a model, we resort to three main types of structural priors: sparsity, smoothness and symmetries. In the context of cryo-EM, the last two constitute the bulk of the typical structural priors:
%--- which provides an alternative, perhaps simpler space to reason in, as we will see later in this review.\\
%Although explicit assumptions about the statistical characteristics of the noise are not often reported, commonly employed Wiener filters and cross-correlation goodness-of-fit measures rely on the assumption that the noise is independent and Gaussian distributed.

\subsection{Smoothness}


Smoothness refers to the property by which a signal, or quantity of interest, varies with "no abrupt change" over continuous regions. As explained by Scheres (2012) \cite{Scheres2012RELION}, "because macromolecules consist of atoms that are connected through chemical bonds, the scattering potential will vary smoothly in space, especially at less than atomic resolution."  Smoothness of the recovered scattering potential $V$ thus appears to be a reasonable assumption, which is implemented in different ways depending on the parametrization chosen:

\begin{description}
\item[Smoothness of the 3D image.] The smoothness assumption holds in image space as the image is a projection of the electron field --- which is itself continuous. This smoothness is encoded by the normal distribution. This also calls to mind the "ridge penalty", a similar type of regularisation in statistics.

%    This yields methods that \textbf{target inference in the image domain through the reconstruction of a 3D density function}. This is a potentially more efficient approach, since inference is done on the original space of the image. Yet, the non-linearity in Equation~\ref{eq:image} means that the model used to perform inference must be able to go beyond linearities --- at the price of potentially more complex algorithms.
\item[Smoothness of the Fourier coefficients.]   The smoothness of the 3D density map translates into smoothness over neighbouring Fourier coefficients. In a Bayesian pipeline, this is typically parametrized by assuming that these coefficients are sampled from a normal distribution.  
    The RELION algorithm (Scheres \cite{Scheres2012RELION}) is based on such a smoothness assumption.  This prior is encoded by assuming independent Gaussian priors on the Fourier components of the signal: $ V_l \sim N(0, \tau_l^2) $. Note here that the algorithm is not encouraging any other type of structure (e.g sparsity through spike-and-slab prior, etc).
    
\item[Smoothness of the deformation field.] 3DFlex \cite{Punjani2021} directly exploits the knowledge that conformational variability of a protein is the result of physical processes that transport density over space.  This means that mass and local geometry are preserved. As a result, this method implements a convection operator that outputs the deformation field. 3DFlex exploits prior knowledge of smoothness and local rigidity in the deformation field. 

\item[Smoothness of the function over 3D coordinates in Fourier domain.] Cryo-DRGN\cite{Zhong2019ReconstructingModels} and Cryo-Fold\cite{zhong2021exploring} represent the volume as the function $f: \Omega^3 \rightarrow \mathbb{R}$ over a 3D domain. In practice, this function is implemented by a neural network, which constrains it to be continuous, and possibly smooth if the activation functions used by the network are themselves smooth (sigmoids, for example).
\end{description}


\subsection{Rigidity}


Other constraints exploit physical properties and knowledge of the system to constrain the reconstruction. Specifically, due to the fact that the molecules studied in cryo-EM are frozen, we can assume that their conformational heterogeneity will not present large variations. As a result, we can assume that the molecular structure has some type of ``rigidity". This is implemented in practice by refraining the variables describing the shape heterogeneity from varying excessively. Depending on the parametrization chosen to represent the volume heterogeneity, the rigidity constraint takes different forms:

\begin{description}
\item[Rigidity of the deformation field.] The deformation field that parametrizes volume heterogeneity in 3D-Flex\cite{Punjani2021} can be constrained to only generate ``small" deformation, through a regularization term. This is integrated as a ``structure loss" of the deep learning training procedure of 3D-Flex\cite{Punjani2021}.
    
\item[Rigidity in (pseudo)-atoms coordinates.] The (pseudo-) atoms coordinates that parametrize the volume heterogeneity in Cryo-Fold\cite{zhong2021exploring} are constrained to be close to a base conformation's coordinates, via an $L2$ penalization on the deformations. This forms the ``structure loss" integrated in the objective function for the training procedure.

\item[Rigidity in deviation from (pseudo)-atoms coordinates.] Here, the volume is parametrized as a set of deviations of pseudo-atoms coordinates, compared to a base conformation, as in Cryo-DeepMind\cite{Rosenbaum2021}. The rigidity of the molecular structure is thus enforced by adding a constraint that takes the form of a L2 regularization constraining the $\Delta c_j$ to be small, and effectively forming the ``structure loss" added to the optimization objective of this approach.
\end{description}

We also note that the methods that do not assume any heterogeneity in volumes $V_i$ but rather model the volume as a unique possible conformation $V$, are essentially relying on the rigidity assumption, assuming that variations around $V$ are not large. 


% High resolution methods that assume rigidity of the target molecule, which can result in blurred, low-resolution density for flexible regions \cite{Punjani2017CryoSPARC:Determination}.This has led to the development of methods that target non uniform refinement, which automatically accounts for structural variability.

% \paragraph{(b) Heterogeneity} Recent methods have began casting doubt on the validity of the smoothness assumption uniformly over space. In fact Punjani et al contend that smoothness does not hold uniformly, and smoothness priors that put equal weight  on all coefficients are at the risk of undersmoothing in some regions of the molecule, and oversmoothing in others.

% When are they going to suggest group-lasso/hierarchical Bayes for that one?


% \paragraph{(c) Geometry} The last main type of constraint typically found in the statistics literature consists in finding symmetries, invariances or equivariances in the structure of the data. Let us begin by summarizing what these notions mean in mathematics. A shape (parametrized by, let's say, a system of three coordinates) is said to be symmetric around an axis (let's call it $x$) if $s(x,y,z) = s(-x,y,z)$. The shape is said to be invariant to an action $\rho$ if it remains unchanged: $\rho s = s$. An example is translation invariance ---  in the context of cryo-EM, shape are typically not symmetric enough to be neither symmetric nor invariant. Finally, the shape is said to be equivariant if $\rho s(x,y,z) = s(\rho(x,y,z))$.  This is a property that make sense for cryo-EM: the shape is equivariant to the action of rotations for instance, and the recovered volume should make use of this property. This is starting point of the method taken by Miolane et al. \cite{MiolanePoitevin2020CVPR} lies on assuming geometric conditions for the latent space. In particular, the latent space that they recover is equipped with the representation of the group of 2D-rotations. 
% Formally, a Lie group can be thought of as a non-Euclidean space of continuous symmetries, where the product and inverse map are smooth functions --- the celebrated example being the group of 3D (or 2D) rotation SO(3) (resp. SO(2)) . For the purpose of this review, let us highlight that assuming that the data is equivariant to a \textbf{Lie} group action is essential to the computations down the line: the smoothness of the product and inverse operator make it easy to take gradients, and to solve for the model parameters. So, while the mathematical formalism behind Lie groups is beyond the scope of this article, let us emphasise the importance of assuming smoothness the group actions over the shape.\\
% In the case of cryo-EM, as per the discussion of Miolane et al, a more realistic assumption is that the space should be equipped with 3D rotations rather than 2D.
% %Additionally, the representation of the group of rotations is not enforced, but rather hypothesized and observed in the latent space by leveraging results from group theory in the image space.
% Demonstrating good performance on 2D-images, this paper paves the way for the consideration of geometry as a way of constraining the problem.
%proposed an approach where the latent space of the VAE is equipped with the representation of the Lie group of rotations. Miolane et al. showed that variational inference can be used to learn the 2D rotation from real data. However, only 2D rotations are considered in this paper. Additionally, the representation of the group of rotation is not enforced, but rather hypothesized and observed in the latent space by leveraging results from group theory in the image space.

% Note: interestingly, there seems to be very few methods that use CNNs for this task. It would seem that they would be a natural candidate. They could be because they encode spatial information, but not equivariances. So could we find a compromise?





==> CryoReview 2021 (6)/appF-experiments.tex <==
This appendix summarizes the experiments conducted in the papers cited in this review, in Table~\ref{tab:experiments}. As mentioned in the main text, we observe a great diversity of datasets, which explains the difficulty encountered in comparing methods' performances and accuracies.

\begin{table}[]
\scalebox{0.91}{
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\rowcolor[HTML]{EFEFEF} 
                                                           & Biomolecule                             & \# of images & Image size & Data Type    & Noise  \\ \hline
\rowcolor[HTML]{FAFAE7} 
\cellcolor[HTML]{EFEFEF}                                   & \cellcolor[HTML]{FAFAE7}                & 50,000       & 128 x 128  & Synthetic    & No/Yes \\ \cline{3-6} 
\rowcolor[HTML]{FAFAE7} 
\cellcolor[HTML]{EFEFEF} &
  \multirow{-2}{*}{\cellcolor[HTML]{FAFAE7}Ribosome 80S (EMPIAR-10028)} &
  105,247 &
  90 x 90 &
  Experimental &
  Yes \\ \cline{2-6} 
\rowcolor[HTML]{FAFAE7} 
\cellcolor[HTML]{EFEFEF}                                   & Ribosome 50S (EMPIAR-10076)             & 131,899      & 90 x 90    & Experimental & Yes    \\ \cline{2-6} 
\rowcolor[HTML]{FAFAE7} 
\multirow{-4}{*}{\cellcolor[HTML]{EFEFEF}\cryodrgn}        & Protein complex                         & 50,000       & 64 x 64    & Synthetic    & N/A    \\ \hline
\rowcolor[HTML]{FAFAE7} 
\cellcolor[HTML]{EFEFEF}\cryofold                          & Haemoglobin (PDB 5NI1)                  & 50,000       & 128 x 128  & Synthetic    & Yes    \\ \hline
\rowcolor[HTML]{FAFAE7} 
\cellcolor[HTML]{EFEFEF}                                   & Tri-snRNP spliceosome (EMPIAR-10073)    & 102,500      & 180 x 180  & Experimental & Yes    \\ \cline{2-6} 
\rowcolor[HTML]{FAFAE7} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\threedflex} &
  TRPV1 ion-channel (EMPIAR-10059) &
  200,000 &
  128 x 128 &
  Experimental &
  Yes \\ \hline
\rowcolor[HTML]{FEF5F4} 
\cellcolor[HTML]{EFEFEF}\cryoposenet                       & E.coli adenylate kinase (PDB 4AKE1)     & 9,000        & 128 x 128  & Synthetic    & No/Yes \\ \hline
\rowcolor[HTML]{FAFAE7} 
\cellcolor[HTML]{EFEFEF}                                   & Ribosome 50S (EMPIAR-10076)             & 124,900      & N/A        & Experimental & Yes    \\ \cline{2-6} 
\rowcolor[HTML]{FAFAE7} 
\cellcolor[HTML]{EFEFEF}                                   & Precatalytic spliceosome (EMPIAR-10180) & 327,490      & N/A        & Experimental & Yes    \\ \cline{2-6} 
\rowcolor[HTML]{FAFAE7} 
\multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}\egmm}            & SARS-CoV-2 spike protein (EMPIAR-10492) & 55,159       & N/A        & Experimental & Yes    \\ \hline
\rowcolor[HTML]{FEF5F4} 
\cellcolor[HTML]{EFEFEF}\cryomaxwelling                    & GroEL-GroES protein                     & 40,000       & 128 x 128  & Synthetic    & Yes    \\ \hline
\rowcolor[HTML]{FEF5F4} 
\cellcolor[HTML]{EFEFEF}                                   & \cellcolor[HTML]{FEF5F4}                & 2, 544       & 128 x 128  & Synthetic    & No     \\ \cline{3-6} 
\rowcolor[HTML]{FEF5F4} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\cryovaegan} &
  \multirow{-2}{*}{\cellcolor[HTML]{FEF5F4}Ribosome 80S (EMPIAR-10028)} &
  5,119 - 8,278 - 4,917 &
  128 x 128 &
  Experimental &
  Yes \\ \hline
\rowcolor[HTML]{FAFAE7} 
\cellcolor[HTML]{EFEFEF}\cryodeepmind                      & Aurora A Kinase (Simulated)             & 63,000       & 64 x 64    & Synthetic    & Yes    \\ \hline
\rowcolor[HTML]{FAFAE7} 
\cellcolor[HTML]{FAFAE7}                                   & 80S ribosome (PDB 3J79 and 3J7A)        & 1,000,000    & 128 x 128  & Synthetic    & No/Yes \\ \cline{2-6} 
\rowcolor[HTML]{FAFAE7} 
\cellcolor[HTML]{FAFAE7}                                   & SARS-CoV-2 spike protein (PDB 6VYB)     & 1,000,000    & 128 x 128  & Synthetic    & No/Yes \\ \cline{2-6} 
\rowcolor[HTML]{FAFAE7} 
\cellcolor[HTML]{FAFAE7}                                   & Spliceosome (PDB 5NRL)                  & 1,000,000    & 128 x 128  & Synthetic    & No/Yes \\ \cline{2-6} 
\rowcolor[HTML]{FAFAE7} 
\multirow{-4}{*}{\cellcolor[HTML]{FAFAE7}\cryoai}          & 80S ribosome (EMPIAR-10028)             & 105,247      & 256 x 256  & Experimental & Yes    \\ \hline
\rowcolor[HTML]{FEF5F4} 
\cellcolor[HTML]{EFEFEF}\cryogan                           & $\beta$-galactosidase                   & 41,000       & 180 x 180  & Synthetic    & Yes    \\ \hline
\rowcolor[HTML]{FEF5F4} 
\cellcolor[HTML]{EFEFEF}                                   & $\beta$-galactosidase (EMPIAR-10061)    & 41,123       & 192 x 192  & Experimental & Yes    \\ \hline
\rowcolor[HTML]{FAFAE7} 
\cellcolor[HTML]{EFEFEF}\multicryogan & Heat-shock protein Hsp90                & 100,000      & 32 x 32    & Synthetic    & Yes    \\ \hline
\end{tabular}
}
\caption{Summary of synthetic and experimental cryo-EM datasets on which the reconstruction methods have been tested. The light red background indicates methods that perform homogeneous reconstruction, and the light yellow background heterogeneous reconstructions.}
\label{tab:experiments}
\end{table}

==> CryoReview 2021 (6)/appG-classification.tex <==

This last appendix provides details in the classification of the reconstruction methods, in the form of two tables. Table~\ref{tab:volumes} compares the generative models and Table~\ref{tab:inference} compares the inference methods. 

\begin{table}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|
>{\columncolor[HTML]{D9EAFF}}c |
>{\columncolor[HTML]{D9EAFF}}c |
>{\columncolor[HTML]{D9EAFF}}c |
>{\columncolor[HTML]{D9EAFF}}c |
>{\columncolor[HTML]{D9EAFF}}c |
>{\columncolor[HTML]{D9EAFF}}c |}
\hline
    %\parbox[c]{2mm}{\cellcolor[HTML]{EFEFEF}}& 
    \multicolumn{2}{|c|}{\cellcolor[HTML]{EFEFEF}
        \textbf{\begin{tabular}[c]{@{}c@{}}Volume\\Param.\end{tabular}}} & 
    \cellcolor[HTML]{EFEFEF}
        \textbf{Space} &
    \cellcolor[HTML]{EFEFEF}\textbf{Conformational Model} &
        %\textbf{\begin{tabular}[c]{@{}c@{}}Conformational\\Model\end{tabular}} & 
    \cellcolor[HTML]{EFEFEF}
        \textbf{Approach} &
    \cellcolor[HTML]{EFEFEF}
        \textbf{\begin{tabular}[c]{@{}c@{}}Hidden\\ Variable\end{tabular}} &
    \cellcolor[HTML]{EFEFEF}
        \textbf{\begin{tabular}[c]{@{}c@{}}Known\\ Variable\end{tabular}} &
    \cellcolor[HTML]{EFEFEF}
        \textbf{\begin{tabular}[c]{@{}c@{}}Reference\\ Volume\end{tabular}}\\ 
\hline
    \hline
        & 
        & 
        \cellcolor[HTML]{D9EAFF} & 
        \cellcolor[HTML]{D9EAFF} & 
        \cryoposenet & 
        \begin{tabular}[c]{@{}c@{}}-\\Rotation\\-\end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}CTF\\-\\Translation\end{tabular} & 
        Free\\ 
    \cline{5-8} 
        & 
        &
        \multirow{-2}{*}{\cellcolor[HTML]{D9EAFF}Image} & 
        \multirow{-2}{*}{\cellcolor[HTML]{D9EAFF}
            \begin{tabular}[c]{@{}c@{}}Homogeneous\\ $z \longrightarrow V$ \end{tabular}} &
        \cryogan &
        \begin{tabular}[c]{@{}c@{}}-\\Rotation\\Translation\end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}CTF\\-\\-\end{tabular} & 
        Free\\
    \cline{4-8} 
        \parbox[c]{2mm}{\multirow{-3}{*}{\rotatebox[origin=c]{90}{\textbf{Discrete Representation}}}} & 
        \parbox[c]{2mm}{\multirow{-2}{*}{\rotatebox[origin=c]{90}{Voxel Grid}}} & 
        & 
        \begin{tabular}[c]{@{}c@{}}Heterogeneous\\ $z \longrightarrow V$ \end{tabular} & 
        \multicryogan & 
        \begin{tabular}[c]{@{}c@{}}-\\Rotation\\Translation\end{tabular}& 
        \begin{tabular}[c]{@{}c@{}}CTF\\-\\-\end{tabular} &
        Free\\ 
  \cline{4-8}
        & & &
        \begin{tabular}[c]{@{}c@{}}Heterogeneous\\ $z \longrightarrow f(U(z_j), V_0)$ \end{tabular} & 
        \threedflex & 
        \begin{tabular}[c]{@{}c@{}}-\\-\\-\end{tabular}& 
        \begin{tabular}[c]{@{}c@{}}CTF\\Rotation\\Translation\end{tabular} &
        Yes\\ 
    \cline{3-8} 
        &
        & 
        \cellcolor[HTML]{DFFFD3} & 
        \cellcolor[HTML]{DFFFD3}
            \begin{tabular}[c]{@{}c@{}}Homogeneous\\ $z = (\mu_V, \sigma_V) \longrightarrow V$\end{tabular}& 
        \cellcolor[HTML]{DFFFD3}\cryomaxwelling & 
        \cellcolor[HTML]{DFFFD3}
            \begin{tabular}[c]{@{}c@{}}-\\Rotation\\Translation\end{tabular}&
        \cellcolor[HTML]{DFFFD3}
            \begin{tabular}[c]{@{}c@{}}CTF\\-\\-\end{tabular} &
        \cellcolor[HTML]{DFFFD3}Free\\
    \cline{4-8} 
        & 
        & 
        \multirow{-2}{*}{\cellcolor[HTML]{DFFFD3}Fourier} & 
        \cellcolor[HTML]{DFFFD3}
            \begin{tabular}[c]{@{}c@{}}Heterogeneous\\ $z \in \{1, .., K\} \longrightarrow \{V_1, ..., V_K\}$ \end{tabular}& 
        \cellcolor[HTML]{DFFFD3}\relion &
        \cellcolor[HTML]{DFFFD3}
            \begin{tabular}[c]{@{}c@{}}-\\Rotation\\Translation\end{tabular}&
        \cellcolor[HTML]{DFFFD3}
            \begin{tabular}[c]{@{}c@{}}CTF\\-\\-\end{tabular} &
        \cellcolor[HTML]{DFFFD3}Free\\ 
    \cline{4-8} 
        & 
        & 
        \multirow{-2}{*}{\cellcolor[HTML]{DFFFD3}} & 
        \cellcolor[HTML]{DFFFD3}
            \begin{tabular}[c]{@{}c@{}}Heterogeneous\\ $z \in \{1, .., K\} \longrightarrow \{V_1, ..., V_K\}$ \end{tabular}& 
        \cellcolor[HTML]{DFFFD3}\cryosparc &
        \cellcolor[HTML]{DFFFD3}
            \begin{tabular}[c]{@{}c@{}}-\\Rotation\\Translation\end{tabular}&
        \cellcolor[HTML]{DFFFD3}
            \begin{tabular}[c]{@{}c@{}}CTF\\-\\-\end{tabular} &
        \cellcolor[HTML]{DFFFD3}Free\\ 
    \hline
    \hline
        & 
        \parbox[t]{2mm}{}{\multirow{-1}{*}{\rotatebox[origin=c]{90}{\begin{tabular}[c]{@{}c@{}}Neural\\ Network\end{tabular}}}} & 
        Image & 
        \begin{tabular}[c]{@{}c@{}}Homogeneous\\ $z = (\mu_V, \sigma_V, CTF_V) \longrightarrow V_i(2D)$\end{tabular} & 
        \cryovaegan & 
        \begin{tabular}[c]{@{}c@{}}CTF\\2D Rotation\\-\end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}-\\-\\Translation\end{tabular} &
        Free\\ 
    \cline{3-8} 
        \parbox[t]{2mm}{\multirow{-2}{*}{\rotatebox[origin=c]{90}{\textbf{Continuous Field}}}} & 
        & 
        \cellcolor[HTML]{DFFFD3} & 
        \cellcolor[HTML]{DFFFD3}
            \begin{tabular}[c]{@{}c@{}}Heterogeneous\\ $z \longrightarrow V_j$\end{tabular} & 
        \cellcolor[HTML]{DFFFD3}\cryodrgn & 
        \cellcolor[HTML]{DFFFD3}
            \begin{tabular}[c]{@{}c@{}}-\\Rotation\\Translation\end{tabular}&
        \cellcolor[HTML]{DFFFD3}
            \begin{tabular}[c]{@{}c@{}}CTF\\-\\-\end{tabular} &   
        \cellcolor[HTML]{DFFFD3}Free\\ 
        \cline{4-8}
        & &
        \cellcolor[HTML]{DFFFD3}Fourier & 
        \cellcolor[HTML]{DFFFD3}
            \begin{tabular}[c]{@{}c@{}}Homogeneous\\ $z \longrightarrow V_j$\end{tabular} & 
        \cellcolor[HTML]{DFFFD3}\cryoai & 
        \cellcolor[HTML]{DFFFD3}
            \begin{tabular}[c]{@{}c@{}}-\\Rotation\\Translation\end{tabular}&
        \cellcolor[HTML]{DFFFD3}
            \begin{tabular}[c]{@{}c@{}}CTF\\-\\-\end{tabular} &   
        \cellcolor[HTML]{DFFFD3}Free\\ 
    \cline{2-8}
        &
        &
        &
        \cellcolor[HTML]{D9EAFF}
            \begin{tabular}[c]{@{}c@{}}Heterogeneous\\ $z \longrightarrow \{c_j, A_j, \sigma_j\}_{j\in[1,N]}$ or $\{\Delta c_j\}_{j\in[1,N]}$ ; ($N$ ``blobs") \end{tabular}& 
        \egmm & 
        \cellcolor[HTML]{D9EAFF}
            \begin{tabular}[c]{@{}c@{}}-\\-\\-\end{tabular}& 
        \cellcolor[HTML]{D9EAFF}
            \begin{tabular}[c]{@{}c@{}}CTF\\Rotation\\Translation\end{tabular} &
        \cellcolor[HTML]{D9EAFF}Free or Yes\\ 
    \cline{4-8}
        &
        \parbox[t]{2mm}{}{\multirow{-2}{*}{\rotatebox[origin=c]{90}{\begin{tabular}[c]{@{}c@{}}Gaussian\\ Mixture\end{tabular}}}} &
        \multirow{-2}{*}{\cellcolor[HTML]{D9EAFF}Image} &
        \cellcolor[HTML]{D9EAFF}
            \begin{tabular}[c]{@{}c@{}}Heterogeneous\\ $z \longrightarrow \{c_j\}_{j\in[1,N]}$; ($N$ residues) \end{tabular}& 
        \cryofold& 
        \cellcolor[HTML]{D9EAFF}
            \begin{tabular}[c]{@{}c@{}}-\\-\\-\end{tabular}& 
        \cellcolor[HTML]{D9EAFF}
            \begin{tabular}[c]{@{}c@{}}CTF\\Rotation\\Translation\end{tabular} &
        \cellcolor[HTML]{D9EAFF}Free\\ 
    \cline{4-8}
        &
        &
        &
        \cellcolor[HTML]{D9EAFF}
            \begin{tabular}[c]{@{}c@{}}Heterogeneous\\ $z \longrightarrow \{\Delta c_j\}_{j\in[1,N]}$; ($N$ residues) \end{tabular}& 
        \cryodeepmind& 
        \cellcolor[HTML]{D9EAFF}
            \begin{tabular}[c]{@{}c@{}}-\\Rotation\\Translation\end{tabular}& 
        \cellcolor[HTML]{D9EAFF}
            \begin{tabular}[c]{@{}c@{}}CTF\\-\\-\end{tabular} &
        \cellcolor[HTML]{D9EAFF}Yes\\ 
    \hline
\end{tabular}
}
\caption{Classification of reconstruction methods in terms of the parametrization of the volume $V$ (or $\tilde{V}$), \textit{i.e.} the model of conformational heterogeneity with the conformation variable $z$, use of image versus Fourier space, representation as a discrete or continuous field, and with a reference-free or reference-based encoding. We also indicate whether nuisance variables are hidden or assumed to be known in the reconstruction methods cited. When not specified, the latent variable $z$ belongs to a vector space $\mathbb{R}^L$.} 
\label{tab:volumes}
\end{table}


\begin{table}[]
\scalebox{0.98}{
\begin{tabular}{|c|c|cc|cc|}
\hline
\rowcolor[HTML]{DAE8FC} 
\cellcolor[HTML]{EFEFEF} &
  \textbf{Posterior $p(h_i|x_i)$} &
  \multicolumn{2}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Mode $\hat h_i$}} &
  \multicolumn{2}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Variational $q(h_i)$}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
 &
  \textbf{} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Non-Amortized}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Amortized \\ (encoder)\end{tabular}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Non-Amortized}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Amortized\\ (encoder)\end{tabular}} \\ \hline
Distribution on $h_i$ &
  $p(h_i|x_i)$ &
  \multicolumn{1}{c|}{$ \argmax _z p(h_i|x_i)$} &
  $\text{Enc}_\xi(x_i)$ &
  \multicolumn{1}{c|}{$q_{\eta_i}  \in \mathcal{Q}$} &
  $q_{\text{Enc}_\xi(x_i)}\in \mathcal{Q}$ \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}\textbf{Name}} &
  \textbf{EM} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Approx. EM}} &
  \textbf{Am. EM / AE} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Var. EM  / AD}} &
  \textbf{Var. Am. EM / VAE} \\ \hline
\cellcolor[HTML]{EFEFEF} &
  \begin{tabular}[c]{@{}c@{}}RELION\cite{Scheres2012RELION}\\ (pose $R_i, t_i$ and \\ conformation $z_i$)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}RELION\cite{Scheres2012RELION}\\ (noise $\sigma_i$) (*)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}CryoPoseNet \cite{Nashed2021endtoend} \\ (rotation $R_i$)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3DFlex\cite{Punjani2021}\\ (conformation $z_i$)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}CryoDRGN\cite{Zhong2019ReconstructingModels}\\ (conformation $z_i$)\end{tabular} \\ \cline{2-6} 
\cellcolor[HTML]{EFEFEF} &
   &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\cryosparc\\ (rotation $R_i$) (*)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}E2GMM\cite{Chen2021}\\ (conformation $z_i$)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\cryomaxwelling\\ (pose $R_i, t_i$ and \\ conformation $z$)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}CryoVAEGAN\cite{MiolanePoitevin2020CVPR}\\ (2D rotation $R_i$\\ and $\text{CTF}_i$)\end{tabular} \\ \cline{2-6} 
\cellcolor[HTML]{EFEFEF} &
   &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}CryoDRGN\cite{Zhong2019ReconstructingModels}\\ (pose $R_i, t_i$) (*)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}\cryoai \\ (pose $R_i, t_i$)\end{tabular} &
  \multicolumn{1}{c|}{} &
  \begin{tabular}[c]{@{}c@{}}atomVAE\cite{Rosenbaum2021}\\ (pose $R_i, t_i$ and \\ conformation $z_i$)\end{tabular} \\ \cline{2-6} 
\multirow{-4}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Inference on $h_i$\\ (E-step)\end{tabular}} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}3DFlex\cite{Punjani2021}\\ (conformation $z_i$)\end{tabular}} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \begin{tabular}[c]{@{}c@{}}CryoFold\cite{zhong2021exploring}\\ (conformation $z_i$)\end{tabular} \\ \hline
\end{tabular}
}
\caption{Classification of cryo-EM reconstruction algorithms with respect to the inference on the conformation $z_i$ and on the unknown hidden variables $h_i$. The inference step updates the posterior $p(h_i|x_i$, or its mode $\hat h_i$, or a variational approximation $q(h_i)$ of it --- which corresponds to the 3 main columns of the table. The works by Zhong et al. (2019, 2021) are classified in several cells, as inference of the conformation $z_i$ is performed via a VAE, but the inference of the poses $R_i, t_i$ is performed with an optimization algorithm. The notation (*) specifies that the optimization associated with this step is fully performed (until convergence to local extremum) while its absence indicates that only a gradient step is taken toward the optimum.}
\label{tab:inference}
\end{table}

==> CryoReview 2021 (6)/dynamics.tex <==
\section{Determination of conformational landscapes}

most recent \cite{GOMEZBLANCO2022106673}

==> CryoReview 2021 (6)/glossary.tex <==
\newglossaryentry{cryoem}
{
    name=cryo-EM,
    description={Cryogenic Electron Microscopy}
}

\newglossaryentry{reconstruction}
{
    name=reconstruction,
    description={In the context of imaging, reconstruction usually refers to tomographic reconstruction of 2D images into a 3D volume}
}

\newglossaryentry{poses}
{
    name=poses,
    description={The unknown 3D orientation and 2D translation of the particle within a given projection image}
}

\newglossaryentry{generativemodel}
{
    name=generative model,
    description={A generative model is a statistical model of the joint probability distribution for the data and the underlying quantity of interest. It is a process that describes how data is generated, using probability distributions. By sampling from this model, we create new data points}
}

\newglossaryentry{deepgenerativemodels}
{
    name=deep generative models,
    description={A class of generative models leveraging deep neural networks}
}

\newglossaryentry{spi}
{
    name=single particle images,
    description={Single Particle Imaging refers to imaging modalities where data, \emph{albeit} corrupted, is collected about individual particles, as opposed to ensemble averaging imaging modalities such as X-ray crystallography or NMR}
}

\newglossaryentry{particles}
{
    name=particles,
    description={In cryo-EM, each copy of an imaged molecule is referred to as a \emph{particle}}
}

\newglossaryentry{conformational-hetero}
{
    name=heterogeneity,
    description={%A defining characteristic of single particle cryo-EM is its ability to image individual \gls{particles} of the target object. 
    Heterogeneity refers to structural variability between the imaged particles, whether from compositional variability in the sample or conformational dynamics associated with the molecule. Heterogeneous reconstruction algorithm aim to model the \gls{conformation landscape} associated with the target molecule}
}

\newglossaryentry{conformation landscape}
{
    name=conformational landscape,
    description={Molecules exhibit shape variability as they thermally diffuse on their high-dimensional energy potential surface, also known as their conformation landscape. Indeed, each atom of the molecule is associated with 6 degrees of freedom, three for their position in space and three for their momentum. The joint distribution over all these degrees of freedom is directly related to the pairwise interaction between atoms which add up to the potential energy of the molecule. The likelihood of a conformation is dictated by the potential energy value associated with this conformation and thus by the relative position of atoms. One could think of the potential energy function as a surface in high-dimension with basins corresponding to stable conformations separated by high energy intermediates. The overall energy scale and relative depths of the basins is dictated by thermodynamics observables such as the temperature; Low temperature will exacerbate differences in energy and differentially increase the likelihood of conformations found in basins relative to higher energy intermediate, for example}
}

\newglossaryentry{colvar}
{
    name=collective variables,
    description={The conformational space of a molecule can be defined by features that are functions of the coordinates of the molecule's atoms, often referred to as collective variables since most interesting features tend to capture global collective motions of the atoms}
}


%%%%%%% ACRONYMS %%%%%

\newacronym{ctf}{CTF}{Contrast Transfer Function}

\newacronym{psf}{PSF}{Point Spread Function}

\newacronym{ml}{ML}{Maximum Likelihood}

\newacronym{map}{MAP}{Maximum a Posteriori}

\newacronym{em}{EM}{Expectation-Maximization}

\newacronym{elbo}{ELBO}{Evidence Lower Bound}

\newacronym{kl}{KL}{Kullback-Leibler divergence}

\newacronym{vi}{VI}{Variational Inference}

\newacronym{ai}{AI}{Amortized Inference}

\newacronym{gan}{GAN}{Generative Adversarial Network}

\newacronym{fsc}{FSC}{Fourier Shell Correlation}

\newacronym{rmsd}{RMSD}{Root Mean Square Deviation}

==> CryoReview 2021 (6)/sec0-intro.tex <==

\begin{wrapfigure}{r}{0.4\textwidth}
\vspace*{-0.2in}
    \includegraphics[width=0.4\textwidth]{figs/cryo_genmodel_flat_biomol.pdf}
     \setlength{\belowcaptionskip}{-4pt} 
      \setlength{\abovecaptionskip}{-4pt} 
    \caption{Acquisition of 2D cryo-EM images (2D projections) from 3D biomolecular volumes.}
    \label{fig:electron_microscope}  \vspace*{-0.08in}
\end{wrapfigure}

High-resolution reconstruction of molecular volumes from \gls{spi} has the potential to facilitate new breakthroughs in our ability to understand fundamental biological mechanisms and engineer macromolecular function \cite{Ourmazd2019,Renaud2018cryo}. In this context, cryo-electron microscopy (\gls{cryoem}) has fostered a revolution in structural biology by allowing the imaging of biomolecules in solution at atomic resolution \cite{Nakane2020atomicres,emdb}.
However, the estimation of these molecules' 3-dimensional (3D) volume from cryo-EM data continues to pose a formidable challenge. In this setting, observations are limited to the raw 2D projections of molecules  (also called \gls{particles}) relative to an incoming electron beam, while their 3D orientation and position (jointly called \gls{poses}) are unknown --- see Figure~\ref{fig:electron_microscope}. Reconstructing molecular volumes therefore also requires recovering a number of hidden variables such as each particle's 3D orientation. The difficulty of this task is further compounded by a combination of factors, including the variability in the shape of any given molecule (also referred to as structural ``\gls{conformational-hetero}''), the non-linear physics of the data acquisition process, as well as extremely low signal-to-noise ratios --- concepts formalized in the image formation model below.

    
 \paragraph{Image Formation Model.}
The process of image formation in cryo-EM involves several physical phenomena, including pairwise interactions between atoms, interactions between the electron beam and the molecule's electrostatic potential, or microscope effects. 
We refer the reader to Dill \textit{et al.}\cite{dill2010molecular}, Kohl and Reimer\cite{Kohl}, and Vulovic \textit{et al.}\cite{VULOVIC201319} for in-depth descriptions of these phenomena. Nonetheless, in most cases\cite{Scheres2012RELION,VULOVIC201319}, each image $X_i$ in a dataset of  $n$ images of single \gls{particles}
can be modeled as a random sample from the following \gls{generativemodel}:
\begin{equation}\label{eq:image}
    X_i = \text{PSF}_i * (t_i \circ \Pi_{2D} \circ R_i) (V^{(i)})  + \epsilon_i, \qquad \text{with} \quad i=1 \cdots n.
\end{equation}
\noindent Here, $R_i$ is a 3D rotation representing the 3D orientation of the volume $V^{(i)}$ with respect to the direction of the electron beam. The oriented volume is subsequently ``pierced through'' by the electron beam and projected onto the detector --- an operation represented in Equation~\eqref{eq:image} by the 2D-projection operator $\Pi_{2D}$. The  variable $t_i$ represents the 2D translation of the projected volume with respect to the center of the image. %The rotation $R_i$ and translation $t_i$ are collectively called the ``pose" variables. 
The effect of the microscope's lens is modeled through the convolution $*$ of the 2D projection by an image-dependent operator $\text{PSF}_i$ called the Point Spread Function (\acrshort{psf}) of the microscope whose parameters can depend on the image. Finally, additional noise $\epsilon_i$ is introduced in the observed image, and typically assumed to be Gaussian with zero mean and variance $\sigma_i^2$. Note that the underlying volume $V^{(i)}$ is allowed to depend on $i$. This allows us to account for ``conformational heterogeneity'', a concept whereby a molecule does not necessarily exist in a single state, but rather, that its volume corresponds in fact to one of several stable geometries that can be achieved by this  molecule.

An equivalent generative model can be formulated via the Fourier transform of Equation~\eqref{eq:image} which we present in Appendix~\ref{appB-operators}. In Fourier Space, the convolution $*$ of the projected volume by the PSF becomes a computationally lightweight element-wise matrix multiplication $\odot$ between the 2D Fourier transform of the projected image and that of the PSF (known  as the {\it Contrast Transfer Function}, or {\it CTF}). Operating in Fourier space is thus common in many cryo-EM volume reconstruction algorithms.



%\paragraph{The reconstruction problem} The objective of this inference problem is therefore to recover the underlying shape $V$. This would be a standard statistical problem, were it not for the fact that the variables $H_i= (\text{PSF}_i, \sigma_i, t_i, R_i, z_i)$ (\textit{i.e.} the covariates of the image) are unknown --- also called "hidden" or "latent" in statistical terminology. Thus, they will have to be filled in --- or ``imputed''. This yields a difficult and expensive statistical problem: the number of unknowns and variables increases with the size $n$ of the dataset, as for each particle image $X_i$, we need to (1) find the associated rotation $R_i$, translation $t_i$, $\text{PSF}_i$, $\sigma_i$ and conformation variable $z_i$ to (2) impute a description of the conformational landscape $V$.

\paragraph{Challenges of Cryo-EM and Deep Generative Modeling.} Whether in image or Fourier space, the image formation model described by Equation~\eqref{eq:image} gives us the first clue about the difficulty of the reconstruction problem. \textit{Only the recovery of the set of possible 3D molecular volumes $V^{(i)}$  (called the  \gls{conformation landscape}) is relevant - yet the image also depends on a number of additional unknown nuisance variables}, such as
%Note here that the index $i$ indicates a possible dependency of the volume on the image: as we will describe in the next section, a number of current methods for high-resolution volume reconstruction try and account for "conformation heterogeneity", or image-specific deviations from a given baseline conformation. On the other hand, 
the pose  ($R_i$, $t_i$) or the microscope-dependent $\text{PSF}_i$. As noted by Singer \textit{et al.} \cite{singer2020computational}, these nuisance variables do not bring any information of biological relevance but may impact the quality (and difficulty) of the reconstruction. Reconstructing molecular volumes thus becomes a highly non-convex optimization problem, putting algorithms at risk of being overly sensitive to initialization \cite{Rosenbaum2021} or converging to one of many local minima \cite{boyd2004convex}. The difficulty of the task is also compounded by the high levels of radiation damage, structured (non-white) noise and altogether remarkably low signal-to-noise ratios that cryo-EM images usually exhibit. Given these difficulties, reconstruction algorithms rely on using copious amounts of data, but often struggle to process the wealth of incoming images\cite{Kimanius2016AcceleratedRELION-2}, to the point where ``the cost of image analysis can exceed 500,000 CPU hours on large, expensive computer clusters''\cite{Punjani2017CryoSPARC:Determination} for a single experiment. In this context, recent efforts have turned to unsupervised deep learning for cryo-EM reconstruction, \textit{i.e.} approaches allowing significant speed-ups through the use of gradient methods and GPUs. Given their potential to advance the field by addressing the challenges mentioned here, we propose here a critical review of deep generative modeling for cryo-EM volume reconstruction. 


%conditions for which traditional methods from computer vision and deep learning have often not been stress-tested. 

%and thus need to be estimated together with $V^{(i)}$. 


% This, together with low signal-to-noise ratio, makes cryo-EM reconstruction an exceedingly difficult problem. 
% %Most advances in volume reconstruction typically focus on one part of the recovery (e.g. jointly inferring volumes $V^{(i)}$ and rotations $R_i$), while assuming the remainder of variables to be estimable ahead of time via an external algorithm. 
% In this context, method design face three main challenges:
% \begin{description}[topsep=0em, leftmargin=0.3cm, noitemsep]
% \item[(a) Scalability.] Due to the number of unknown variables that have to be estimated, algorithms must rely 
% \item[(b) Robustness to initial conditions.] The high number of unknown variables 
% \item[(c) Robustness to noise.] Experimental cryo-EM images, characterized by image sample damage, structured (non-white) noise and altogether remarkably low signal-to-noise regimes may lead to failures of reconstruction methods.
% \end{description}

% Despite these challenges, the last three years have witnessed a proliferation of new reconstructions methods anchored in deep generative modeling and unsupervised deep learning. Among other advantages, these approaches . In light of these methods' potential 

% However, despite promising results on simulated datasets, these methods face considerable challenges when applied to real cryo-EM images, characterized by image sample damage, structured (non-white) noise and altogether remarkably low signal-to-noise regimes\footnote{We refer the reader to Section~\ref{sec3-discussion} and Table~\ref{tab:experiments} for a detailed discussion on the experiments.}. Many of these algorithms have not been properly vetted and stress-tested in experimental conditions \cite{Ullrich2019,zhong2021exploring, Rosenbaum2021, Nashed2021endtoend}, and their ability to do well on real data remains elusive. 

%Together, these three hurdles make inference for cryo-EM volume reconstruction an immensely challenging area of research.%, both from a computational and from a statistical perspective.
% Cryo-EM reconstruction methods vary according to the amount of information that is assumed known, \textit{i.e.} which latent covariates in $H_i$ are assumed to be given (which implies that they must be computed beforehand via an external algorithm), and which will need to be imputed during reconstruction. In fact, almost all the approaches presented in this review assume that the CTF (or PSF) has been estimated and is known; it is indeed possible to estimate the CTF independently from reconstructing the volume\cite{Rohou2015CTFFIND4:Micrographs}

\paragraph{Related Work.} Several reviews have already begun surveying  challenges and advances in cryo-EM reconstruction.
%Several reviews have began to survey challenges and advances in the field, typically focusing on a subset of the various facets of this vast program. 
The reviews by Singer \textit{et al.}\cite{singer2020computational} and Bendory \textit{et al.}\cite{bendory2020single} provide a complete description of cryo-EM reconstruction, %including details on the physics of the imaging process along with the multiple stages of the reconstruction pipelines. 
but focus on mathematical foundations of general computational methods, rather than specifically on deep learning approaches. 
%In fact, most of the methods presented in these two reviews predate a number of the deep modeling methods presently described. 
Reviews by Si \textit{et al.}\cite{si2021artificial}, Ede \textit{et al.} \cite{ede2021deep} and Wu \textit{et al.} \cite{WuReview2021} describe the pervasiveness of deep learning methods along all steps of the cryo-EM pipeline, without specialising  to high-resolution volume reconstruction. By contrast, our review is a deep dive into the most recent deep generative models for cryo-EM reconstruction.%, and most methods we survey were not published at the times of the aforementioned reviews.
%We emphasize here that such generative approaches are not the only way of performing cryo-EM volume reconstruction. Other approaches (such as moment-based methods \cite{Sharon2019MethodAngles}) have been proposed, but fall outside of the scope of the present review. 
%Moreover, with the exception of cryoDRGN (Zhong \textit{et al.}, 2019 \cite{Zhong2019ReconstructingModels}), this review does not include the latest deep generative modeling methods.
%In the survey by Ede \textit{et al.} \cite{ede2021deep}, the role of deep learning in electron microscopy is reviewed in introduction in relation to problems of denoising, classification (labelling) and segmentation. 
%While this last review presents deep generative modeling and describes various architectures for autoencoders, variational autoencoders, and generative adversarial networks, the associated sections are mostly expository, and none of the most recent deep generative modeling advances in cryo-EM are included. Finally, the review by Wu \textit{et al.} \cite{WuReview2021} provides a recent update on the review by Ede \textit{et al.} \cite{ede2021deep} and includes a high-level description of the most recent deep generative modeling advances, but without any particular focus on the volume reconstruction problem. 

\paragraph{Objective and Contributions.} Our objective is to shed light into the similarities and differences among recent state-of-the-art, deep-generative reconstruction methods, which we classify according to {\it(i) \it their parametrization of the generative model} (Section~\ref{sec1-generative_models_and_lvms}) and {\it(ii) the inference tools} deployed to fit this generative model (Section~\ref{sec2-inference}). This unification of recent works along a consistent statistical framework allows us to highlight trends, outstanding challenges, and avenues for improvements in the field (Section \ref{sec3-discussion}). We draw insights from our experiences with these approaches to provide an account of the hurdles and potential difficulties that arise in their deployment to real cryo-EM data. Finally, through this review, we hope to catalyze deep learning advances by providing machine learning practitioners and computer vision experts a thorough overview of the challenges that are unique to cryo-EM. %We hope that this review will provide an avenue for these experts to quickly grasp the challenges of the field.% and to provide them more support as they start off in the field. 
% To summarize, our main contributions are:
% \begin{itemize}[itemsep=0.05em, topsep=0em, bottomsep=1em]
%     \item Organizing and contrasting state-of-the-art parametrization choices in cryo-EM deep generative modeling in Section~\ref{sec1-generative_models_and_lvms} and Tables~\ref{tab:volumes}-\ref{table:comp_two}, while highlighting the practical advantages and drawbacks of each choice.\vspace{-2mm}
%     \item Unifying state-of-the-art inference methods for cryo-EM reconstruction in a consistent statistical framework in Section~\ref{sec2-inference}, Figure~\ref{fig:vae} and Table~\ref{tab:inference}, while performing a critic of their performances in terms of accuracy-speed trade-offs.\vspace{-2mm}
%     \item Presenting outstanding issues, burning challenges and promising avenues for future research in deep generative models for cryo-EM reconstruction in Section~\ref{sec3-discussion} and Table~\ref{tab:experiments}.
% \end{itemize}


%While this review covers the statistical foundations for modern reconstruction methods in cryo-EM, it does not address other topics related to statistics such as validation metrics or connections with statistical thermodynamics. We leave these topics for future work.

%\paragraph{Our Objectives.} In this paper, we critically review recent cryo-EM reconstruction approaches leveraging deep generative modeling. Our review contrasts traditional generative methods with their new deep-learning based counterparts, while emphasizing the core statistical and computer science concepts behind each algorithm. We organize cryo-EM reconstruction pipelines according to (1) the parametrization of the reconstruction problem through generative models in Section~\ref{sec1-generative_models_and_lvms} and (2) the inference tools deployed to invert these generative models in Section~\ref{sec2-inference}. While this review covers the statistical foundations for modern reconstruction methods in cryo-EM, it does not address other topics related to statistics such as validation metrics or connections with statistical thermodynamics. We leave these topics for future work.

==> CryoReview 2021 (6)/sec1-generative_models.tex <==


The objective of cryo-EM imaging algorithms is to produce a 3D reconstruction of a given molecule from a dataset of images $\{X_i\}_{i =1 \cdots n}$, where each image corresponds to a ``2D projection'' of the molecule at a different (unknown) orientation and position (Figure~\ref{fig:electron_microscope}). A fundamental hurdle to this objective lies in the fact that each molecule has its own unknown conformation (or shape). Methods that account for this \gls{conformational-hetero} are called \textbf{heterogeneous reconstruction methods}, and can typically aspire to higher resolution reconstructions --- often at the cost of more involved and expensive computations. Conversely, \textbf{homogeneous reconstruction methods} neglect this shape variability and usually represent the \gls{conformation landscape} as a unique molecular volume. This section reviews how choices both in accounting for conformation heterogeneity and in parametrizing the volume yield different formulations of the cryo-EM image formation model. 

 
 \subsection{Conformation Variable $z$.}\label{confvarz}
 
Heterogeneous reconstruction methods introduce an additional variable $z_i$ for each image $i$ within the formation model of Equations~\eqref{eq:image}, which we call the conformation variable. Depending on whether conformation heterogeneity is modeled through a discrete number of states or as a continuous variable, the conformational landscape can be encoded as a discrete family of volumes $\mathcal{V}=\{V_z,~z \in\{1,\ldots,K\}\}$ \textbf{(discrete heterogeneity)}, or as a continuous family $\mathcal{V}=\{V(z),~z \in\mathbb{R}^L\}$ for some integer $L$ \textbf{(continuous heterogeneity)}\cite{Jonic2017}. In both cases, the family is indexed by the variable $z$. We use the notations $V_z$ and $V(z)$ interchangeably. Homogeneous reconstruction can in fact be taken as the special case where $\mathcal{V}$ only comprises a single volume, so that $K=1$ or $L=0$ (i.e. forcing $z=0$). We now write $V^{(i)} = V(z_i)$ in Equation~\eqref{eq:image}.

\paragraph{Interpretation of the Conformation Variable}
From a statistical mechanics perspective, the conformation variable $z_i$ encodes the location of any given single particle along the conformational landscape\cite{dill2010molecular}. For example, if $z_i\in \mathbb{R}$, $z_i$ can be used to sort conformations along a ``conformation path'', that is, a sequence of small transformations that would interpolate two main preferred, dynamically stable states (or conformations) for the molecule. When continuous, the dimension $L$ of this cursor variable $z$ could in principle take any value between 0 (no heterogeneity) and $O(N)$, with $N$ the number of atoms in the molecule. However, two factors tend to drastically limit the number of dimensions of $z$. First, most of the main global dynamics of a molecule are captured by a few \gls{colvar} associated with its low-frequency motion, effectively averaging out a lot of the effects of the high number of degrees of freedom associated with faster motions \cite{Noe2017}. Second, imaging conditions often reduce the ability to resolve the remaining motions, thus reducing the effective dimensionality of $z$\cite{Katsevich2015}. 
%(see Katsevich \emph{et al}\cite{Katsevich2015} for a mathematical discussion on the effective rank of the covariance matrix capturing variations around the mean 3D volume).
In other words, limits in the imaging technology itself restrict the dimension of the variable $z$. In the case of discrete heterogeneity, $z \in \{1, .., K\}$ is an index of minimum energy wells (conformations) in the conformational landscape. Imaging conditions also reduce the ability to resolve too many metastable states, thereby restricting practitioners to choose a low value for $K$.

\paragraph{Discrete vs Continuous Conformational Heterogeneity: Pros, Cons and Discussion.}
Discrete heterogeneity has a rich history in cryo-EM. Popularized by the Class3D\cite{Scheres2012RELION, SCHERES2010295} extension of \relion, it offers the advantage of delivering readily interpretable results: a set of $K$ volumes, representing $K$ main stable states of the molecules. Discrete heterogeneity is thus particularly adequate in certain (common) scenarios where the conformation landscape has local energy minima that produce distinct states. However, one of the main drawbacks of this method consists in the necessary selection of the number $K$ of appropriate conformations. Theoretically, this could be done by cross-validation. In practice, due to the significant computing costs that cross-validation implies, $K$ is chosen in an ad hoc fashion by the experimenter and rarely motivated by strong quantitative arguments (see Haselbach \emph{et al}\cite{Haselbach2018} for a rare example). %An alternative to cross-validation would be to leverage dimensionality reduction methods such as \threedva\cite{PUNJANI2021107702} where cross-validation of clustering results is much less expensive and can be used to determine a number of appropriate clusters. Such dimensionality reduction methods also enable the practitioner to visualize whether a continuous conformational heterogeneity would be more appropriate. 
%\paragraph{Continuous Conformational Heterogeneity: Pros and Cons.}

Consequently, many recent methods have turned to a continuous representation of heterogeneity which does not require specifying a number $K$ of conformations. This representation is also often deemed to be closer to the underlying biology, as molecules do not exist as finite/discrete sets of shapes. Rather, a more realistic analogy is to think of molecules as random samples from the equilibrium distribution over their conformational space\cite{dill2010molecular}. However, while a continuous representation could be more scientifically relevant, it remains to be determined how accurate the reconstruction of the conformational space by the space indexed by $z$ truly is. This latter point will be critical to address for heterogeneous reconstruction methods to become more quantitative and directly comparable to other measures from biophysicists and biochemists. We discuss in section \ref{sec3-discussion} the challenges of assessing the precision of such approaches, which probably constitutes one of the main open questions in the field. Additionally, despite its initial appeal, continuous conformation heterogeneity comes with significant theoretical and practical caveats. From a physics perspective, it is still unclear whether the full landscape (at room temperature) is sufficiently well sampled by cryo-EM to justify modeling conformations with a continuous rather than discrete distribution: the sample preparation process in cryo-EM --- and most specifically the grid-freezing step--- affects the distribution of conformations which might not reflect the heterogeneity of conformations at room temperature\cite{Bock2022}. From a statistical perspective, using a continuous distribution necessitates the generative model to be able to sample from the full conformation landscape, a requirement that is itself a considerable challenge for large molecules: the strong constraints, e.g. on on bond lengths and torsion angles, make up for a complex, non-convex landscape that is difficult to sample from. %This requires finding efficient ways of sampling conformations.
%--- thereby intersecting challenges in cryo-EM volume reconstruction with that in molecular dynamics, another dynamic open area of research where neural network approaches have also been deployed \cite{Noe2020}. 
Despite these caveats, Table~\ref{tab:volumes} shows that continuous heterogeneity is gaining traction amongst the most recent reconstruction advances.
    

\subsection{Molecular Volume $V(z)$}\label{definingV} 
The cryo-EM reconstruction problem can thus be understood as recovery of the underlying \gls{conformation landscape} $\mathcal{V}$ and the corresponding probability distribution. The next critical step thus consists in finding a judicious parametrization for each volume $V(z) \in \mathcal{V}$. This requires choosing first an ``output space'' (image space vs. Fourier space, inducing real vs complex values), second, an ``encoding style'' (reference-free vs. reference-based) and third, and ``input domain'' (continuous vs. discrete).

\subsubsection{Defining the output space: image space or Fourier space}
Equations~\eqref{eq:image}-\eqref{eq:fourier} show that the image formation model can be described equivalently in image space or Fourier space. Thus, each volume within the family of conformations $\mathcal{V}$ can be described either in terms of its pixel intensities or its Fourier coefficients. In either case, the volume $V(z)$ associated to the conformation variable $z$ is defined on an input domain $\Omega\subset\mathbb{R}^3$ (the space of coordinates) and outputs values in an output space that is either $\mathbb{R}$ for pixel intensities representing the electron scattering potential of the molecule, or $\mathbb{C}$ to encode the amplitude and phase of the Fourier coefficients. %We call the choice of $\mathbb{R}$ (image) or $\mathbb{C}$ the choice of the output domain, while the choice of $\Omega\subset\mathbb{R}^3$ will be described later as the choice of the input domain.

\paragraph{Image versus Fourier space: Pros, Cons and Discussion.}{
From a practical standpoint, the choice of the output space is guided by the set of properties and constraints that the analyst wishes to use to guide volume reconstruction. Historically, the Fourier approach has been preferred.
%due in part to the ease with which the slicing, rotation and translation operations can be performed
As summarized by Punjani \textit{et al.} \cite{Punjani2021}, working in Fourier space has the benefits of (a) reducing the computational cost of the image formation model (see discussion of Equation~\ref{eq:fourier}), and (b) allowing closed-form maximum likelihood reconstructions when molecules' orientations and positions are known. However, recent methods such as \threedflex have favored image space, where constraints (e.g. smoothness of the deformation, conservation of energy, etc.) are more interpretable and where operations such as interpolation and deformation of the molecule's density map are more naturally parametrized --- whereas the same operations require a careful treatment in Fourier space. For example, interpolation in Fourier space can introduce unwanted artifacts. As highlighted in Table \ref{tab:volumes}, image space computations constitute a promising and increasingly popular avenue for future developments in cryo-EM reconstruction.
}
 

\subsubsection{Defining an encoding: reference-free or reference-based volume}

The next step lies in the choice of an ``encoding" for the volume $V(z)$. Cryo-EM analysts typically have two choices: {\it (i) using a reference-based parametrization}, which encodes the conformation landscape through its deviation $\Delta V(z)$ from a reference conformation $V_0$, such that $V(z) = V_0 + \Delta V(z)$; or {\it (ii) using a reference-free parametrization} which directly describes each $V(z)$, for instance as a set of atomic coordinates or a low-dimensional embedding, but with no notion of ``reference'' conformation.  %From a practical standpoint, whether to choose a reference-free or reference-based method is guided by the number of unknown variables. In this section, we propose focusing on reference-based methods, which, when tackling conformation heterogeneity, seem to offer a sounder optimization program.

\paragraph{Reference-based versus reference-free: Pros, Cons and Discussion}
%This approach has the advantage of naturally biasing the representation of $V$ such that $\Delta V(z) = 0 $ implies $V(z) = V_0$, which in turn, can yield better conformations given the complexity of the problem. 
% This reference volume can be chosen from  existing data or information about the molecule --- obtained either through a first pass on the image data using a low resolution method or through  external prior knowledge on the shape of the molecule.
%Interestingly, there does not seem to be a strong preference for reference-free over reference-based methods, nor for refinement over ab-initio approaches. 
If the  column ``Reference Volume" of Table~\ref{tab:volumes} reflects the historical popularity of reference-free encodings, the most recent methods relying on deep-learning seem to have favored a reference-based approach. For instance, \egmm first learns a reference $V_0$ called the ``neutral representation" which then serves in a reference-based encoding of $V(z)$ to further refine the reconstruction by accounting for conformational variability. In \cryodeepmind, Rosenbaum \textit{et al.} uses a $V_0$ called a ``base conformation" described as a set of atom coordinates, obtained from an auxiliary method (such as an homogeneous reconstruction or a set of atom coordinates predicted by AlphaFold \cite{alquraishi2019alphafold}). The existing reference acts as a statistical prior on the molecular volume, thereby further constraining and guiding the recovery of the conformation landscape. By contrast, \threedflex uses a reference volume $V_0$, called a ``canonical density", which is learned jointly with the conformational heterogeneity. This has the advantage of foregoing the need to split the pipeline in sequential steps, while allowing to borrow strength from the joint estimation of all parameters. 

%Reference-based methods offer the advantage of further constraining the reconstruction of the 3D molecular volume, which can help the convergence of the algorithm. In fact, the volume $V_0$ can be either learned (ab initio methods), or chosen from existing data (refinement methods --- more on this in Appendix \ref{appA-abinitio-vs-refinement}). However, a potential drawback is that the conformation heterogeneity might become biased towards the reference $V_0$.
% The fact that no "reference-free" (or "reference-based") trend arises among current methods is interesting. 
Constraining the conformation recovery using a reference offers significant advantages for ensuring the success (and convergence) of these methods given the non-convexity of the problem. This template can be either learned (ab initio methods), or chosen from existing data (refinement methods --- more on this in Appendix \ref{appA-abinitio-vs-refinement}). The general agreement across all methods consists in tackling this hierarchically, starting with parameters which have the strongest impact on the signal, such as defocus or pose, and gradually focusing on those whose effect is more subtle, such as local deformations. As such, biasing the solution $V$ towards a reference $V_0$, such that $\Delta V(z) = 0 $ implies $V(z) = V_0$, can provide an interesting way of ensuring a more reliable and consistent --- but potentially biased --- solution. 
Depending on the optimization method used, this can in fact be critical to the success of the pipeline: Rosenbaum \textit{et al.}\cite{Rosenbaum2021} report that adopting a reference template and warm-starting their algorithm is indispensable to ensure the recovery of good conformations. However, because they fundamentally bias conformations $V(z)$ to ``hover'' around $V_0$, 
%(this is roughly a linearization of the conformation heterogeneity around a main "mode")
the success of such methods necessitates a reliable $V_0$. This can also incur higher computational costs, since such methods typically require running a first reconstruction method. This explains the interest for alternative, reference-free methods: three out of the six  heterogeneous methods in Table~\ref{tab:volumes} allow to recover molecular volumes without any  prior template. The extent to which these reference-free methods are likely to succeed on real-images still remains to be characterized.

%\paragraph{Reference-based ab-initio methods.} 
% In contrast, one finds referenced-based ab-initio methods, such as \threedflex which uses a reference volume $V_0$, called a ``canonical density" or ``canonical 3D map". However, there, $V_0$ is not supposed known, it is learned jointly with the conformational heterogeneity. These methods have the advantages of not requiring running several pipelines sequentially, and are potentially more amenable to borrow strength from the joint estimation of all parameters. 


%\paragraph{Theoretical justification} 
%  The underlying reason behind this strategic choice can be understood in terms of focusing the exploration of solutions as close to global minima as possible while increasing the complexity of the model being learned.






\subsubsection{Defining the input domain: discrete or continuous}
The volume $V(z)$ represents a scalar 3D field (electrostatic potential, or its Fourier transform) and is defined as a function from the input domain $\Omega\subset\mathbb{R}^3$ to an output space $\mathbb{R}$ (or $\mathbb{C}$). We now describe the parametrization of $\Omega$ and distinguish two cases, depending on whether the volume is defined as a discretized or as a continuous scalar field.

\paragraph{Discretized Domain and Explicit Parametrization.} The first class of approaches models the electrostatic potential as a discrete 3D map.
%: the reconstruction estimates the electrostatic potential at every location (or for any voxel) of a discretized 3D-space. 
In this case, the function $V(z)$ is defined on a discretized subspace (a grid) of $\mathbb{R}^3$, namely $\Omega=\{1,\ldots,D\}^3$, where $D$ represents the length of the 3D voxel grid or frequency grid. $V(z)$ is explicitly parametrized by the values it takes at each location (or voxel) of $\Omega$. This choice is also called an {\it explicit} parametrization, a term that will become clear in the next paragraph. Using a vectorial formalism, the vector $V(z)$ corresponds to voxels' intensity values, with $V(z)\in \mathbb{R}^{D^3}$ or $\in \mathbb{C}^{D^3}$. In this case, the resolution of the reconstructed volume is fixed by the choice of the granularity of the grid. However, the vectorial formalism would imply that $V(z)$ becomes an infinite-dimensional vector when it is represented continuously (see next paragraph). For this reason, we prefer to use a functional formalism and define the volume $V(z)$ as a function (not as a vector), whether it is modeled as a discrete or continuous field. Discrete domains are adopted by methods like \relion-Refine3D and \relion-Class3D\cite{Scheres2012ADetermination} --- which associate voxels with corresponding intensities in Fourier space ---, and like \cryoposenet or \threedflex in image space.% --- which target the reconstruction of the pixel intensity at each voxel.


\paragraph{Continuous Domain and Implicit Parametrization.} The second class of methods model the volume $V(z)$ as a continuous field, \textit{i.e.} as a function on a continuous domain ($\Omega=\mathbb{R}^3$ or $\Omega=[-0.5,0.5]^3$). The domain $\Omega$ is infinite, and one cannot explicitly maintain in memory the values that $V(z)$ takes on $\Omega$. The solution is then to adopt an explicit parametrization for $V(z)$ using parameters $\theta\in\Theta \in \mathbb{R}^p$.
%(with $\Theta$ is a finite-dimensional space $\mathbb{R}^p$ for some integer $p$). 
Depending on whether or not these parameters have a physical meaning (\textit{e.g.} centroids of pseudo-atoms), the function $V(z)$ can be encoded:
\vspace{1.2mm}
\begin{description}[noitemsep, leftmargin=0cm, topsep=0em,labelindent=0cm]
\item[(i) Using Neural Networks.] Some methods use neural networks to represent $V(z)$ as a (real or complex) function of a 3D position vector. The parametrization is called ``implicit" because the values of $V(z)$ are not stored in memory; instead, the practitioner can ``query" the neural network by inputing any location $x\in \mathbb{R}^3$ and receiving a value for $V(z)$ at $x$. In this case, the parameters $\theta$ --- \textit{i.e.} the weights of the neural network --- do not have a physical meaning. Examples of this approach include \cryodrgn and \cryoai, both operating in Fourier space using a reference-free volume encoding.
\vspace{1.2mm}

\item [(ii) Using Gaussian Mixtures.] Other approaches constrains the volume $V(z)$ by modeling the source of the electrostatic potential: its individual atoms or pseudo-atoms. Indeed, at a granular level, the molecular volume can be approximated by a mixture of $N$ Gaussian functions (called scattering form factors\cite{Kohl}) of the form:
\begin{equation}\label{eq:mixture}
    V_z(x) = \sum_{j=1}^N A_j \exp \left( - \frac{||c_j - x ||^2}{2\sigma_j^2}\right),
\end{equation}
where $x\in\mathbb{R}^3$ represents a 3D position, and $c_j \in \mathbb{R}^3$ are the 3D coordinates of the $N$ individual atoms or pseudo-atoms. The parameters $A_j \in \mathbb{R}$ and $\sigma^2_j \in \mathbb{R}$ describe how each (pseudo-)atom contributes to the electrostatic potential. In practice, these approaches always implement conformational heterogeneity, and do so through a continuous conformation variable $z\in \mathbb{R}^L$ that passes through a neural network to output $c_j$, and possibly $A_j$ and $\sigma^2_j$. This approach also models $V_z$ as a continuous field, as defined by Equation~\eqref{eq:mixture}, but the parameters defining each volume ($\theta=\{c_j, A_j, \sigma^2_j)\}_{j=1,...,J}$) now have a physical meaning. 
Among this general class of methods, works differ in whether $A_j, \sigma_j^2$ are assumed to be known, and in the interpretation given to the variable $c_j$. \egmm use a conformation variable $z$ that encodes the coefficients $c_j, A_j,\sigma_j^2$ and defines the $c_j$ as coordinates of ``coarse grained atoms" (reference-free). \cryofold assumes $A_j = A$ and $\sigma_j = \sigma$ known and fixed while using $c_j$ to represent ``groups of atoms''. \cryodeepmind also assumes $A_j = A$ and $\sigma_j = \sigma$ known and fixed, models the $c_j$ as the coordinates of the atoms, and uses the conformation variable $z$ to encode heterogeneous deviations $\Delta c_j.$% i.e. the deviation from a reference conformation of atoms (reference-based). More details are given in the supplementary materials.
\end{description}

\paragraph{Discretized and Continuous Domains: Pros, Cons and Discussion.} Contrary to the discretized domains, approaches using continuous domains potentially allow to achieve sharper, enhanced resolutions (within the Nyquist limit), as any coordinate of $\mathbb{R}^3$ can be fed to $V(z)$. Moreover, within continuous approaches, pseudo-atomic methods effectively add constraints to $V(z)$ by modeling it as a mixture of Gaussians, and even more so when assuming a reference conformation $V_0$. The increasing availability of folded protein shapes --- traditionally from the Protein Data Bank\cite{ROSE2021166704} and more recently through the advent of AlphaFold\cite{alquraishi2019alphafold} --- have indeed enabled access to relatively reliable atom coordinates of reference conformations $V_0$, that can enrich the recovery of the molecular volume. We also note that reference-based representation such as that proposed in  \cryodeepmind and \cryofold are more amenable to the inclusion of molecular dynamics information to the volume reconstruction process. 
%Perhaps expectedly, the authors of \cryodeepmind found that using a reference-based method with respect to some base conformation was critical: randomly initializing the atomic coordinates did not yield useful structures --- thereby highlighting  the crucial need for sensible initialization in these approaches.










% \subsection{Hidden and Known Variables}\label{hiddenvar}

% Functions can be parameterized described through sets of real parameters in $\mathbb{R}^p$, where $p$ is some integer value. In the case of cryo-EM, we denote as $\theta \in \Theta \subset \mathbb{R}^p$ the parameters associated with the function $V$, that takes as input the conformation variable $z$ and input domain coordinates $x \in \Omega$. Thus, the observed images $X_i$ are generated through another function $f_V$ of image-specific variables $H_i = (\text{PSF}_i, \sigma_i, t_i, R_i, z_i)$ and shared parameters ${\theta}$:
% \begin{equation}\label{eq:function}
%      X_i = f_V(H_i, \theta), \quad \text{for $i=1, ..., n$},
% \end{equation} 
% where, given a description of the conformational landscape $V$, $f_V$ is known and provided by Equations~\eqref{eq:image}-\eqref{eq:fourier}. The objective of this inference problem is thus to find the function $V$. 
 
% This would be a standard statistical problem, were it not for the fact that the variables $H_i= (\text{PSF}_i, \sigma_i, t_i, R_i, z_i)$ (\textit{i.e.} the covariates of the image) are unknown --- also called "hidden" or "latent" in statistical terminology. Thus, they will have to be filled in --- or ``imputed''. This yields a difficult and expensive statistical problem: the number of unknowns and variables increases with the size $n$ of the dataset, as for each particle image $X_i$, we need to (1) find the associated rotation $R_i$, translation $t_i$, $\text{PSF}_i$, $\sigma_i$ and conformation variable $z_i$ to (2) impute a description of the conformational landscape $V$.

% \paragraph{Specifying Hidden Variables}

% The statistical problem above describes an extreme version of the cryo-EM reconstruction task where the model in Equation~\eqref{eq:function} is completely agnostic: all latent variables in $H_i= (\text{PSF}_i, \sigma_i, t_i, R_i, z_i)$ are assumed to be unknown and have to be imputed simultaneously during reconstruction. In reality, it is very difficult to recover all variables in $H_i$ at once. Cryo-EM reconstruction methods vary according to the amount of information that is assumed known, \textit{i.e.} which latent covariates in $H_i$ are assumed to be given (which implies that they must be computed beforehand via an external algorithm), and which will need to be imputed during reconstruction. In fact, almost all the approaches presented in this review assume that the CTF (or PSF) has been estimated and is known; it is indeed possible to estimate the CTF independently from reconstructing the volume\cite{Rohou2015CTFFIND4:Micrographs}. The methods presented in this review subsequently differ in the latent variables that are effectively imputed: as shown in Table~\ref{tab:volumes}, some methods assume that the translation $t_i$ is known and focus on the problem of estimating specific conformation variable $z_i$ with associated $V(z_i)$, or vice versa. Section~\ref{sec2-inference} will further explain Table~\ref{tab:volumes} and present the inference methods that are used to impute the different latent variables in each approach.
%while Appendix~\ref{appA-relion-examples} gives specifics about these modeling choices in the cases of  \relion-Refine3D and \relion-Class3D.




==> CryoReview 2021 (6)/sec2-inference.tex <==
% Conventions:
% uppercase: random variable
% lowercase: value






%Section~\ref{sec1-generative_models_and_lvms} introduced the generative model for cryo-EM images, its possible parametrizations --- with an emphasis on the parametrizations of the biomolecular volume ---, and corresponding objective functions. 
We now turn to the description of the inference methods used in deep generative modeling for cryo-EM reconstruction. These methods recover the volume $V$ by finding optimal parameters $\theta$, conformation variables $z_i$ and nuisance variables $(\text{PSF}_i, t_i, R_i)$ of the generative model (Eq \ref{eq:image}). In this section, $\theta$ collectively denotes the parameters that describe the conformational landscape as a function of $z$, and the parameters of the function $V_{z}:x \to \Omega$ that associates a position $x$ to an output intensity. We refer to the conformation variable and poses jointly as the ``hidden variables'' and denote them as $H_i = (z_i, \text{PSF}_i, R_i, t_i)$.
%of the conformational landscape $V$ in the presence of nuisance variables. %Whether $V$ is defined on a discretized 3D grid or continuous 3D domain, we refer to the parameters associated with this function as $\theta$. 
For the sake of concision, this section focuses on general inference methods, and we reserve a description of their variations for Appendix~\ref{subsec:variations_EM}. % Instead, we attempt in our main text to give a critical perspective on these methods, highlighting potential hurdles and avenues for improvement.

\paragraph{Setting Up the Inference Problem: Observed Likelihood vs Full Likelihood} 
%Once the latent variables are specified, one can properly formalize the inference problem and specify an appropriate loss/objective function; The  optimization of the latter allows the recovery of the $\theta$. 
In the context of deep generative modelling for cryoEM, the cornerstone of inference is  simply the observed  likelihood $p_\theta(x) = p(x | \theta)$ associated with each image $x$. This likelihood is computed from the generative model in Equation~\eqref{eq:image} (or its Fourier counterpart -\eqref{eq:fourier}), which we seek to maximize as a function of $\theta$. However, the generative model depends on hidden variables $H_i=(\text{PSF}_i, t_i, R_i, z_i)$. In most cases, the optimization of the full likelihood of each observation $p(x_i, h_i, \theta)$ would be quite simple, if only the $H_i$ were observed. Thus, given $n$ observed images $x_1, ..., x_n$, one solution could be to jointly recover the parameters $\theta$ and hidden variables $H$ (considered here as fixed quantities, as opposed to random variables) that maximize the log-likelihood $\ell(X, \theta)= \sum_{i=1}^n\log(p_\theta(x_i, h_i))$. Mathematically, this requires solving the following optimization problem:
\begin{align}\label{eq:loglike}
\theta^{*}, H^{*} = \text{argmax}_{\theta, H}  \sum_{i=1}^n \log(p_\theta(x_i, h_i))
\end{align}

It is in fact a classical exercise in statistics to show that in this case, as the number of estimated variables grows with the number of data points, the estimate of $\theta$ is no longer guaranteed to converge to the real underlying value as $n$ goes to infinity ($\lim_{n\to \infty} \mathbb{E}[\theta^{*}] \neq \theta^{\text{true}} $). 
We thus have to resort to strategies that treat hidden variables as random variables, and that fit the parameters $\theta$ based on the ``observed likelihood'' $L(X, \theta)$. In this case, the objective becomes:
\begin{align}\label{eq:loglike}
\theta^* = \text{argmax}_{\theta} L(X, \theta) \quad \text{ where } \quad  
L(X, \theta)= \sum_{i=1}^n \log p(x_i| \theta) 
= \sum_{i=1}^n \log \int_{h_i} p(x_i, h_i|\theta) d\mu(h_i) 
%= \sum_{i=1}^n \log \int_{z_i} p(x_i|z_i, \theta) p(z_i |\theta)dz_i,
%\log p(\theta | X_i) &=\log \ell  + \log p(\theta)
\end{align}
where $d\mu(h)= p(h) dh$ is the probability measure associated to the hidden variables $H$.
%Methods with such an objective --- referred to as  maximum-likelihood (\acrshort{ml}) approaches --- view the parameters $\theta$ as unknown real values, as opposed to random variables. 
 However, this marginal likelihood requires an integral over all possible values of $H_i$. This quantity is difficult to compute directly, or in statistical terminology, ``intractable''. Consequently, the crux  of the optimization pipeline is to find a way to effectively approximate it.
 %, we only know $p_\theta(x_i, z_i)$.


\begin{figure}[h!]
\centering
    \includegraphics[width=.99\textwidth]{figs/em_lower_bound_cleaned_v2.pdf}
    %   \setlength{\belowcaptionskip}{-8pt} 
    %   \setlength{\abovecaptionskip}{-8pt} 
    \caption{Maximization of the log-likelihood $\theta \rightarrow L(X, \theta)$ in $\theta$ by maximizations of a series of lower bounds: $\mathcal{L}(q^{(0)}, X, \theta)$, $ \mathcal{L}(q^{(1)}, X, \theta)$, etc. The $\theta^{(t)}$s across iterations $t=0, 1, 2, ...$ are represented by colored dots and correspond to successive maxima of the lower bounds. Left: The lower bounds are tangent to $\theta \rightarrow L(X,  \theta)$, which is realized when $q$ is the posterior of the hidden variables. Right: The lower bounds are not tangent to $\theta \rightarrow L(X,  \theta)$, but show a ``gap" that corresponds to the KL divergence between $q$ and the posterior of the hidden variables, see Equation~\eqref{eq:KL}.}
    \label{fig:lb}
\end{figure}

\subsection{Unifying Inference Methods}

Since the observed log-likelihood $L(X,\theta)$ in the objectives of Equations~\eqref{eq:loglike}-\eqref{eq:logpost} is intractable, optimization is usually performed by targeting a proxy for $L(X, \theta)$, called the \acrfull{elbo}.
For the sake of clarity and concision, we highlight here the common statistical thread of cryo-EM reconstruction methods leveraging deep generative modeling, that all use an ELBO-based optimization and refer the reader to Appendix~\ref{appC-elbo} for further discussion on their variations.

\paragraph{Evidence Lower Bound (ELBO)} 
%The cryo-EM reconstruction inference methods do not directly target the maximization of the log-likelihood.
%The full likelihood $L(X, H, \theta)$ would be easier to optimize with respect to $\theta$, as its definition does not involve an integral, but it depends on hidden variables $H$ which are inaccessible.
The trick behind the  \acrfull{elbo}  consists in proposing a series of distributions $q^{(0)}, ...,q^{(t)}$ for the hidden variables $H$, and maximizing a series of ``easily'' computable lower-bounds $\mathcal{L}(q^{(0)}, X, \theta), ...,  \mathcal{L}(q^{(t)}, X, \theta)$ for $L(X,\theta)$ in an iterative fashion --- see Figure~\ref{fig:lb}. By iteratively maximizing these lower bounds with respect to $\theta$, the true likelihood $L(X, \theta)$ also increases.
%(that is, that $q$ is close to the actual distribution $p(h|x, \theta)$), 
The hope is that the value of $\theta$ obtained through their maximization 
%of these proxies
will be close to the value realizing the maximum of $L(X, \theta)$, if the lower bounds are tight enough --- \textit{i.e.} for small ``gaps" in Figure~\ref{fig:lb}.



The lower bounds $\mathcal{L}(q, X, \theta)$ are found by showing that, for any probability distribution $q_i$ on the variables $h_i$, the observed log-likelihood can be written as the sum of two terms (derivations provided in Appendix~\ref{appC-elbo}):
\begin{align}\label{eq:KL}
     L(X, \theta)  =  \mathcal{L}(q, X, \theta) + \sum_{i=1}^n \text{KL}(q_i(h_i) \parallel p_{\theta}(h_i|x_i))
     = \sum_{i=1}^n \Big[ \mathcal{L}_i(q_i, x_i, \theta) +  \text{KL}(q_i(h_i) \parallel p_{\theta}(h_i|x_i)) \Big]
\end{align}
where
%  = \int_{z_i} q(z_i) \log\left(\frac{\log p(x_i, z_i| \theta)}{q(z_i)}\right)d_zi\\
%  = \int_{z_i} \log p(x_i, z_i| \theta)q(z_i) dz_i -\int_{z_i} q(z_i)\log q(z_i) dz_i
%  =  \int_{z_i} \log p(x_i, z_i| \theta)q(z_i) dz_i + H(q)
    %  & = \log L(X, \theta) - KL(q \parallel p(z|x, \theta)) \\
    %  &= \int_z \log p(x, z| \theta)q(z|x) dz  + H(q) \\
$KL$ is the \acrfull{kl} defined as $KL(q \parallel p)=\int  q(x) \log \frac{q(x)}{p(x)} dx$, and the terms $\mathcal{L}_i$ write:
\begin{equation}\label{eq:elbo}
\mathcal{L}_i(q_i,x_i, \theta) 
 =  \int_{h_i} q_i(h_i) \log p_\theta(x_i|h_i) dh_i - \text{KL} \left( q_i(h_i) \parallel p_\theta(h_i) \right). 
%  = \int_{h_i}  q_i(h_i) \log p_\theta(x_i, h_i) dh_i - \int_{h_i}  q_i(h_i) \log q_i(h_i) dh_i.
\end{equation}

%We observe that the KL divergence in Equation~\eqref{eq:KL} differs from the KL divergence in Equation~\eqref{eq:elbo}.
The divergences $\text{KL}(q(h_i) \parallel p_\theta(h_i|x_i))$ in Equation~\eqref{eq:KL} are always non-negative. Thus, for any joint distribution $q=\{q_i\}_{i=1\cdot n}$, the function $\mathcal{L}(q,X, \theta)$ provides a valid lower-bound to $L(X, \theta)$ (see Figure~\ref{fig:lb}), called the Evidence Lower Bound (ELBO):
$$ \forall q,\forall \theta, \quad  \mathcal{L}(q,X, \theta) \leq L(X, \theta). $$

The lower-bounds $\mathcal{L}(q^{(t)},X, \theta)$ are proxies for $L(X, \theta)$, that  - in contrast to $L(X, \theta)$ - can be computed and maximized in $\theta$.
% ELBO-based inference methods iteratively maximize the ELBO $\mathcal{L}(q,X, \theta)$ in $\theta$ by refining the distributions $q_i^{(t)}$ at each iteration $t$ until convergence of the ${\theta}^{(t)}$ provides a series of computable lower bounds to the log-likelihood that, in turn, allows to optimize $\theta$.

% \begin{figure}
%  \vspace*{-0.3in}
%  \centering
%     \includegraphics[width=0.4\textwidth]{figs/posterior_distributions.pdf}
%     %  \setlength{\belowcaptionskip}{-4pt} 
%     %   \setlength{\abovecaptionskip}{-4pt} 
%     \caption{Possible choices for the distribution $q$ on the hidden variables $h$, where we have dropped the indices $i$ for convenience of notations. The choice of $q$ determines the lower bounds to $L(X, \theta)$ in Figure~\ref{fig:lb}. The inference methods used in cryoEM reconstruction can be contrasted by the choice of $q$: as the true posterior $p_\theta(h|x)$ represented by the green line, as the Dirac distribution $\delta(h)$ represented by the vertical dashed gray line or as a distribution within a known parameterized family $\mathcal{Q}$, such as the family of Gaussian distributions, represented by the brown dashed line.}
%     \label{fig:posterior_distributions}  \vspace*{-0.18in}
% \end{figure}

% \begin{wrapfigure}{r}{0.4\textwidth}
%  \vspace*{-0.3in}
%     \includegraphics[width=0.4\textwidth]{figs/posterior_distributions.pdf}
%     %  \setlength{\belowcaptionskip}{-4pt} 
%     %   \setlength{\abovecaptionskip}{-4pt} 
%     \caption{Possible choices for the distribution $q$ on the hidden variables $h$, where we have dropped the indices $i$ for convenience of notations. The choice of $q$ determines the lower bounds to $L(X, \theta)$ in Figure~\ref{fig:lb}. The inference methods used in cryoEM reconstruction can be contrasted by the choice of $q$: as the true posterior $p_\theta(h|x)$ represented by the green line, as the Dirac distribution $\delta(h)$ represented by the vertical dashed gray line or as a distribution within a known parameterized family $\mathcal{Q}$, such as the family of Gaussian distributions, represented by the brown dashed line.}
%     \label{fig:posterior_distributions}  \vspace*{-0.18in}
% \end{wrapfigure}

\paragraph{Inference Methods Based on an ELBO.}  While the ELBO holds for any $q$, some choices are more judicious than others. In fact, the goal is to select an optimal $q$, such that the gap between $\mathcal{L}(q,X, \theta) \leq L(X, \theta)$ is small: this will insure that the maximization of $\mathcal{L}(q,X, \theta)$ with respect to $\theta$ yields estimates $\theta^*$ that are also appropriate (and close to the true optimum ${\theta}^{\text{true}}$) for maximizing $L(X, \theta)$ --- see Figure~\ref{fig:lb} (right). Inference methods in cryo-EM subsequently differ in the choices of the distributions $q_i^{(t)}$ for each $i$ and at each iteration $t$, thereby yielding different lower bounds $\mathcal{L}(q,X, \theta)$: %The gap between $L(X, \theta)$ and the ELBO $\mathcal{L}(q, X, \theta)$
    %in the inequality:
    %$$\mathcal{L}_i(q, X, \theta) \leq L_i(X, \theta),$$
% is $\text{KL} \left( q_i(h_i) \parallel p_\theta(h_i | x_i)\right)$ and is in fact a function of $q_i$ which we wish to minimize --- see Figure~\ref{fig:lb} (right). The challenge of these methods thus consists in  finding the ``best proxies'' $q_i$ for the unknown posteriors $p_{\theta^{(t)}}(h_i|x_i)$ that make this gap as tight as possible while allowing a sound and efficient optimization of  the parameters $\theta$:

\begin{description}[noitemsep, leftmargin=0cm, topsep=0.05cm,labelindent=0cm]
\item [\bf (i) Using the posteriors given current parameters (EM algorithm):] Computing the posteriors $p_{\theta}(h_i|x_i)$ using the current estimated value $\theta^{(t)}$ of $\theta$ allows choosing $q_i^{(t)}(h_i) = p_{\theta^{(t)}}(h_i|x_i)$ for each $i$ at iteration $t$ --- see Figure~\ref{fig:posterior_distributions}. The inequality: 
    $$\mathcal{L}_i(p_{\theta^{(t)}}(h_i|x_i), X, \theta) \leq L_i(X, \theta),$$
becomes an equality for $\theta^{(t)} = \theta$. This makes the lower-bound $ \mathcal{L}(q, X, \theta)$ tangent to $L(X, \theta)$ at $\theta = \theta^{(t)}$: progressively \\
maximizing $\mathcal{L}(q, X, \theta)$ with respect to $\theta$ will induce convergence to a local maximum of $L(X, \theta)$ in $\theta$, as seen in Figure~\ref{fig:lb} (left). This is the strategy adopted by \acrfull{em} algorithm (more details in Appendix~\ref{appC-elbo}). The EM is an iterative algorithm which consists of two steps. In the first step (called the expectation step), given current parameters values $\theta^{(t)}$, we compute the posterior $q_i^{(t)}(h_i) = p_{\theta^{(t)}}(h_i|x_i)$  to plug into our ELBO. In the second (the maximization step), $\theta^{(t+1)}$ is taken to be the value of $\theta$ that maximizes the ELBO. This sequence of two steps is usually repeated until convergence. Cryo-EM methods adopting this approach are given in the first column of Table~\ref{tab:inference}. As explained in Appendix~\ref{appC-elbo}, while the EM algorithm does not have any convergence guarantees, it nonetheless guarantees to increase the likehood at each step.

\item [(ii) Approximating the posteriors given current parameters (Variational EM algorithm):] In certain cases, the choice of $q_i^{(t)}(h_i)$ as the posterior $p_{\theta^{(t)}}(h_i|x_i)$ is neither computationally attractive nor feasible. In this case, we might prefer approximating each posterior by finding its ``best approximation'' $q_i^*$ within a family of functions called variational family $\mathcal{Q}$. Cryo-EM reconstruction methods consider two choices that include approximating the posteriors by {\it (i) their ``mode", i.e. the value $\hat h_i$ of $h_i$ that maximizes $p_{\hat{\theta}^{(t)}}(x, h)$}. In this case, each $q_i$ effectively becomes a Dirac distribution at $\hat h_i$; or {\it (ii) or a general distribution $q_i$ within a family $\mathcal{Q}$}: $q_i$ is for example a Gaussian distribution -- see Figure~\ref{fig:posterior_distributions}. Cryo-EM methods adopting this approach are given in the last two columns of Table~\ref{tab:inference}, within the ``non-amortized" subcolumns.

    %--- not necessarily restricted to the family of the posteriors $p_{\theta^t}(h|x)$.
    %  Approximations (i) and (ii) are the focus of Subsections~\ref{subsec:mem} and \ref{subsec:vem} respectively in Appendix~\ref{appC-elbo}, and the last two columns of Table~\ref{tab:inference}.
\end{description}


\paragraph{Exact or Approximate Posteriors: Pros, Cons, Discussion.} The EM algorithm, that uses exact posteriors, holds several advantages: it is simple and stable, since all updates can only improve the observed log-likelihood. However, it is also potentially slow: the rate of convergence is known to be linear with rate proportional to the fraction of information about $\theta$ in $L(\theta, X)$ \cite{Dempster1977MaximumAlgorithm}. Variational EM algorithms can be faster; yet they potentially loose in accuracy as their ELBOs do not provide tight lower-bounds to the log-likehood $L(X, \theta)$ (Figure~\ref{fig:lb}, right). As a result, we do not have any guarantee that they converge to an (even local) maximum of $L(X, \theta)$.






\subsection{Introducing Amortized Inference}

\begin{figure}[h!]
\centering
    \includegraphics[width=0.9\textwidth]{figs/generative_framework.png}
    % \setlength{\belowcaptionskip}{-8pt} 
    % \setlength{\abovecaptionskip}{-28pt} 
    \caption{\textbf{Comparison of generative reconstruction methods.} Volume represented in image space (resp. Fourier space) are outlined in blue (resp. orange). CryoDRGN\cite{zhong2021cryodrgn} is similar to cryoDRGN2\cite{zhong2021cryodrgn2}, except rotations and translations are given by an upstream homogeneous reconstruction. CryoVAEGAN\cite{MiolanePoitevin2020CVPR} does not explicitly store a representation of the volume and therefore does not appear in the figure. VG = Voxel Grid ; NN = Neural Network ; GM = Gaussian Mixture.}
    \label{fig:vae}
\end{figure}

%The variational inference methods described above are ``non-amortized", in contrast to the amortized variational inference methods that we present now. While non-amortized variational inference can lead precise inference on the latent variables, amortized variational inference offers the opportunity to provide methods with enhanced computational efficiency.

While potentially more computationally attractive than the original EM algorithm, Variational EM requires solving $n$ optimization problems to find an approximate posterior $q_i$ 
%for each hidden variable in $h_i = (R_i, t_i, \text{PSF}_i, z_i)$, and 
for each image $i$ in $1, ..., n$. This is computationally expensive, as the number of $q_i$ to estimate increases as the number of images $n$ increases. 
%As a result, recent methods rely on \acrfull{ai}  the E-step, either within the modal EM of Subsection~\ref{subsec:mem}, or within the variational EM of Subsection~\ref{subsec:vem}. 
%The M-step is still unchanged, and can be used as a MLE or MAP estimation.
%In the case of RELION for instance, the number of Fourier coefficients quickly explodes with (a) the resolution that has to be achieved, and (b) the number of images.  
%Moreover, inference can be slow, and this is not amenable to more complex models, such as the ones including conformation heterogeneity, which, if modeled, typically makes the posterior intractable.
Consequently, recent methods have resorted to using an additional approximation called \acrfull{ai}, which collapses the $n$ optimizations problems into one. Instead of finding the best corresponding  $q^*_i$ for each $i$
%$\hat h_i$  (in modal EM) or $\eta_i$ defining $q_{\eta_i}$ (in variational EM)
, AI optimizes the parameters $\xi$ of a function $\text{Enc}_\xi$ that predicts the parameters of the distribution $q_i^*(h_i)$ when given $x_i$ as input, i.e.: $\text{Enc}_\xi(x_i) \simeq ( \mathbb{E}[h_i], \text{Var}[h_i]))$, where, in this example,  the variational family $\mathcal{Q}$ is chosen to be the set of Gaussian distributions.
%or $\text{Enc}_\xi(x_i) \simeq \eta_i$. 
In other words,instead of solving $n$ separate problems, Amortized Inference predicts the parameters of the posterior of image $i$ using the observed image as input. The function $\text{Enc}_{\xi}$ is traditionally called an encoder. More details --- including a description of updates performed in AI --- can be found in Appendix~\ref{appC-elbo}. Cryo-EM methods using this approach are shown in the ``amortized" subcolumns of Table~\ref{tab:inference}.


%The traditional inference of $p_\theta(h_i | x_i)$, i.e. learning a distribution close to $p_\theta(h_i | x_i)$ for each $i$, is replaced by a simpler problem: learning a prediction model $x_i \rightarrow \text{Enc}_\xi(x_i) \simeq p_\theta(h_i | x_i) $ where the parameter $\xi$ is shared among the $i$'s. 
% \paragraph{Amortized Modal EM as dual optimization algorithm} AI in the E-step of the Modal EM gives rise to an amortized modal EM, with two steps at each iteration $(t)$:
% \begin{description}
%   \item[(a) Inference on latent variables $h_i$] The parameters $\xi$ parametrizing the encoder is computed via:
%   \begin{equation}
%       \xi^{(t)} = \argmin_\xi \sum_{i=1}^n ||f_{V_\theta}(\text{Enc}_\xi(x_i)) - x_i||^2,
%   \end{equation}
%   \item[(b) Maximization on model's parameter $\theta$] The parameter $\theta$ is updated via:
%   \begin{equation}
%       \theta^{(t)} = \argmax_\theta \mathcal{L}(q_{\eta_i}^{(t)}, \theta).
%   \end{equation}
%  \end{description}
% The optimization alternates between optimizing over $\xi$ and optimizing over $\theta$, thus being an instance of a dual ascent algorithm.


% \paragraph{Amortized Variational EM as Dual Optimization Algorithm} AI in the E-step of variational EM leads to an amortized variational EM:
% \begin{description}
%   \item[(a) Inference on hidden variables $h_i$] The parameters $\xi$ parametrizing the encoder is computed via:
%   \begin{equation}
%       \xi^{(t)} = \argmax_\xi \sum_{i=1}^n KL(q_{\text{Enc}_\xi(x_i)}||p_{\theta^{(t-1)}}(h_i|x_i)
%   \end{equation}
%   which generates $n$ distributions $q_{\eta_i}^{(t)}$ parametrized by $\eta_i = \text{Enc}_{\xi^{(t)}}(x_i)$.
%   \item[(b) Maximization on model's parameter $\theta$] The parameter $\theta$ is updated via:
%   \begin{equation}
%       \theta^{(t)} = \argmax_\theta \mathcal{L}(q_{\eta_i}^{(t)}, \theta).
%   \end{equation}
%  \end{description}
% The optimization alternates between optimizing over $\xi$ and optimizing over $\theta$, thus being an instance of a dual ascent algorithm.

% The variational inference problem is an optimization problem that maximizes a proxy of the likelihood, or a proxy of the posterior distribution of the parameters, called the ELBO and defined as:
% \begin{align*}
% ELBO &=  \log \ell  - KL(q_\phi||p(h_i|X_i)) \\ 
% ELBO^{MAP} &=  ELBO  + \log p(\theta)
% \end{align*}
% to be optimized over $\theta$(or over the parameters of the posterior of $\theta$) and over the parameters $\phi$ defining the function predicting $q_i$. 

% Such amortized variational inference methods hold several advantages over the variational EM algorithms. They provide faster inference, on a larger set of problems, due to the information compression that is achieved by $z$, and due to the fact that $n$ optimizations are replaced by 1 optimization in step (a).

% In the EM and variational EM algorithms, as well as in their amortized versions, the optimization yielding the posterior $q_i$ can be conducted fully at each iteration, or only partially by taking a gradient step--- see the difference between ``EM" and ``gradient EM" methods in Appendix~\ref{appC-elbo}. In the case of amortized inference, we call these methods amortized (variational) EM and amortized (variational) gradient EM respectively. The main uses of amortized variational gradient EM in cryo-EM come in the form of (variational) autoencoders, which we describe next.\\


% \paragraph{Full versus gradient and (variational) autoencoders}  If the optimization is not fully performed at each iteration, but only a gradient step is taken, we have a gradient amortized variational EM, also called an autoencoder when the variational family is a variational family of delta distributions, and a variational autoencoder when the variational family is a family of Gaussian distributions. We can see it as a gradient ascent of the cost function ELBO, in the coordinates $\phi$ and $\theta$.




% Yet, contrary to explicit Bayesian model, the solution here implicitly captures the information: without post-processing procedures, it is impossible to attribute any specific coefficient of $z$ to any of the hidden variables. Consequently, \textbf{one of the challenges of cryo-EM reconstruction lies in our ability to disentangle pose from heterogeneity and volume in latent space}. This explains both the difficulty of the task, and why there exists so many different approaches to the problem. 





%This subsection details the architectures of autoencoders and variational autoencoders that have been used in the Cryo-EM literature, and complements the previous subsections by adding considerations related to the losses that emerge from the optimization steps (a)-(b).
\paragraph{Implementation of Amortized Inference with Variational Autoencoders} In cryo-EM reconstruction, amortized inference is deployed in the context of variational autoencoders, denoted VAEs. VAEs are deep architectures that model the parameters of the variational family $\text{Enc}_\xi$ described above as a neural network with weights $\xi$ --- therefore leveraging the expressivity of this class of functions to get an optimal (amortized) variational approximation. The entire VAE pipeline thus consists of two steps: an encoder, which is simply a neural network with weights $\xi$ corresponding to the function $\text{Enc}_\xi$ described above, and a decoder, which allows to create ``mock samples'' that will then be compared with the observed ones based the generative model with parameter $\theta$ chosen in Section~\ref{sec1-generative_models_and_lvms}. Here, the decoder is almost entirely dictated by the process described in Equation\ref{eq:image} and goes beyond the conventional fully connected networks or convolutional neural networks used in image processing.

%that learns to map inputs to distributions
% %(in the non-variational ``AE'' version) 
% by leveraging amortized inference. In other words, the family $\mathcal{Q}$ consists of the set of distributions parameterized by% to reduce input data to an approximation of their latent variables.
% %(in their variational ``VAE'' version). 
%  an encoder and a decoder: 
% That is, the aim is to find an encoder that efficiently encodes all the information in the image necessary for the recovery of the image by the decoder: 
%Another way of going about is to use embeddings that implicitly encore the shape and volume of the biomolecule of interest. In this case, each coefficient of the embedding is not necessarily interpretable, but implicitly encode a parametrization of the problem.

% \begin{description}[noitemsep, leftmargin=0cm, topsep=0.05cm,labelindent=0cm]
% \item[(a) Encoder - Inference on hidden variables $h_i$] The encoder takes an image $x_i$ as input, and outputs the parameters (for instance, its mean and variance) for the best approximation to $p(h_i|x_i, \theta)$.% that allows to sample a low-dimension representation of the image . 
% The function $\text{Enc}_\xi$ is a neural network with weights $\xi$, such that $h_i \sim q_{\text{Enc}_\xi(x_i)}$.
% %Practically, this encoding/approximation is achieved (typically) through a neural network (called the encoder). 
%  %The encoder (ie, the neural network) has weights $\phi$ and maps an input $x_i$ to variable $z$, so that $z = \mathcal{E}nc_{\phi}(x_i)$. 
%  \item[(b) Decoder - Estimation of model's parameter $\theta$] The decoder takes as input a sample from this distribution and outputs a reconstructed image $\hat x_i$ of the original image $x_i$. %Note that, ``image reconstruction" refers to the reconstruction of the original 2D image, and not of the molecular volume. The volume is reconstructed by recovering parameters and variables of the deep generative model. 
%  The decoder is therefore a function $\text{Dec}_\theta$ such that: $\hat{x}_i = \text{Dec}_\theta(h_i)$, that is traditionally encoded by neural network with weights $\theta$. In cryo-EM, the architecture of the decoder can be guided by the image formation model in Equations~\eqref{eq:image}-\eqref{eq:fourier}, and therefore consists of a tailored architecture that goes beyond the conventional fully connected networks or convolutional neural networks used in image processing.
% \begin{itemize}
%     \item An component that describe how information in the latent variable $z$ is linked to the volume $V$.
%     \item A projection operator, that is able to take the reconstructed volume, and map it to the observed image. Note that this requires the disentanglement of the pose (rotation, translation), volume and potentially, heterogeneity parameters --- which is not automatically assumed by the latent space model.
%     %This is where it gets tricky. We need to be able to disentangle the pose and conformation:
%     % \begin{itemize}
%     %     \item In Fourier space, 2D projection images can be related to volumes as 2D central slices in 2D space. Thus given a smaple from $q_{\xi}(z|X) $, an estimate of the a rotation and shift parameter an image can be reconstructed by the decoder. This image has to be translated by the image's in-plane shift and multiplied by the CTF before it is compared to the input image.
%     % \end{itemize}
% \end{itemize}
% \end{description}
The learnable parameters $\xi$ and $\theta$ of the encoder and the decoder are fitted through stochastic gradient descent via backpropagation of the  ELBO  through the neural network. Compared to traditional cryo-EM reconstruction methods leveraging the EM algorithm, variational Autoencoders can be interpreted as extending the E-step (encoder) and the M-step (decoder) of the EM algorithm. The VAE architectures of cryo-EM reconstruction methods using amortized inference are given in Figure~\ref{fig:vae}. In this review, we have also included for comparison purposes a non-variational version of this procedure (the  \threedflex auto-encoder). Here, the authors consider the hidden variables as non-random variables, but add a fix amount of gaussian noise to regularise the embeddings. While the final loss is therefore adapted, this is essentially a VAE where the variance is fixed, while only the mean is learned.  % which also respectively perform inference on the hidden variables (E-step) and estimation of parameters (M-step).

% We note that (variational) autoencoders perform minimizations, as opposed to maximizations, since deep learning methods traditionally minimize a loss function that represents an equivalent of the negative log-likelihood or the negative ELBO. We detail the optimization procedures of the auto-encoder and variational autoencoder in the supplementary materials.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\textwidth]{figs/comp_vae_em.png}
%     \caption{Caption}
%     \label{fig:comp_vae_em}
% \end{figure}

\paragraph{Amortized Inference: Pros, Cons, Discussion} Amortized inference is faster than its non-amortized counterparts, but adds an additional error (called the amortization error). We observe that several methods use amortized inference, but often to estimate one hidden variable: e.g. only the rotation $R$ or only the conformation variable $z$. Table~\ref{tab:inference} classifies the reconstruction methods by the type of inference chosen for each variable within $h_i= (R_i, t_i, \text{PSF}_i, z_i)$ and indeed, we note that this choice does not have to be consistent across all hidden variables. Many methods ``mix and match'' inference techniques, using for example a variational EM for the hidden rotation variable $R_i$ and a VAE for the conformation variable $z_i$. 
%Researchers effectively choose which parameters or latent variables are assumed to be known, which will be estimated, and if so with which inference methods.
Moreover, it becomes apparent from Table~\ref{tab:inference} that (variational) autoencoders are the most common type of approaches implemented for cryo-EM reconstruction. 
%They have allowed researchers to model the variability of biomolecular shapes (conformation heterogeneity) using a \textit{continuous} latent variable representing the shape, as opposed to the \textit{discrete} latent variables \textit{representing discrete states or conformation clusters}, as it was usually done before 2020. 

While deep generative methods for cryo-EM volume reconstruction can be unified with the framework described above (as well as with traditional Expectation Maximization approaches), we observe that each of them has its own specificities or ``implementation tricks". They differ, for example, in their choice of variational family, or loss function that adapts the ELBO to facilitate convergence of the optimization procedure, see Appendix~\ref{appC-elbo}. These testify to the difficulties encountered in training these algorithms in the context of cryo-EM images with low signal-noise ratios.%, as well as to the complexity of comparing them --- as detailed in the next Section. 



% \paragraph{Inference methods: Pros, Cons, and Discussion} We observe that most methods actually do not strictly follow the original optimization method of the VAE, but supplement it with a wide range of additional losses or modifications --- that the respective authors present as necessary for convergence of their models at training time. These testify to the difficulties encountered in training these algorithms in the context of cryo-EM images with low signal-noise ratios, as well as to the complexity of comparing them --- as detailed in the next Section. Additionally, performing a principled comparison of their results becomes a hard task. 



% We also note that EM and amortized inference are but two popular methods to perform inference among a variety of options. Inference could also be performed using other techniques. Recent works have for instance resorted to the use of Generative Adversarial Networks (Appendix~\ref{appC-elbo}, section~\ref{subsec:gans}) and auto-encoders, for which we provide a brief description in the appendix.

% In this sense, methods differ by how much they want to work towards the end-to-end goal (that is, assuming less and trying to infer more), versus how much they want to specialise and enhance a specific component of the pipeline (e.g, for the purpose of this review, volume estimation, or heterogeneity modeling).

% We also note that, due to the volume of the data in cryo-EM, exact Bayesian inference procedures --- such as Gibbs sampling\cite{Gelfand1990} or Hamiltonian Monte Carlo\cite{Duane1987} --- cannot be deployed because of computational constraints. Cryo-EM reconstruction methods thus have to use the scalable inference schemes described in this review, that possibly approximate in the sense that they often approximate the true posterior of the hidden variables by another distribution $q$.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


==> CryoReview 2021 (6)/sec3-discussion.tex <==

%Deep-generative models for cryo-EM reconstruction offer a variety of options and alternatives, both in the parametrization of the problem that they adopt, as well as in the type of ELBO that they use as part of the optimization procedure. 
Given the wide number of options to reconstruct molecular volumes from cryo-EM images, it is natural to ask: \textit{which reconstruction method is in fact the most promising?} In this last section, we focus on the need for establishing a set of metrics and benchmark tasks that can be used to quantitatively compare the performance of these methods. Starting with a review of the tools currently available, the first take-away of this section is the urgent need for new metrics and benchmarks. The evaluation of these methods' performance is currently difficult and inherently limited. We nonetheless highlight, as a second take-away, promising features in current developments, which, in our opinion, these developments pave the way for future improvements in cryo-EM reconstruction.

\subsection{Assessing Reconstruction Performances: Need for New Metrics}

Performance metrics can be categorized in two classes: (a) those that assess a method's ability to provide good \textbf{spatial resolution} (i.e. distinguishing different atoms), and, in the case of heterogeneous methods, (b) those that assess a method's ability to provide good  \textbf{conformation resolution} (i.e. distinguishing different conformations). %We show that existing metrics are unsuited to properly quantify performances of the new reconstruction methods presented in this review.


\subsubsection{Assessing Spatial Resolution} 
%Evaluation of the quality of a spatial reconstruction depends on the choice made to represent the volume (see Section \ref{definingV}).

\paragraph{Resolution of discretized reconstructions (3D maps). } When the reconstructed volume is parametrized as an explicit 3D map, the most widespread measure used to evaluate its spatial resolution is the \acrfull{fsc}\cite{haraus1986}. As described by Singer \textit{et al.}\cite{singer2020computational}, this quantity measures the correlation over a 3D shell between two reconstructed volumes:
\begin{align}\label{eq:fsc}
    FSC_k(U,V)= \frac{\sum_{s \in S_k}U_sV_s^*}{\sqrt{\sum_{s \in S_k} |U_s|^2 \sum_{s \in S_k} |V_s|^2} }.
\end{align} 
Here, $S_k$ is the set of Fourier voxels in a spherical shell at distance $k$ from the origin, and
$U$ and $V$ are the Fourier transforms of the 3D volumes that we compare. Typically, $U$ and $V$ correspond to two independent reconstructions on separate halves of the dataset, in which case, the criterion for a method to be deemed to perform well is for the two reconstructed volumes to be similar. The method's resolution is then defined as the highest resolution for which $U$ and $V$ agree ``enough''. This is precisely what the FSC (Equation \ref{eq:fsc}) captures: the FSC is close to 1 when the two maps are close. This is usually the case for small $k$, as low-frequency signal is strong, but the FSC generally decays to zero as the signal-to-noise decreases. The result is often plotted as a curve, with axis $x=k$. The resolution of the reconstruction corresponds to the maximum value of $k$ such that $FSC_k \geq 0.143$ --- a criterion chosen to match resolution criteria used in X-ray crystallography\cite{VANHEEL2005250}. For synthetic datasets where a ground-truth volume is available, the FSC is measured between the reconstruction and the ground-truth; in which case the resolution criterion correspond to the maximum value of $k$ such that $FSC_k \geq 0.5$. %Theoretically, for a dataset of images of size $D \times D$, the reconstructed 3D map will be a cube of size $D\times D\times D$ voxels per side, of same physical length $l$\todo{I don't understand what l is} as the pixels and the maximum achievable resolution will be $k^{-1} = 2 l$ --- the so-called \emph{Nyquist limit}.

\paragraph{Resolution of continuous reconstructions. } %Most methods that  represent the volume as as a continuous field, rather than a discrete grid typically recover heterogeneous conformations. This means that the spatial resolution needs to be evaluated on an ensemble, not just one reconstructed volume (see next subsection). 
Methods that represent the volume as a continuous field are relatively new, and it might be worth reassessing appropriate metrics for evaluating spatial accuracy in this case. 
%While such methods are typically evaluated by sampling along a grid (as in \cryodrgn) to compute the FSC, a natural question arise: what should be the resolution of the chosen grid, and should it match the resolution of the image discretized domain? We argue here that these methods calls for new metrics quantifying spatial accuracy:
\begin{description}[noitemsep, leftmargin=0.cm, topsep=0.05cm,labelindent=0cm]
\item[(i) Implicit Parametrizations] 
%For methods that use an implicit volume parametrization (e.g., through an neural network), a simple solution is again to resample one reconstructed (continuous) volume on a discrete grid (as in \cryodrgn) and use the FSC measure just described. 
While interpolation between image pixels and map voxels is necessary in the discrete case, both for projection and for backprojection, implicit representations of the volume (e.g., through an neural network) enable sampling without interpolation during training. It would be interesting to investigate whether this provides a benefit in terms of reconstruction quality. We do not expect implicit representations to suddenly \emph{unlock} information, since the information content is determined by the discrete nature of the images and their pixel size, but they might provide new actionable ways to implement prior informations about the volume, such as smoothness and stereochemistry, that would result in reconstructions of higher quality.
%offer an opportunity to revisit our definition of spatial resolution\cite{VANHEEL2005250}. Consider the Fourier volume that is learned during the reconstruction step. Each image in the dataset, once oriented and centered, provides a set of $D\times D$ values along a central plane of the Fourier volume. When the dataset is considered as a whole, the density of experimentally sampled positions will be denser at the origin than it will be at the periphery of the volume. As a result, the statistical error made on the predicted value of the volume should increase with the resolution, thereby possibly providing a proxy for the spatial resolution. However, there is not yet an established metric to compare continuous fields.
\item[(ii) Atomic Parametrizations] Parametrizations of the volume with atomic models represents an opportunity to revisit the notion of spatial resolution. The traditional measure of similarity between two atomic models that only differ in the cartesian coordinates $U$ and $V$ of their $N$ constituting atoms (using a consistent orientation of the molecule for $U$ and $V$) is the \acrfull{rmsd}. This quantity is defined as:
\begin{align}\label{eq:rmsd}
 RMSD(U,V) = \sqrt{\frac{1}{N}\sum_{i=1}^{N}|U_i-V_i|^2},
 \end{align}
%  \todo{Actually, would we use the RMSD? Or the Gromov distance between positions? Maybe the overall position does not matter, since it should be invariant to rotations, and we should rather talk about methods for comparing point cloud data,}
%The scientific community developing methods for simulating and analyzing molecular dynamics simulations ran into the same issue of having to develop metrics for comparing atomic models, and they also used the RMSD initially. 
However, it was soon recognized that this metric had a very narrow range for interpretability \cite{kufareva2011methods}: it is a global measure of similarity, which is not suited to capture the local --- but meaningful--- changes in protein structure. To complicate the matter, measuring the RMSD between two atomic models assumes that they are both in the same reference frame, which might not always be defined. 
To improve the sensitivity of the metric, atomic models are routinely reduced to features with desired properties, e.g. vectors of internal coordinates independent of the reference frames. For example, reducing the atomic model to its backbone dihedral angles or to a list of atomic contacts has been shown to yield better clustering of conformations \cite{scherer2019variational}.  The development of new established metrics to evaluate these models is thus an important avenue of development.
%However, no method to date uses the $RMSD$ measure directly - only \cryodeepmind uses it as a pairwise measure averaged over two ensembles - while it could be a unifying metric that compares methods according to their end goal: an atomic-level reconstruction. 
%In the more specific context of cryoEM, atomic models can be built \emph{a posteriori} by fitting them in the reconstructed 3D maps. This task offers its own challenges which are summarized in Lawson \textit{et al.} \cite{Lawson2021} However, as seen in Section~\ref{sec1-generative_models_and_lvms}, a number of recent methods directly reconstruct atomic models from images without resorting to building 3D maps first, calling for new approaches for assessing the error made on the predicted position of atoms, a new proxy for the achieved spatial resolution of the reconstruction.
\end{description}
%is typically done through a set of experiments on synthetic and experimental data. Synthetic data is usually simulated with a known reference volume that is projected using a forward model such as the one in Eq.\ref{eq:image} to generate ``mock images" with known CTF, rotation angles and controlled signal-to-noise ratios. Synthetic datasets allow in particular to evaluate a method's accuracy in recovering any hidden variables, while keeping the others fixed and assuming that they are known. The metrics used to evaluate the quality of the reconstruction in synthetic and experimental settings typically involve computing \footnote{We refer the reader to the excellent review by Singer \textit{et al.}\cite{singer2020computational} for a wider description of the topic.}:
%\begin{description}[noitemsep, topsep=0.1em]
%\item[Fourier Shell Correlation (FSC) between two maps $U$ and $V$:] As described in greater details by Singer et al\cite{singer2020computational}, this quantity measures the correlation over a 3D shell between two reconstructed volumes, defined as:
%$$ FSC (k)= \frac{\sum_{s \in S_k}U_sV_s^*}{\sqrt{\sum_{s \in S_k} |U_s|^2 \sum_{s \in S_k} |V_s|^2} } $$
%where $S_k$ is the set of Fourier voxels in a spherical shell at distance $k$ from the origin, and
%$U$ and $V$ are the Fourier transforms of the 3D volumes that we need to compare. Typically, $U$ and $V$ are the reconstructed volumes inferred separately on two halves of the dataset: the method is said to perform well if the two reconstructed volumes $U$ and $V$ are similar, and the resolution of the method's reconstruction is estimated as the best resolution for which $U$ and $V$ agree. The FSC is close to 1 when the two maps are close. This is typically the case for small $k$, as low-frequency signal is strong, but FSC generally decays
%to zero as the signal-to-noise decreases. The result is often plotted as a curve, with axis $x=k$. The final resolution of the recovered map corresponds to the maximum value of $k$ such that $FSC(k) \geq 0.143$ --- a criterion that is chosen to match resolution criteria used in X-ray crystallography.  This is one of the most standard reference metrics in cryoEM. In fact, most methods (with the exception perhaps of \cryodeepmind) reviewed in the present paper use this metric to evaluate their recovered spatial resolution.
%\item[Fourier Shell Correlation between map and atomic model] This is a variation on the previous metric and
%called the ``map-to-model FSC''.  In this case, the reported resolution is the maximum value of  $k$ such that the Fourier Shell Correlation is above 0.5. For instance, \relion  reports, on top of two-halves FSCs,  FSC calculations against available crystal structure as an additional objective inidication of reconstruction quality.
%\item[Variants of the Root Mean Squared Error (RMSE).] This method compares the root-mean-square deviation between 3D map. However, because images are random samples from the underlying volume, this metric needs to be adapted to compare distributions --- which is done by using the Earth Mover (or Wasserstein) Distance:  ground truth samples and predictions are aligned, their RMSD computed. An optimal assignment algorithm is then run to assign each ground truth sample to a corresponding prediction, and the reported RMSD is computed on this  assignment. This is one of the metrics used by  \cryodeepmind to evaluate their algorithm.
%\end{description}
%On an additional note, the validity of the pose imputation part of the algorithm (if present) is typically performed via a synthetic ablation study, where all other variables are assumed to be known. Results are shown as a histogram of residuals in rotation angles.


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}



\subsubsection{Assessing Conformation Resolution: An Ill-Defined Problem} 

While not flawless, the evaluation of spatial resolution is a relatively well-characterized task. By contrast, evaluating conformation heterogeneity is a more ambiguous problem. To evaluate the quality of the reconstructions allowing continuous heterogeneity, methods such as \threedflex or \cryodrgn perform a post-hoc analysis of the recovered latent space, showing the flexible deformation that are induced by sweeping through the space of possible $z$s and visually inspecting the corresponding deformations. However, proper objective and quantitative measures of conformation heterogeneity remain to be established: there currently exists no standardized measure or gold-standard task to evaluate how well a method is able to capture it.

We could design a new metric, inspired by the high-level idea of the FSC. Using two halves of the dataset to infer two independent continuous distributions of conformations, we evaluate whether the distributions agree using a metric such as the Wasserstein distance - modulo change of coordinate system for the conformation variable $z$. In the case where a ground-truth conformation is available for each image (e.g. in simulations), the inferred distribution could be compared to the true distribution. 
In the case of methods able to generate one 3D volume for each image in the dataset, one could consider a hierarchical clustering approach where depth in the hierarchy tree corresponds to the conformational resolution. In more concrete terms, for all resolution $k$, the FSC between each volume pairs would be measured and the resulting distance matrix used for clustering. Data points that fall within the same clusters would be indistinguishable at $k$ while images that would fall in different clusters would correspond to conformations that differ by at least $k$.
The development of such metrics is key to make sustainable advances in next-generation cryo-EM reconstructions. 
% \todo[inline]{TO BE DEVELOPED:\\
% In fact, evaluating heterogeneity holds several challenges:
% (a) defining a distance between conformations,\\
% (b) determine the (physical?) validity of these conformations 
% }



\subsection{Quantitative Comparison of Performances: Lack of Common Benchmarks} 

Beyond the need for new performance metrics that are better adapted to new advancements in the field, it is most certainly the lack of established benchmarks that, to this day, make reconstruction methods very hard to compare.
%Perhaps partly due to the relatively novel use of deep learning methods for cryo-EM molecular reconstruction, there exists no standard benchmarks for evaluating a method's performance --- or at least, not to the authors' knowledge. 
Such benchmarks are dramatically needed, as we cannot rely on statistical theory since the convergence properties of estimations relying on (amortized) variational inference are not completely characterized. In fact, the quantitative assessment of the methods' relative performance has yet to overcome three main hurdles:
\begin{description}[noitemsep, leftmargin=0cm, topsep=0.05cm,labelindent=0cm]
\item [\bf (i) Lack of benchmark datasets:] Current methods are developed and tested 
%“in-house” datasets (comprising real and/or simulated cryo-EM images), neither readily available to the public nor easy to compare. 
on a wide range of synthetic and experimental datasets that differ in the nature of the biomolecule being imaged, the dataset size, image size and associated resolution --- with very little overlap across methods - see Table~\ref{tab:experiments}. There is unfortunately no ``MNIST''\cite{deng2012mnist} or ``Imagenet''\cite{deng2009imagenet} for cryo-EM. Most methods resort to evaluating their performance on synthetic data,
%, thereby controlling certain variables such as noise levels.
%--- thereby allowing them to control and assume known certain variables, such as pose for instance, and evaluate the accuracy of the reconstruction with one variable at a time. 
yet no cryo-EM simulator acts as a standard to generate simulated images in a unified way. Synthetic datasets vary in the realism of the image formation model used for simulation, \textit{e.g.} in the noise model, the signal-to-noise ratio or the distribution of nuisance variables (e.g. poses). Subsequent experiments are typically performed on real ``in house'' data --- but there too, the important diversity within the characteristics of these evaluation datasets therefore makes the comparison of these methods a strenuous task.
\item[\bf (ii) Lack of benchmarking  procedures:] Reconstruction methods vary in the complexity of the task that they set out to accomplish, assuming more or less nuisance variables (such as poses or PSF) to be known -- see Table~\ref{tab:volumes} and Figure~\ref{fig:vae}. This makes it difficult to compare methods on a fair ground. We need to establish modular benchmarking procedure that  would enforce a  fair comparison of reconstruction performances, eg, testing the recovery of the pose, volume or conformations, with other nuisance variables being known and fixed.%, as well as 
\item [\bf (iii) Lack of benchmark codebase and infrastructure:] Finally, reconstructions methods are not necessarily publicly accessible, are implemented across different programming languages, and/or are tested on different software or hardware. Creating a codebase that re-implements these methods for a proper evaluation using a unified infrastructure would unfortunately represent a gigantic implementation effort. Currently, this lack of codebase poses a significant hurdle in the accessibility and comparison of the methods: it is currently impossible to disentangle the effect of their proposed statistical learning problem, their programming language, implementation tricks, or software infrastructure.
\end{description}

%As a result of this lack of benchmark, methods are still developed mostly ``agnostically'' to one another.

\subsection{Qualitative Comparison of Performances}

Despite the hurdles associated with performing quantitative comparisons, we propose a  qualitative evaluation of  the different methods based on both published results and our personal experience. This allows us to highlight promising directions  --- to the  least, in the authors' opinion --- for further developments. %This brings us to detail our perspective on the most promising directions taken by the field, and whether recent deep learning reconstruction methods are deemed to replace traditional reconstruction pipelines.

\subsubsection{Accuracy}

% As methods are inherently designed to do different tasks (some focus on recovering the poses - e.g. \cryovaegan -  while others are more holistic - e.g. \cryodrgn), we compare how they perform on each of the components of the pipeline. The experiments led by the methods reviewed in this paper are summarised in Appendix \ref{appF-experiments}:
Despite encouraging accuracy results, some methods seem to face considerable challenges when applied to real cryo-EM images, as they have not been properly vetted and stress-tested in experimental conditions \cite{Ullrich2019,zhong2021exploring, Rosenbaum2021, Nashed2021endtoend} -- see  Table~\ref{tab:experiments}. We consider the lack of results on experimental data as a proxy for a limited applicability in the context of real signal-noise ratios regimes. In order to be adopted by cryo-EM practitionners, these methods will need to overcome the signal-noise regime and demonstrate the accuracy reported in the papers on a larger set of (benchmark) datasets.


Despite the difficulty of the task and lack of standardized benchmarks, recent developments in deep generative modeling have shown impressive promise in overcoming the current computational and accuracy bottlenecks in all three following directions:
\begin{description}[noitemsep, leftmargin=0cm, topsep=0.05cm,labelindent=0cm]
\item[\bf (i) Poses:] Poses are important nuisance variables that have the potential to damage the reconstruction, if incorrectly predicted. Accuracy of the predicted rotation is measured on synthetic datasets with a mean/median square error (MSE) against the corresponding ground-truth. Historically, preference was given to methods that did not use amortized inference for the rotation estimation (e.g. \cryosparc or \cryodrgn), as they  outperformed their amortized counterparts predicting rotations with an encoder (e.g. \cryoposenet and \cryoai): \cryodeepmind was for instance one of the only methods using amortized inference for the recovery of the poses, and reported difficulties in the joint training of poses and conformation --- highlighting the difficulty of accurate amortized inference in this setting. However, the accuracy gap between methods is closing: \cryoai now showcases an rotation accuracy at the same order of magnitude compared to \cryosparc and \cryodrgn on a real dataset. This was facilitated by the theoretical insights drawn from \cryoai, who show that amortized inference techniques tend to get stuck in local minima where the predicted molecule
contains unwanted planar symmetries due to their projections on a 2D surface.  The solution that they propose to alleviate this problem is to use the symmetrized loss:
$$ \ell_{\text{sym}} = \sum_{i}\min\{||{X}_i - \text{PSF}_i * (t_i \circ \Pi_{2D} \circ R_i) (V^{(i)})||^2, ||R_\pi({X}_i) - \text{PSF}_i * (t_i \circ \Pi_{2D} \circ R_i) ({R}_{\pi}(V^{(i)}))||^2    \}. $$
where $R_\pi$ is a rotation with angle $\pi$.
This has recently opened the door to significant gains in accuracy in the prediction of the poses, allowing for the first time pose estimation to be done through amortized inference. 
We anticipate that it is through such developments and theoretical insights that reconstruction algorithms will be able to fully leverage amortized inference for rotation prediction, hereby providing significant speed-ups.
\item[\bf (ii) Volumes:] Methods based on (pseudo-)atomic volume parametrizations - \egmm, \cryofold and \cryodeepmind - do not compare themselves to their counterparts, probably due to the fact that they were published concurrently in 2021 and/or do not use the same definition of ``pseudo-atoms" that are respectively: means of 3D Gaussian distributions, residues or actual atoms. As a consequence, we do not comment on them. For methods generating 3D maps, it has been reported by Punjani \& Fleet \cite{Punjani2021} that amortized inference can translate into resolution loss. Yet, recent methods such as \cryodrgn and \cryoai publish examples of reconstructed volumes as 3D maps whose resolution is visually comparable to the ones obtained by \cryosparc, on down-sampled imaged. Our opinion is that amortized methods can reach near-atomic resolution reconstructions, but this has not been demonstrated yet. If so, we expect them to replace traditional reconstruction pipelines in the long run, since they offer the promise to be significantly faster and to tackle much larger datasets - a desired feature to enable sufficient sampling of the conformational landscape.
\item[\bf (iii) Conformations:] Methods based on pseudo-atomic volumes parametrizations do not provide examples of conformation trajectories that allow us to compare them. For methods generating 3D maps, \cryodrgn and \threedflex seem to be some of the most promising approaches, as they seem to allow greater resolutions in the recovered trajectories, based on our personal visual assessment of the examples of conformation trajectories shown in the corresponding papers. This remains to be confirmed by a quantitative assessment over a larger number of conformation trajectories.
\end{description}



\subsubsection{Reproducibility}

Adoption of these methods by practitioners will require their reproducibility, or robustness to different initializations, implementation tricks or choice of hyperparameters:
\begin{description}[noitemsep, leftmargin=0cm, topsep=0.05cm,labelindent=0cm]
\item[\bf (i) Initialization:] The non-convex nature of the problem puts it at very high-risk of being non robust and sensitive to initialization --- this is a phenomenon sometimes referred to as ``Einstein from noise''\cite{henderson2013avoiding} (also described in Singer \textit{et al.} \cite{singer2020computational}).
%the model is too heavily biased towards a reference template, and the optimization scheme fails to find the true signal in the data --- ``hallucinating'' instead a solution close to the initialization point. 
Luckily, most of the current methods show encouraging signs of robustness to perturbations. In our experience, \cryodrgn seems consistent for different random initializations of the neural model when fixing the poses: the conformation space does not seem to be vastly affected.
This robustness can however be challenged by extremely low signal and/or heterogeneous datasets, in which case certain conformations can go missing. 
\item[\bf (ii) Tricks:] The inference methods presented often make use of additional implementation tricks (e.g. warm-starting with a known conformation), and specific regularization schemes: e.g. \cryodeepmind suggests starting with an initial phase of pose-only training, which, once realized, ensures that the further joint learning of poses and volume is successful. Both \cryodeepmind and \cryofold regularize the recovered structure by penalizing bond lengths, but the impact of the regularization yet remains to be properly characterized, and in particular, its potential to frustrate the optimization landscape. The importance of tricks and regularizations, and combinations thereof, is still ill-understood and would require an in-depth analysis, as it
%reports that warm-starting their algorithm is essential in ensuring the success of the volume recovery: they 
hints towards a difficult optimization landscape for this method, and its sensitivity to initial conditions.
\item[\bf (iii) Hyperparameters:] Choosing hyperparameters such as the dimension of the latent space in algorithms such as \cryodrgn induces more or less regularization: too small and it regularizes the model too much; too large leads to underfitting of the 3D model. \cryodrgn usually sets it to $d=8$, but, given how heterogeneity arises, this is necessarily molecule dependent. The field will need --- to the least--- rule-of-thumb guidelines on how to choose these hyperparameters if these methods are to be adopted by practitioners.
\end{description}

The robustness of these new methods needs to be confirmed on a wider set of datasets, including datasets with high levels of noise. The fact that they rely on user-defined implementation tricks and hyperparameters might not be an obstacle to their adoption, as conventional methods such as \relion or \cryosparc also do.

%However, in a large amount of settings, \cryodrgn manages to find consistent conformations when the poses are fixed. 
%Its capacity to operate reliably when the poses are unknown remains to be evaluated.

% Moreover, each inference method (from Section~\ref{sec2-inference}) uses a different parametrization of the volume (from Section~\ref{sec1-generative_models_and_lvms}). It is thus challenging to disentangle the importance of each choice in the reconstruction pipeline. 


\subsubsection{Efficiency}

Our last axis of comparison is computational efficiency: both in time and memory requirements. First, if we take the size of the datasets used in experiments as a proxy for efficiency, then \threedflex, \cryoai, \egmm, and \cryodrgn seem to be able to process remarkable amounts of information. Additionally, we offer our own practical experience by-way of rule of thumb.
%with the hope of guiding the practitioner in correctly calibrating their expectations when running the different methods. Overall, cryo-EM volume reconstructions take a considerable amount of time. 
With datasets typically of more than 100GB, training times can take up to 10 hours (including the required pre-processing steps) for methods like \relion --- that is, for a run that has little hyperparameter tuning compared to alternative deep learning methods. Newer methods like \cryodrgn hold great promise in terms of reconstruction: however, such sophisticated methods can further benefit from gains in efficiency, both from the computational side and in terms of memory requirements. Efficient updates of a model's parameters can thus be seen as a current computational bottleneck and offers an interesting avenue for future research.







==> CryoReview 2021 (6)/tables-tgn/table_inference_jan22.tex <==
%[TODO EXPAND ON THIS]
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\scalebox{0.95}{
\begin{tabular}{|c|c|cc|cc|}
\hline
\rowcolor[HTML]{DAE8FC} 
\cellcolor[HTML]{EFEFEF} &
  \textbf{Posterior $p(h_i|x_i)$} &
  \multicolumn{2}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Mode $\hat h_i$}} &
  \multicolumn{2}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Variational $q(h_i)$}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
 &
  \textbf{} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Non-Amortized}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Amortized \\ (encoder)\end{tabular}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Non-Amortized}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Amortized\\ (encoder)\end{tabular}} \\ \hline
Distribution on $h_i$ &
  $p(h_i|x_i)$ &
  \multicolumn{1}{c|}{$ \argmax_{h_i} p(h_i|x_i)$} &
  $\text{Enc}_\xi(x_i)$ &
  \multicolumn{1}{c|}{$q_{\eta_i}  \in \mathcal{Q}$} &
  $q_{\text{Enc}_\xi(x_i)}\in \mathcal{Q}$ \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}\textbf{Name}} &
  \textbf{EM} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Approx. EM}} &
  \textbf{Am. EM / AE} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Var. EM  / AD}} &
  \textbf{Var. Am. EM / VAE} \\ \hline
\cellcolor[HTML]{EFEFEF} &
  \begin{tabular}[c]{@{}c@{}}\relion\\ (rotation $R_i$ and \\ conformation $z_i$) (*)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\relion\\ (noise $\sigma_i$) (*)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}\cryoposenet\\ (rotation $R_i$)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\cryomaxwelling\\ (rotation $R_i$ and \\ conformation $V$)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}\cryodrgn\\ (conformation $z_i$)\end{tabular} \\ \cline{2-6} 
\cellcolor[HTML]{EFEFEF} &
   &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\cryosparc\\ (rotation $R_i$) (*)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}\egmm\\ (conformation $z_i$)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\threedflex\\ (conformation $z_i$)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}\cryovaegan\\ (2D rotation $R_i$\\ and $CTF_i$)\end{tabular} \\ \cline{2-6} 
\cellcolor[HTML]{EFEFEF} &
   &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\cryodrgn\\ (rotation  $R_i$) (*)\end{tabular}} &
   &
  \multicolumn{1}{c|}{} &
  \begin{tabular}[c]{@{}c@{}}\cryodeepmind\\ (rotation $R_i$\\ and conformation $z_i$)\end{tabular} \\ \cline{3-3} \cline{6-6} 
\cellcolor[HTML]{EFEFEF} &
   &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\cryofold\\ (rotation $R_i$) (*)\end{tabular}} &
   &
  \multicolumn{1}{c|}{} &
  \begin{tabular}[c]{@{}c@{}}\cryofold\\ (conformation $z_i$)\end{tabular} \\ \cline{3-3} \cline{6-6} 
\multirow{-5}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Inference on $h_i$\\ (E-step)\end{tabular}} &
  \multirow{-3}{*}{} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\threedflex\\ (conformation $z_i$)\end{tabular}} &
  \multirow{-3}{*}{} &
  \multicolumn{1}{c|}{\multirow{-3}{*}{}} &
  \multicolumn{1}{l|}{} \\ \hline
\end{tabular}
}
\caption{Classification of cryoEM reconstruction algorithms with respect to the inference on the hidden variables $h_i$ . The inference step updates the posterior $p(h_i|x_i$, or its mode $\hat h_i$, or a variational approximation $q(h_i)$ of it --- which corresponds to the 3 main columns of the table. The works by Zhong et al. (2019, 2021) are classified in several cells, as inference of the conformation $z_i$ is performed via a VAE, but the inference of the poses $R_i$ is performed with an optimization algorithm. The notation (*) specifies that the optimization associated with this step is fully performed (until convergence to local extremum) while its absence indicates that only a gradient step is taken toward the optimum.}
\label{tab:inference}
\end{table}

==> appA2-details-input-domain.tex <==

\subsection{Details on Parameterizations using a Discrete Input Domain}


We give details on cryo-EM reconstruction methods which leverage a discrete input domain to represent the biomolecular volume:

\begin{itemize}
\item \relion-Class3D\cite{SCHERES2010295} and \cryosparc use discrete conformational heterogeneity through $K$ clusters and $z \in \{1, ..., K\}$, in Fourier space with a reference-free encoding. As a result, each of the $K$ volumes $\tilde{V}_z$ is parametrized by its $J$ 3D Fourier coefficients, where $J = D^3$. The target of inference is thus the coefficients $\tilde{V}_{j,k}$ for the volume corresponding to each of these $K$ clusters, where $j=1 \cdots J$ indexes the Fourier coefficients, and $k$ the $K$ clusters. \relion-Refine3D is a homogeneous reconstruction method where the volume is a single parameter $\tilde V$ independent of the image $X_i$.

\item \cryoposenet does not consider conformational heterogeneity: it is a homogeneous reconstruction method, where the volume is a single parameter $V$ independent of the image $X_i$. \cryoposenet operates in image space, using a reference-free encoding, where the volume is represented as 3D map over a discrete domain, i.e. as a set of image intensities on the voxel grid: $V \in \mathbb{R}^{D^3}$. \cryogan also uses the same representation in image space with a reference-free encoding for homogeneous reconstruction, while \multicryogan uses the same representation for heterogeneous reconstruction.

\item \threedflex models conformational heterogeneity through a continuous conformation variable $z$, in image space, with a reference-based encoding where the volume is represented as deviations from an initial template $V_0$. Here, Punjani \textit{et al.} propose learning a deformation field $U \in {\mathbb{R}^3}^{D^3}$ with respect to the conformation $V_0$, that is explicitly represented by the coefficients of its 3D vectors at each of the voxels of the discrete domain. Consequently, the function $V$ writes: $V(z) = f(U(z),V_0)$, where $f$ is a ``convection operator" used to deform the volume $V_0$ based on $U$, and $z$ is the conformation variable. The deformation flow $U$ is parametrized through a neural network.
\end{itemize}

\subsection{Details on Parameterizations using a Continuous Input Domain}

We give additional details on the parameterization of the biomolecular volume with (pseudo-)atome coordinates. Among this general
class of methods, different works differ in the interpretation given to the variable $c_j$ and in whether $A_j, \sigma^2_j$ are assumed
to be known:

\begin{itemize}
\item \textbf{ $c_j$ as  coordinates of ``coarse-grained atoms".} The $c_j$ are coordinates of ``coarse-grained atoms", which are not explicitly mapped onto groups of atoms within the molecular structure, nor are they linked by any molecular chain structure, but rather consist of independently moving ``blobs". \egmm introduces this approach and uses it in a reference-free encoding. The authors describe its benefits as (a) reducing the number of parameters to represent the molecule at any level of detail (in constrast with the grid-approaches) and (b) providing a natural way of modeling cryo-EM maps --- which, as described in the introduction, are the projections of the electrostratic potential "blob" around each atom. In \egmm, Chen \textit{et al.} use a conformation variable $z$ that encodes the coefficients $c_j, A_j, \sigma_j^2$ defining $V_z$ in Equation~\eqref{eq:mixture}.
\item \textbf{$c_j$ as 3D coordinates of groups of atoms.}  The $c_j$ are interpreted as coordinates of ``residues", \textit{i.e.} physical groups of atoms that constitute the molecular structure of proteins. \cryofold relies on this approach in a reference-free encoding. The conformation variable $z$ only encodes the coordinates $c_j$, while $A_j = A$ and $\sigma_j = \sigma$ are assumed known and fixed.
\item \textbf{$c_j$ as 3D coordinates of (pseudo)-atoms.} The $c_j$ are coordinates of actual atoms that constitute the molecular structure of proteins, or potentially pseudo-atoms: i.e. a 3D position that does not exactly correspond to the actual atom but averages known positions of real atoms. In \cryodeepmind, Rosenbaum \textit{et al.} explore this approach, using a reference-based encoding. In other words, Rosenbaum \textit{et al.} consider that a template molecular shape $V_0$ is given, with associated coordinates $c_j$ that form a ``base conformation", that is chosen as a folded molecular chain. The volume is here parametrized in terms of the deviations from that template, expressed as residuals, or small variations $\Delta c_j$ corresponding to different conformations relative to this base conformation. In this work, the conformation variable $z$ encodes the deviations $\Delta c_j$ while $A_j = A$ and $\sigma_j = \sigma$ are assumed known and fixed.
\end{itemize}

==> appA4-relion-examples.tex <==
\paragraph{Example: Modeling Choices in \relion-Refine3D \cite{Scheres2012RELION} and \relion-Class3D\cite{SCHERES2010295}} We illustrate the choices that can be made for inference, through the examples of \relion-Refine3D \cite{Scheres2012RELION} and \relion-Class3D\cite{SCHERES2010295}. \relion-Refine3D\cite{Scheres2012RELION} 
assumes the \acrshort{ctf} to be known, and the volume $V^{(i)}=V$ to be a parameter. Given this image generative model, \relion-Refine3D\cite{Scheres2012RELION} uses a Bayesian approach that consists of (a) modeling the unknown parameter $V$ as a random variable, \textit{i.e.} modeling the Fourier coefficients of the volume $\tilde{V}_j$ as random variables, (b) modeling latent variables in $H_i$ as random variables, \textit{i.e.} assuming that the Fourier poses (describing particles' orientation and position) are random variables, and (c) specifying probability distributions on these random variables, \textit{i.e.} priors in statistical terminology. 
Specifically, \relion-Refine3D\cite{Scheres2012RELION} assumes that the Fourier coefficients $\tilde{V}_{j}$ are sampled from independent Gaussian distributions: $\tilde{V}_{j} \sim N(0, \tau_j^2)$, while the pose latent variables are assumed to be uniformly distributed. The purpose of the inference is to find the parameters of the probability distributions --- \textit{i.e}, for the Gaussian variables $\tilde{V}_{j}$, the means and standard deviations --- that best explain the observed data.
\relion-Class3D\cite{SCHERES2010295} operates similarly, but each image is generated from a set of $K$ volumes, $V_1, ..., V_K$, which are parameters modeled as random variables. 

==> dynamics.tex <==
\section{Determination of conformational landscapes}

most recent \cite{GOMEZBLANCO2022106673}

==> tables-tgn/table_inference_jan22.tex <==
%[TODO EXPAND ON THIS]
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\scalebox{0.95}{
\begin{tabular}{|c|c|cc|cc|}
\hline
\rowcolor[HTML]{DAE8FC} 
\cellcolor[HTML]{EFEFEF} &
  \textbf{Posterior $p(h_i|x_i)$} &
  \multicolumn{2}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Mode $\hat h_i$}} &
  \multicolumn{2}{c|}{\cellcolor[HTML]{DAE8FC}\textbf{Variational $q(h_i)$}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
 &
  \textbf{} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Non-Amortized}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Amortized \\ (encoder)\end{tabular}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Non-Amortized}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Amortized\\ (encoder)\end{tabular}} \\ \hline
Distribution on $h_i$ &
  $p(h_i|x_i)$ &
  \multicolumn{1}{c|}{$ \argmax_{h_i} p(h_i|x_i)$} &
  $\text{Enc}_\xi(x_i)$ &
  \multicolumn{1}{c|}{$q_{\eta_i}  \in \mathcal{Q}$} &
  $q_{\text{Enc}_\xi(x_i)}\in \mathcal{Q}$ \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}\textbf{Name}} &
  \textbf{EM} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Approx. EM}} &
  \textbf{Am. EM / AE} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Var. EM  / AD}} &
  \textbf{Var. Am. EM / VAE} \\ \hline
\cellcolor[HTML]{EFEFEF} &
  \begin{tabular}[c]{@{}c@{}}\relion\\ (rotation $R_i$ and \\ conformation $z_i$) (*)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\relion\\ (noise $\sigma_i$) (*)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}\cryoposenet\\ (rotation $R_i$)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\cryomaxwelling\\ (rotation $R_i$ and \\ conformation $V$)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}\cryodrgn\\ (conformation $z_i$)\end{tabular} \\ \cline{2-6} 
\cellcolor[HTML]{EFEFEF} &
   &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\cryosparc\\ (rotation $R_i$) (*)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}\egmm\\ (conformation $z_i$)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\threedflex\\ (conformation $z_i$)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}\cryovaegan\\ (2D rotation $R_i$\\ and $CTF_i$)\end{tabular} \\ \cline{2-6} 
\cellcolor[HTML]{EFEFEF} &
   &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\cryodrgn\\ (rotation  $R_i$) (*)\end{tabular}} &
   &
  \multicolumn{1}{c|}{} &
  \begin{tabular}[c]{@{}c@{}}\cryodeepmind\\ (rotation $R_i$\\ and conformation $z_i$)\end{tabular} \\ \cline{3-3} \cline{6-6} 
\cellcolor[HTML]{EFEFEF} &
   &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\cryofold\\ (rotation $R_i$) (*)\end{tabular}} &
   &
  \multicolumn{1}{c|}{} &
  \begin{tabular}[c]{@{}c@{}}\cryofold\\ (conformation $z_i$)\end{tabular} \\ \cline{3-3} \cline{6-6} 
\multirow{-5}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Inference on $h_i$\\ (E-step)\end{tabular}} &
  \multirow{-3}{*}{} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\threedflex\\ (conformation $z_i$)\end{tabular}} &
  \multirow{-3}{*}{} &
  \multicolumn{1}{c|}{\multirow{-3}{*}{}} &
  \multicolumn{1}{l|}{} \\ \hline
\end{tabular}
}
\caption{Classification of cryoEM reconstruction algorithms with respect to the inference on the hidden variables $h_i$ . The inference step updates the posterior $p(h_i|x_i$, or its mode $\hat h_i$, or a variational approximation $q(h_i)$ of it --- which corresponds to the 3 main columns of the table. The works by Zhong et al. (2019, 2021) are classified in several cells, as inference of the conformation $z_i$ is performed via a VAE, but the inference of the poses $R_i$ is performed with an optimization algorithm. The notation (*) specifies that the optimization associated with this step is fully performed (until convergence to local extremum) while its absence indicates that only a gradient step is taken toward the optimum.}
\label{tab:inference}
\end{table}
